Lower Bounds for Matroid Optimization Problems with a Linear Constraint

We study a family of matroid optimization problems with a linear constraint (MOL). In these problems, we seek a subset of elements which optimizes (i.e., maximizes or minimizes) a linear objective function subject to (i) a matroid independent set, or a matroid basis constraint, (ii) additional linear constraint. A notable member in this family is budgeted matroid independent set (BM), which can be viewed as classic $0/1$-knapsack with a matroid constraint. While special cases of BM, such as knapsack with cardinality constraint and multiple-choice knapsack, admit a fully polynomial-time approximation scheme (Fully PTAS), the best known result for BM on a general matroid is an Efficient PTAS. Prior to this work, the existence of a Fully PTAS for BM, and more generally, for any problem in the family of MOL problems, has been open. In this paper, we answer this question negatively by showing that none of the (non-trivial) problems in this family admits a Fully PTAS. This resolves the complexity status of several well studied problems. Our main result is obtained by showing first that exact weight matroid basis (EMB) does not admit a pseudo-polynomial time algorithm. This distinguishes EMB from the special cases of $k$-subset sum and EMB on a linear matroid, which are solvable in pseudo-polynomial time. We then obtain unconditional hardness results for the family of MOL problems in the oracle model (even if randomization is allowed), and show that the same results hold when the matroids are encoded as part of the input, assuming $P \neq NP$. For the hardness proof of EMB, we introduce the $\Pi$-matroid family. This intricate subclass of matroids, which exploits the interaction between a weight function and the matroid constraint, may find use in tackling other matroid optimization problems.

==> Implications.tex <==
\section{Implication for a Parameterized Matroid Problem}
\label{sec:additional}


In this Section we describe  an additional implication of \Cref{thm:emi} for a parameterized decision problem considered by Fomin et al.\ \cite{FGKSS23}. In \cite{FGKSS23} the authors present a ``pseudo-polynomial parameterized algorithm'' for a matroid problem in which the matroid is representable over a finite field. We use \Cref{thm:emi} to show the result cannot be extended to arbitrary matroids in the oracle model while retaining a similar running time. 


Given a graph $G=(V,F)$ and a path $Q$ in $G$ we use $V(Q)$ to denote the set of vertices on the path $Q$.   Consider the following problem.
%Consider for example {\em generalized weighted colored paths} problem considered by Fomin et al.\ \cite{FGKSS23}.

\problem{  {\sc Generalized Weighted Colored Paths} (GWCP)}{
	{\bf Instance }  & An undirected  graph $G=(V,F)$, two sets $A,B\subseteq V$, a representable matroid $(V, \cI)$ over a finite field of order $q$ (that is, the elements of the matroid are the vertices of the graph), and $p,k,T\in \mathbb{N}$.\\
	{\bf A solution} & $p$ vertex disjoint paths $Q_1,\ldots, Q_p$  starting from a vertex in  $A$ and terminating in a vertex in  $B$, such that there is $X\subseteq V(Q_1)\cup \ldots \cup V(Q_p)$  which satisfies $X\in \cI$, $w(X)=T$ and $|X|=k$. \\
	{\bf Objective}& Decide if there is a solution.
}

In \cite{FGKSS23} the authors proposed an algorithm for GWCP which runs in time $2^{p+O(k^2 \log(q+k ))} \cdot n^{O(1)}\cdot T$, where $n$ is the number of vertices of the input graph (Theorem 1.5 in \cite{FGKSS23}, the problem was not given a name in \cite{FGKSS23}).  
Similar to the algorithm of \cite{CGM92} for representable EMI, the algorithm of~\cite{FGKSS23} is algebraic and relies on the DeMillo-Lipton-Schwartz-Zippel lemma for polynomial identity testing~\cite{Sc80,DL78,Zi79}.
 Consider the following variant of GWCP, in which the matroid is arbitrary and given via a membership oracle. 

\problem{  {\sc Oracle Generalized Weighted Colored Paths} (Oracle-GWCP)}{
	{\bf Instance }  & $(G=(V,F),A,B,\cI,p,k,T)$ where  $G=(V,F)$ is an undirected graph, $A,B\subseteq V$, $(V, \cI)$ is a matroid, and $p,k,T\in \mathbb{N}$.\\
	{\bf A solution} & $p$ vertex disjoint paths $Q_1,\ldots, Q_p$ starting from a vertex in  $A$ and terminating in a vertex in  $B$, such that that there is $X\subseteq V(Q_1)\cup \ldots \cup V(Q_p)$  which satisfies $X\in \cI$, $w(X)=T$ and $|X|=k$. \\
	{\bf Objective}& Decide if there is a solution.\\
	{\bf Model}& The independent sets of the matroid are accessible only via a membership oracle. 
}


We can use \Cref{thm:emi} to show a lower bound on the running time of algorithms for  Oracle-GWCP. 
\begin{lemma}
There is no randomized algorithm for \textnormal{Oracle-GWCP}  which runs in time $g(k,p)\cdot (n\cdot T)^{O(1)}$ for some function $g(k,p)$.
\end{lemma}
\begin{proof}
Assume towards contradiction that there is a randomized algorithm  $\cA$ for Oracle-GWCP   which runs in time $g(k,p)\cdot (n\cdot T)^{O(1)}$ for some function $g(k,p)$.  Consider the following algorithm for EMI, to which we refer as $\cB$, whose input is an EMI instance $I=(E,\cI,w,k,T)$.
\begin{itemize}
	\item If $|E|<2$ then solve the instance checking for every $S\subseteq E$ if it is a solution.
	\item   Let $E=\{e_1,\ldots, e_n\}$;  define $A=\{e_1\}$, $B=\{e_n\}$, $F=\{ (e_i,e_{i+1})~|~1\leq i<n\}$, and $p=1$. 
	\item  Use $\cA$ to solve the Oracle-GWCP instance $J=(G=(E,F),A,B,\cI, p,k,T)$. If $\cA$ determines  that $J$ is a ``yes''-instance then return that $I$ is a yes-instance. Otherwise, return that $J$ is a ``no''-instance. 
\end{itemize}
Observe that the graph $G=(E,F)$ is a path from $e_1$ to $e_n$ which traverses all the elements (vertices) in $E$. 
Consider the execution of the algorithm given an instance $I=(E,\cI,w,k,T)$. Clearly, the algorithm returns a correct solution in case $|E| <2$. Hence, we may assume w.l.o.g. that $|E|\geq 2$.  Let~$J$ be the Oracle-GWCP instance constructed by the algorithm.

\begin{claim}
	\label{claim:gwcp}
	The \textnormal{EMI} instance $I$  is a ``yes''-instance iff  the \textnormal{Oracle-GWCP} instance $J$ is a ``yes''-instance.
\end{claim}
\begin{claimproof}
	If $I$ is a ``yes''-instance, let $X$ be its solution. Also, let $Q_1$ be the single path in $G$ from $e_1$ to $e_n$. It holds that  $X\subseteq V(Q_1)=E$. Since $X$ is a solution for $I$, we have $X\in \cI$, $|X|=k$ and $w(X)=T$. That is, $Q_1$ is a solution for $J$, and therefore $J$ is a yes instance.
	
	If $J$ is a ``yes''-instance then there is a path $Q_1$ from $e_1$ to $e_n$ and $X\subseteq V(Q_1)$ such that $X\in \cI$, $|X|=k$ and $w(X)=T$. Thus, $X$ is a solution for $I$, and therefore $I$ is a ``yes''-instance.
\end{claimproof}

By \Cref{claim:gwcp}, and since $\cA$ is a randomized algorithm for Oracle-GWCP, it holds that $\cB$ is a randomized algorithm for EMI. The running time of $\cB$ is $g(k,1)\cdot (n\cdot T)^{O(1)}$, in contradiction to \Cref{thm:emi}. Thus, there is no randomized algorithm for Oracle-GWCP which runs in time $g(k,p)\cdot (n\cdot T)^{O(1)}$. 
	
\end{proof}

%
%It can be easily observed that an algorithm for Oracle-GWCP with running time of the form $g(k,p) \cdot \left(n\cdot T\right)^{O(1)}$  for an arbitrary function $g$ can be used to decide EMI in time $f(k) \cdot \left(|I|\cdot T\right)^{O(1)}$. Given an EMI instance $(E,\cI,w,k,T)$  we can generate a graph $G=(E,F)$ where $F$ is a path between two arbitrary elements $a,b\in E$. Also, define $A=\{a\}$ and $B=\{b\}$. It can be easily verified that this Oracle-GWCP has a solution if and only if the EMI instance is a yes instance. Thus, an Oracle-GWCP algorithm in time  $g(k,p) \cdot \left(n\cdot T\right)^{O(1)}$ implies an EMI algorithm in time $g(k,1)\cdot (|I| \cdot T)^{O(1)}$,  in contradiction to  \Cref{thm:emi}.

==> LowerBounds-Absolute.tex <==
\section{Tight Lower Bounds using $\Pi$-Matroids}
\label{sec:tight_absolute}
In this section we use \Cref{thm:emb} and \Cref{cor:deter} to prove \Cref{thm:main}. We rely on the following reduction.

\begin{definition}
	Given an \textnormal{EMB} instance $I =(E,\cI,c,k,T)$ and non-trivial  \textnormal{MOL} problem $P \in \cP \setminus \{(\min,\IS,\leq)\}$ where $P = (\opt,\cF,\triangleleft)$, define $R_P(I) = (E,\cI,v_I,w_{I,P},B_{I,P})$ as the {\em reduced} $P$ instance of $I$ as follows.
	\begin{enumerate}
		\item Define the following auxiliary variable \begin{align*}
		%	n & : \text{The variable representing a natural number.} \\
			d(P) = & \begin{cases}
				0 & ~~\text{if  } \left(\opt = \max, \triangleleft = \leq \right) \text{ or } \left(\opt = \min, \triangleleft = \geq \right) \\
			1 & ~~\text{otherwise.}
			\end{cases}
		\end{align*}
		
		\item For all $e \in E$ define $v_I(e) = 2 \cdot c(E)+c(e)$. 
		\item For all $e \in E$ define $w_{I,P}(e) = 2 \cdot c(E)+c(e) \cdot (-1)^{d(P)}$.
		\item Define $B_{I,P} = k \cdot 2 \cdot c(E)+T \cdot  (-1)^{d(P)}$. 
	\end{enumerate}
\end{definition}



%, our lower bounds for {\sc budgeted matroid independent set}, {\sc exact weight matroid independent set}, {\sc constrained minimum weight basis of a matroid}, and {\sc knapsack cover with a matroid}. All proofs use reductions from the $\Pi$-matroid problem.

%In all of the constructions, we are able to use (with slight modifications) the same family of {\em standard weight} functions and {\em standard budgets}. 


%Specifically, for every $n \in \mathbb{N}_{>0}$ define the standard weight function of $n$ as $w_{n}:[n] \rightarrow \mathbb{N}$ such that for all $i \in [n]$
% \begin{equation}
%	\label{eq:w}
%	w_{n}(i) = i+2 \cdot \textnormal{\textsf{sum}}([n]). 
%\end{equation}
%Also, define the standard budget of  $n,k,\alpha \in \mathbb{N}_{>0}$  as 
%\begin{equation}
%	\label{eq:B}
%	B_{n,k,\alpha} = \alpha+2 k \cdot \textnormal{\textsf{sum}}([n]). 
%\end{equation}

%In deriving the lower bounds for our problems (in
%\Cref{sec:abs_BM,sec:abs_EMI,sec:abs_CMB,sec:abs_KCM}), we use some general results, as stated in \Cref{lem:OPTu,lemma:if,lemma:onlyif}.
The following lemma gives a polynomial bound on the total weight of any subset of the ground set of a reduced instance. 

\begin{lemma}
	\label{lem:OPTu}
%	For every $n \in \mathbb{N}_{>0}$ and $S \subseteq [n]$, it holds that $w_{n}(S) \in \{0,1,\ldots, 3 \cdot n^3\}$. 
	Given an \textnormal{EMB} instance $I =(E,\cI,c,k,T)$ and non-trivial  \textnormal{MOL} problem $P \in \cP \setminus \{(\min,\IS,\leq)\}$ where $P = (\opt,\cF,\triangleleft)$, for every $S \subseteq E$ it holds that $v_{I}(S) \in \{0,1,\ldots, 2 \cdot c(E) \cdot k\}$.  
\end{lemma}

\begin{proof}
	By \eqref{eq:w} we have that $w_{n}(S) \in \mathbb{N}$. Furthermore,  $0 = |\emptyset| \leq |S| \leq \textsf{sum}(S) \leq w_{n}(S)$, and  $$w_{n}(S) \leq n \cdot \max_{i \in [n]} w_{n}(i) = n \cdot \max_{i \in [n]} i+ n \cdot (2 \cdot \textsf{sum}([n])) \leq n^2+ 2 \cdot n^3 \leq 3 \cdot n^3.$$ 
\end{proof}


We use the sets $\mathcal{J}_{n,k}$, $\mathcal{K}_{n,k,\alpha}$, $\mathcal{L}_{n,k,\alpha}(\Pi)$ and $\cI_{n,k,\alpha}(\Pi)$  as in \Cref{def:Matroid}. As in \Cref{sec:Pi} we often omit the subscripts $n,k$ and $n,k,\alpha$ when those are known by context. 
In the next two lemmas, we show that finding  $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$ (with appropriate parameters) is equivalent to finding~$S \in \cI_{n,k,\alpha}(\Pi)$ such that $w_n(S) = B_{n,k,\alpha}$. For the first direction, we have
\begin{lemma}
	\label{lemma:if}
	For every $n,k,\alpha \in \mathbb{N}_{>0}, \Pi \subseteq 2^{[n]}$, and $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$, it holds that $w_{n}(S) = B_{n,k,\alpha}$. 
\end{lemma}
\begin{proof}
	Let $S \in \mathcal{L}(\Pi)$. By \eqref{eq:1}, $|S| = k$ and $\textnormal{\textsf{sum}}(S) = \alpha$. %In addition, let $D = \{x_i~|~i \in S\}$. 
	Therefore, \begin{equation*}
		\label{eq:ole}
		\begin{aligned}
			w_{n}(S) = \sum_{i \in S} \left( i+2 \cdot \textnormal{\textsf{sum}}([n])  \right) = \textnormal{\textsf{sum}}(S)+|S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) = \alpha+2 k\cdot \textnormal{\textsf{sum}}([n]) = B_{n,k,\alpha}. 
		\end{aligned}
	\end{equation*}
	%	 The last equality holds because $\alpha = \textnormal{\textsf{sum}}(S) \leq \textnormal{\textsf{sum}}([n])$. 
	%	Since $S \in \mathcal{L}(\Pi)$ it holds that $S \in \cI$. Thus, by \eqref{eq:ole} $S$ is a solution for $U$ of profit exactly $B$. 
\end{proof}


For the second direction, we show the next result.
\begin{lemma}
	\label{lemma:onlyif}
	Let $n,k, \in \mathbb{N}_{>0}, \alpha \in \left[ n^2\right], \Pi \subseteq 2^{[n]}$, and $S \in \cI_{n,k,\alpha}(\Pi)$ such that $w_{n}(S) = B_{n,k,\alpha}$. Then, $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$. 
\end{lemma}
\begin{proof}
	%Let $F$ be a solution for $U$ of profit at least $B$. Since $c(e) = p(e)$ for every element $e \in E$, then $p(F) = c(F) \leq B$, since $F$ satisfies the budget constraint; thus, since $p(F) \geq B$ we conclude that $p(F) = c(F) = B$. 
	Since $S \in \cI_{n,k,\alpha}(\Pi)$, by \eqref{eq:1}, it suffices to show that $|S| = k$ and $\textsf{sum}(S) = \alpha$. First, assume towards contradiction that $|S| \neq k$. By \eqref{eq:1}, this implies that  $|S|< k$. Thus,
	%We consider two cases. 
%	\begin{enumerate}
%		\item $|S|< k$. Then, 
\begin{equation}
			\label{eq:ol3}
			\begin{aligned}
				w_{n}(S) ={} & \sum_{i \in S} i+|S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
				\leq{} & \sum_{i \in S} i+(k-1) \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
				\leq{} &  \textnormal{\textsf{sum}}([n])+(k-1) \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
				<{} & 2 k\cdot \textnormal{\textsf{sum}}([n]) \\
				<{} & B_{n,k,\alpha}.
			\end{aligned}
		\end{equation} 
		
The last inequality holds since $\alpha \geq 1$. By \eqref{eq:ol3}, we reach a contradiction to $w_{n}(S) = B_{n,k,\alpha}$.		
		
%		\item $|S|>k$. Since $S \in \cI_{n,k,\alpha}(\Pi)$, by \eqref{eq:1} it holds that $|S| \leq k$ and we reach a contradiction. 
		
		\comment{
			\begin{equation}
				\label{eq:ol2}
				\begin{aligned}
					w_{n}(S) ={} & \sum_{i \in S} i+|S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
					\geq{} & \sum_{i \in S} i+(k+1) \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\ 
					\geq{} & 2  \cdot \textnormal{\textsf{sum}}([n]) +2 k\cdot \textnormal{\textsf{sum}}([n]) \\
					>{} & B_{n,k,\alpha}.
				\end{aligned}
			\end{equation}
			The last inequality holds since: if $n = 1$ then $\alpha \leq 1 < 2 \cdot \textsf{sum}([n])$; otherwise, $n > 1$ and it follows that $\alpha \leq n^2 < n^2+n = 2 \cdot \textnormal{\textsf{sum}}([n])$. }%By \eqref{eq:ol2} we reach a contradiction since $F$ is a solution for $U$.
%	\end{enumerate}
We conclude that $|S| = k$. Therefore, 
	$$\textnormal{\textsf{sum}}(S) = \sum_{i \in S} i = w_{n}(S) - |S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) = w_{n}(S) -  2 k \cdot \textnormal{\textsf{sum}}([n]) = B_{n,k,\alpha} - 2 k \cdot \textnormal{\textsf{sum}}([n]) = \alpha.$$ 
	In summary, we have $S \in \cI(\Pi)$, $|S| = k$ and $\textnormal{\textsf{sum}}(S) = \alpha$. By \eqref{eq:1}, it follows that $S \in \mathcal{L}(\Pi)$.
\end{proof}

The next result follows directly from \Cref{lemma:if,lemma:onlyif}.
\begin{cor}
	\label{cor:iff}
	For every $n,k \in \mathbb{N}_{>0}$, $\alpha \in \left[ n^2 \right]$, $ \Pi \subseteq 2^{[n]}$, and $S \in \mathcal{I}_{n,k,\alpha}(\Pi)$ it holds that $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$ if and only if %there is $S \in \cI_{n,k,\alpha}(\Pi)$ such that 
	$w_{n}(S) = B_{n,k,\alpha}$. 
\end{cor}

We use \Cref{cor:iff} to derive lower bounds for several weighted matroid problems. For each of these problems, $\cP$, we use a reduction from $\Pi$-matroid. Given an instance $I$ of $\Pi$-matroid, we construct an instance $U$ of $\cP$ using the standard weight and standard budget.
The optimal solution for $U$ is {\em exactly} $B_{n,k,\alpha}$ (with appropriate parameters) iff $I$ has a solution. 
%\begin{proof}
%	%Clearly, if $\alpha \notin \left[ \textnormal{\textsf{sum}}([n])\right]$ then for all $S \subseteq [n]$ it holds that $\textsf{sum}(S) \neq \alpha$; thus, $\mathcal{L}_{n,k,\alpha}(\Pi) = \emptyset$. Therefore,  by \Cref{lemma:onlyif} there is no $F \in \cI_{n,k,\alpha}(\Pi)$ such that $w_{n}(F) = B_{n,k,\alpha}$ and the claim follows. Otherwise, $\alpha \notin \left[ \textnormal{\textsf{sum}}([n])\right]$. In this case, the proof follows by \Cref{lemma:if} and \Cref{lemma:onlyif}. 
%\end{proof}

%\begin{enumerate}
%	%\item There are $n$ elements $E = \{e_1, \ldots, e_n\}$.
%%	\item $\cI = \cI_{n,k,\alpha}(\Pi)$. 
%	\item For every $i \in [n]$ define $c(i) = p(i) = i+2 \cdot \textnormal{\textsf{sum}}([n])$. 
%	\item Define the budget as $B = \alpha+2 k \cdot \textnormal{\textsf{sum}}([n])$.
%\end{enumerate}


\subsection{Budgeted Matroid Independent Set}
\label{sec:abs_BM}

Recall that definition of the BM problem
\problem{ {\sc Budgeted Matroid Independent Set} (BM)}{
	{\bf Instance} &  
	$I = (E,\cI,c,p,B)$, where $(E,\cI)$ is a matroid, $c:E \rightarrow \mathbb{N}$ is  a cost function, $p:E \rightarrow \mathbb{N}$ is a  profit function and $B \in \mathbb{N}$ is the budget\\
	{\bf Solution}& $S\in \cI$ such that $c(S) \leq B$.\\
	{\bf Objective} & Find a solution $S$ of maximum profit $p(S)$. \\
	{\bf Model } &The collection of  independent sets $\cI$ is accessible only via a membership oracle; the encoding size of the instance $I$ is the encoding size of $(E,c,p,B)$ - the instance without $\cI$. 
	%We decided to repeat the model for all problems. --H 
	%\ariel{we need to re-discuss whether we want to repeat this definition over and over}
}
We first show how a reduction from the $\Pi$-matroid problem can be used to rule out the existence of a Fully PTAS for $\BM$. 

%\thmbm*

\begin{proof}
	
	
	%	\noindent{\bf Proof of \Cref{lem:hard}:}
	Assume towards a contradiction that there is a randomized Fully PTAS $\cA$ for $\BM$. We use $\cA$ to decide the $\Pi$-matroid problem.  Let $I = \left(n,k,\alpha,\mm\right)$ be a $\Pi$-matroid instance. Consider the following algorithm $\cB$ that decides $I$.
	\begin{enumerate}
		\item Construct the $\BM$ instance $%U_{n,k,\alpha}(\Pi) 
		U= ([n],\cI_{n,k,\alpha}(\Pi),w_{n},w_{n},B_{n,k,\alpha})$ along with the membership oracle of $M_{n,k,\alpha}(\Pi)$; note that the elements of $U$ are $[n] = \{1,\ldots, n \}$, the independent sets are the independent sets of the $\Pi$-matroid $\mm$ (i.e., $\cI_{n,k,\alpha}(\Pi)$), the standard weight function $w_n$ is both the profit and the cost function, and the budget is simply the standard budget with parameters $n,k,\alpha$. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
		\item Define $\eps = \frac{1}{6 \cdot n^3}$ and compute $\cA$ on $U$ and $\eps$; let $S$ be the returned solution.  
		\item Return that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. 
	\end{enumerate}
	
	Note that $U$ can be constructed from $I$ in time $\io$ and that $\frac{1}{\eps} = |I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is a (randomized) FPTAS. We now show correctness. %For the correctness, %we show that $\cB$ returns that $I$ has a solution if and only if $I$ indeed has a solution. 
	\begin{itemize}
		\item If $\cB$ returns that $I$ has a solution. Then, $w_n(S) = B_{n,k,\alpha}$; since $S$ is a solution for $U$ it also holds that $S \in \cI_{n,k,\alpha}(\Pi)$. Thus, by \Cref{cor:iff} it holds that $I$ has a solution.  
		\item If $I$ has a solution. Then, there is $T \in \mathcal{L}_{n,k,\alpha}(\Pi)$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$ implying that $T$ is a solution for $U$.  Therefore, with probability at least $\frac{1}{2}$: 
		 \begin{equation}
			\label{eq:sOPT}
			B_{n,k,\alpha} \geq \OPT(U) \geq w_n(S) \geq (1-\eps) \cdot w_n(T) \geq  w_n(T)-\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}-\frac{1}{2}.
		\end{equation} 	The first inequality holds since %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
	the profit and the cost of each element are the same, and the cost of a solution cannot exceed the budget. The third inequality follows (with probability at least $\frac{1}{2}$) because $S,T$ are solutions for $U$, and $S$ is computed by a randomized FPTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPT}, %w.p. at least $\frac{1}{2}$ 
it holds that $w_n(S) = B_{n,k,\alpha}$ w.p. at least $\frac{1}{2}$. Then, $\cB$ returns that $I$ has a solution with probability at least $\frac{1}{2}$.  
	\end{itemize}
	%
	%by \Cref{cor:iff} a solution $T$ for $U$  is a solution for $I$ if and only if %therefore, by  it holds that %algorithm $\cA$ returns a solution for $U$ with profit $B_{n,k,\alpha}$

	
	
	%Therefore, there is a solution for $I$ if and only if $\OPT(U) = B_{n,k,\alpha}$; thus, to conclude we show that $w_n(S) = \OPT(U)$ w.p. at least $\frac{1}{2}$. %if and only if $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$ (i.e., $I$ has a solution).
	%	  
	%  
	%	  we show that w.p. at least $\frac{1}{2}$ it holds that: $w_n(S) = B_{n,k,\alpha}$ if and only if I has a solution. 
%	By the approximation guarantee of $\cA$ with our parameter $\eps$, w.p. at least $\frac{1}{2}$ the solution $S$ satisfies \begin{equation}
%		\label{eq:sOPT}
%		\OPT(U)-w_n(S) \leq \eps \cdot \OPT(I) \leq  \frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = \frac{1}{2}.
%	\end{equation} The first inequality follows because $S$ is a solution computed by an FPTAS with the parameter $\eps$. The second inequality holds since $\OPT(U) \leq 3 \cdot n^3$ from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPT}, w.p. at least $\frac{1}{2}$ it holds that $w_n(S) = \OPT(U)$.  %, by the definition of a randomized FPTAS and since $\eps^{-1} = 2 \cdot |I|^c = \io$.  
	%  
	%If $\alpha > \textnormal{\textsf{sum}}([n])$ by \Cref{def:Matroid} and \Cref{def:problem} there is no solution for $I$ and deciding $I$ is trivial. Thus, for the following, assume w.l.o.g. that $\alpha \leq \textnormal{\textsf{sum}}([n])$. 
	%We define the BM instance $U = (E, \cI, c, p, B)$ such that the following holds. 
	%
	%
	%	By \Cref{lem:OPTu}, for all $S \subseteq [n]$ it holds that $w_{n}(S) \in \mathbb{N}$ and that $\OPT \left( U\right) = n^{O(1)} = \left| U \right|^{O(1)}$; thus, $U$ is a scaled instance of BM. Therefore, if BM has a randomized FPTAS, by \Cref{lem:FPTAStoEXACT} there is a randomized exact algorithm $\cA$ that finds in time $|U|^{O(1)} = \io$ an optimal solution for $U$. 
	%	Clearly, $\OPT(U) \leq B_{n,k,\alpha}$ because the profit and the cost of each element are the same, and the cost of a solution cannot exceed the budget. Since $S$ is a solution for $U$ it follows that $S \in \cI_{n,k,\alpha}(\Pi)$; therefore, by \Cref{cor:iff} it holds that %algorithm $\cA$ returns a solution for $U$ with profit $B_{n,k,\alpha}$
	%	Thus, w.p. at least $\frac{1}{2}$, it holds that $w_n(S) = B_{n,k,\alpha}$ if and only if $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$ (i.e., $I$ has a solution). 
	Hence %by computing $\cA$ on $U$ and getting a solution $S$, 
	the algorithm  correctly decides $I$ with probability at least $\frac{1}{2}$. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
	It follows that $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
	a randomized algorithm which decides the $\Pi$-matroid problem, contradicting \Cref{cor:deter}. 
\end{proof}



\subsection{Exact Weight Matroid Independent Set}
\label{sec:abs_EMI}




%	We say that a problem is {\em Strongly} NP-Hard if it remains NP-Hard if all numbers in the instance of the problem are encoded in unary. 
The proof of \Cref{thm:emi} is similar to the proof of \Cref{thm:bm}.
Recall that $S$ is a {\em solution} for an EMI instance $(E,\cI,w,k,T)$ if $S \in \cI$, $|S| = k$, and $w(S) = T$. 
% \begin{lemma}
%	\label{lem:EMI}
%	For any function $f:\mathbb{N} \rightarrow \mathbb{N}$ there is no algorithm that decides \textnormal{EMI} in time $f(k) \cdot (T \cdot n)^{O(1)}$, where $n$ is the number of elements in the given matroid, $k$ is the rank of the matroid, and $T$ is the target value.  
%%	Unless \textnormal{P=NP}, there is no polynomial time algorithm that decides \textnormal{EMI}. %is \textnormal{Strongly NP-Hard}.  
%\end{lemma}

%\thmemi*

\begin{proof}
	Assume towards contradiction that there is a function $f:\mathbb{N} \rightarrow \mathbb{N}$,  and an algorithm $\cA$ for  \textnormal{EMI} which, given an instance $I=(E,\cI,w,k,T)$, runs in time  $f(k) \cdot \left(T \cdot |I|\right)^{O(1)}$.  
	%We use $\cA$ to attain a randomized algorithm for  the $\Pi$-matroid problem. 
	%By \Cref{lem:randomized}, there is a constant $c$ such that there is no randomized algorithm that decides the $\Pi$-matroid problem in time $c \cdot \frac{{n' \choose k}}{{n'}^3}$. %randomized FPTAS $\cA$ for EMI. 
 % Let $I = \left(n,k,\alpha,\mm\right)$ be a $\Pi$-matroid instance such that $7 \cdot n^3+f(k) \cdot (2 \cdot n^4)^{q} < c \cdot \frac{{n \choose k}}{{n}^3}$. Clearly, since $c,q$ are constants, the above inequality is realized by some $n,k$, where $n$ is sufficiently large w.r.t. $k$.
   Consider the following algorithm for the $\Pi$-matroid problem whose input is instance $I=(n,k,\alpha,M_{n,k,\alpha}(\Pi))$, to which we refer as  $\cB$, that decides $I$.
	\begin{enumerate}
		\item Construct the EMI instance $%U_{n,k,\alpha}(\Pi) 
		U= ([n],\cI_{n,k,\alpha}(\Pi),w_{n},k,B_{n,k,\alpha})$ along with the membership oracle of $M_{n,k,\alpha}(\Pi)$; note that the elements of $U$ are $[n] = \{1,\ldots, n \}$, the independent sets are the independent sets of the $\Pi$-matroid $\mm$ (i.e., $\cI_{n,k,\alpha}(\Pi)$), the standard weight function $w_n$ is the weight function, the target cardinality is $k$, and the target value is the standard budget with the parameters $n,k,\alpha$. %We say that $T \subseteq [n]$ is a solution for $U$ if $T \in \cI_{n,k,\alpha}$ and $w_n(T) = B_{n,k,\alpha}$. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
		\item %Define $\eps = \frac{1}{6 \cdot n^3}$ and 
		Execute $\cA$ on the instance  $U$.  %and let $S$ be the returned solution.  
		 Return that $I$ has a solution if and only if $\cA$ returned that $U$ has a solution.  %$w_n(S) = B_{n,k,\alpha}$. 
	\end{enumerate}
	
	We first assert that $\cB$ is a randomized algorithm for the $\Pi$-matroid problem.
		\begin{itemize}
		\item If $\cB$ returns that $I$ has a solution, then the EMI instance $U$ has a solution $S$. 
		That is,~$w_n(S) = B_{n,k,\alpha}$ and $S \in \cI_{n,k,\alpha}(\Pi)$. Thus, by \Cref{cor:iff} it holds that $S\in \mathcal{L}_{n,k,\alpha}(\Pi)$. That is, $S$ is a solution for $I$, and the response of the algorithm is correct. 
		\item If $I$ has a solution then there is $T \in \mathcal{L}_{n,k,\alpha}(\Pi)$; thus, by  \Cref{cor:iff}, it holds that  $w_n(T) = B_{n,k,\alpha}$ and $|T|=k$ by \eqref{eq:1}, implying that $T$ is a solution for $U$. Therefore, with probability  at least $\frac{1}{2}$ it holds that $\cA$ returns that $U$ has a solution; thus, with probability  at least $\frac{1}{2}$ it holds that $\cB$ returns that $I$ has a solution. 
		%		\begin{equation}
			%			\label{eq:sOPT}
			%			B_{n,k,\alpha} \geq \OPT(U) \geq w_n(S) \geq (1-\eps) \cdot w_n(T) \geq  w_n(T)-\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}-\frac{1}{2}.
			%		\end{equation} 	The first inequality holds since %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
		%		the profit and the cost of each element are the same, and the cost of a solution cannot exceed the budget. The third inequality follows (w.p. at least $\frac{1}{2}$) because $S,T$ are solutions for $U$, and $S$ is computed by a randomized FPTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPT}, %w.p. at least $\frac{1}{2}$ 
		%		it holds that $w_n(S) = B_{n,k,\alpha}$ w.p. at least $\frac{1}{2}$. Then, $\cB$ returns that $I$ has a solution w.p. at least $\frac{1}{2}$.  
	\end{itemize}
	Hence, 
	the algorithm correctly decides  $I$ with probability at least $\frac{1}{2}$. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
	It follows that $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
	a randomized algorithm which decides the $\Pi$-matroid problem.
	
	
	
	
	Note that $B_{n,k,\alpha} = 2k \cdot \textsf{sum}(n) \leq 2k \cdot n^2 \leq 2 \cdot n^3$ since $k \leq n$. 
	Thus, $U$ can be constructed in time $|I|^{O(1)}$. 
	Let $q(n,k)$ be the maximum running time of $\cB$ on an instance of the $\Pi$-matroid problem in which the number of elements is $n$ and  the parameter is $k$. Since $\cA$ runs in time $f(k)\cdot (T\cdot |I|)^{O(1)}$ it follows that there is $q\in \mathbb{N}$ such that 
	 $q(n,k)\leq f(k)\cdot (n\cdot 2\cdot n^3)^{O(1)} \leq f(k)\cdot n^{q}$.
	  Furthermore, by  \Cref{lem:randomized} it also holds that $q(n,k) =\Omega\left( \frac{ {n \choose k }}{n^3}\right) $. 
	  Thus, there are $c>0$ and $M>0$ such that for every $n,k>M$ it holds that $q(n,k) \geq c\cdot \frac{ {n \choose k }}{n^3}$. 
	  Select $\tilde{k}=\max\left\{ M+1, q+10\right\}$, then for every $n>M$ such that $k$ divides $n$ we have
	 $$
	 f(\tilde{k})\cdot n^{q} \geq q(n,\tilde{k})\geq  c\cdot \frac{ {n \choose \tilde{k}}}{n^3} \geq c\cdot \frac{\left(\frac{n}{\tilde{k}}\right)^{\tilde{k}}}{n^3 } ,
	 $$
	 where the last inequality uses the inequality ${ n\choose k } \geq \left(\frac{n}{k} \right)^k$ when $k$ divides $n$.
	 Thus,
	 $$
	 f(\tilde{k})\cdot \tilde{k}^{\tilde{k}} \geq   c\cdot n^{\tilde{k}-3-q}.
	 $$
	 The left hand term in the above equation is a constant  in $n$, while the right hand side goes to infinity as $n$ goes to infinity. Thus, we have a contradiction. Therefore, there is no randomized algorithm for EMI which runs in time $f(k)\cdot (T\cdot |I|)^{O(1)}$.
	
	
	%$7 \cdot n^3+f(k) \cdot (B_{n,k,\alpha} \cdot n)^{q} \leq 7 \cdot n^3+f(k) \cdot (2 \cdot n^4)^{q}$. We now show correctness.  %For the correctness, %we show that $\cB$ returns that $I$ has a solution if and only if $I$ indeed has a solution. 
 
\end{proof}


\comment{
	
	\begin{proof}
		
		
		
		We use a reduction from the $\Pi$-matroid problem.	Let $I = \left(n,k,\alpha,\mm\right)$ be a $\Pi$-matroid instance. We define the following BM instance $U = ([n], \cI, w, T)$ such that the following holds. \begin{enumerate}
			%\item There are $n$ elements $E = \{e_1, \ldots, e_n\}$.
			\item $\cI = \cI_{n,k,\alpha}(\Pi)$. 
			\item Define a weight function $w:[n] \rightarrow \mathbb{R}_{\geq 0}$, where for all $vi \in [n]$ it holds that $w(i) = 1+\frac{i}{2 \cdot n^2}$.  
			\item $T = k+\frac{\alpha}{2 \cdot n^2}$. 
			%			\begin{equation}
				%				\label{eq:w}
				%				w(v) = 1+\frac{f(v)}{2 \cdot n^2}. 
				%			\end{equation}
		\end{enumerate}  
		
		%	Let $X = (E,v,\sigma,D,T)$ be an SSG instance and let $n = |E|$. For every $k \in \{0,1\ldots,n\}$ 
		
		%		Define the matroid $M_{\alpha} = (V,\cI_{\alpha})$, $\cI_{\alpha} = \cI^1_{\alpha} \cup \cI^2_{\alpha} \cup \cI^3_{\alpha}$, such that \begin{equation}
			%			\label{eq:1}
			%			\begin{aligned}
				%				\cI^1_{\alpha} = {} & \{S \subseteq V~\big|~ |S| < k\} \\
				%				\cI^2_{\alpha} = {} & \{S \subseteq V~\big|~ |S| = k, f(S) \neq \alpha\} \\
				%				\cI^3_{\alpha} = {} & \{S \subseteq V~\big|~ |S| = k, f(S) = \alpha, S \in C(G)\}. \\
				%			\end{aligned}
			%		\end{equation}
		
		
		%	For every $\alpha \in [n^2]$ let $T_{\alpha} = k+\frac{\alpha}{2 \cdot n^2}$ and define the EMI instance $I_{\alpha} = (V,\cI_{\alpha},w,T_{\alpha})$.
		
		
		% such that the following holds. \begin{equation}
			%	\label{eq:sB2}
			%	\begin{aligned}
				%	c(e) ={} & \beta \cdot \sigma(e) +v(e)  ~~\forall e \in E \\
				%	p(e) ={} & \alpha+\sigma(e)~~\forall e \in E \\
				%	B ={} & \beta \cdot D+T.
				%	\end{aligned}
			%\end{equation}
			%
			
			\begin{claim}
				\label{claim:r<4}
				For every $\alpha \in [n^2]$ and $Q \subseteq V$ it holds that $Q$ is a solution for $I_{\alpha}$ if and only if $Q \in C(G)$, $|Q| = k$, and $f(Q) = \alpha$. 
			\end{claim}
			
			\begin{proof}
				Let $Q$ be a solution for $I_{\alpha}$. Then, \begin{equation}
					\label{eq:2}
					|Q| \leq w(Q) = T_{\alpha} = k+\frac{\alpha}{2 \cdot n^2} \leq k+\frac{n^2}{2 \cdot n^2} < k+1.  
				\end{equation}
				and 
				\begin{equation}
					\label{eq:3}
					|Q| = w(Q)- \frac{f(Q)}{2 \cdot n^2} = T_{\alpha} - \frac{f(Q)}{2 \cdot n^2}= k+\frac{\alpha}{2 \cdot n^2}- \frac{f(Q)}{2 \cdot n^2} \geq k- \frac{f(Q)}{2 \cdot n^2} \geq k - \frac{n^2}{2 \cdot n^2} > k-1.  
				\end{equation} The second inequality holds since $f(V) \leq n \cdot \max_{v \in V} f(V) = n^2$. By \eqref{eq:2} and \eqref{eq:3} we conclude that $|Q| = k$. Moreover, %it holds that $f(Q) = \frac{\alpha}{}$
				\begin{equation}
					\label{eq:a}
					f(Q) = (w(Q) - k) \cdot 2 n^2  = (T_{\alpha}-k) \cdot 2 n^2 = \alpha.  
				\end{equation} The first equality follows from \eqref{eq:w}. We get that $f(Q) = \alpha$ by \eqref{eq:a}. Therefore, since $|Q| = k$, $f(Q) = \alpha$, and $Q \in \cI_{\alpha}$ ($Q$ is a solution for $I_{\alpha}$), it follows that  $Q \in \cI^3_{\alpha}$; thus, $Q \in C(G)$ by \eqref{eq:1}. 
				
				For the other direction, let $Q \subseteq V$  such that $Q \in C(G)$, $|Q| = k$, and $f(Q) = \alpha$. Then, by \eqref{eq:1} it holds that $Q \in \cI^3_{\alpha}$ and therefore $Q \in \cI_{\alpha}$. Moreover, by \eqref{eq:w} it holds that $w(Q) = k+\frac{f(Q)}{2n^2} = k+\frac{\alpha}{2 \cdot n^2} = T_{\alpha}$.  We conclude that $Q$ is a solution for $I_{\alpha}$. 
			\end{proof}
			
			
			To prove the lemma, consider the following cases. \begin{enumerate}
				\item There is a clique $Q \in C(G)$ of size $|Q| = k$. Let $\alpha = f(Q)$. Then, by Claim~\ref{claim:r<4} it holds that $Q$ is a solution for $I_{\alpha}$. 
				
				\item  There is no clique of size $k$ in $G$. Then, assume towards a contradiction that there is $\alpha \in [n^2]$ such that there is a solution $Q$ for $I_{\alpha}$. By Claim~\ref{claim:r<4} it holds that $Q$ is in particular a clique of size $k$ in $G$ in contradiction. Hence, for all $\alpha \in [n^2]$ there is no solution for $I_{\alpha}$ in this case. 
			\end{enumerate} Thus, by the above, to decide if there is a clique of size $k$ in $G$ we can decide if there is a solution for at least one $I_{\alpha}$ for all $\alpha \in [n^2]$. The reduction takes polynomial time and the weights $w$ are polynomial (in the encoding size of the $k$-clique instance). The proof follows since the $k$-clique problem is known to be strongly NP-Hard.  		\end{proof}
		
		
	}
	
	
	\subsection{Constrained Minimum Basis of a Matroid}
	\label{sec:abs_CMB}
%		\begin{definition}[Constrained Minimum Basis of a Matroid (BM)] 
%		\label{def:CMB}We are given a tuple $U = (E,\cI,\ell,w,L)$, where $(E,\cI)$ is a matroid along with a membership oracle, $c:E \rightarrow \mathbb{N}$ is a cost function, $w:E \rightarrow \mathbb{N}$ is a weight function and $L \in \mathbb{N}$ is a bound. A solution of $U$ is a basis $S\in \cI, |S| = \max_{S' \in \cI} |S'|$ such that $\ell(S) \leq L$. The goal is to find a solution $S$ of $U$ with minimum weight $w(S)$. 
%	\end{definition} 
	
	
	Unlike the reductions used from  BM and EMI,  the reduction from $\Pi$-matroid to CMB uses a  different {\em cost} function. Specifically, for every $n \in \mathbb{N}_{>0}$ define the standard cost function of $n$ as $c_n:[n] \rightarrow \mathbb{N}$ such that for all $i \in [n]$ it holds that \begin{equation}
		\label{leq:w}
		c_n(i) = w_n(i)-2 \cdot i = 2 \cdot \textsf{sum}([n])-i.  
	\end{equation} Moreover, define the standard bound of  $n,k,\alpha \in \mathbb{N}_{>0}$  as \begin{equation}
		\label{leq:B}
		L_{n,k,\alpha} = B_{n,k,\alpha} -2 \cdot \alpha =2 k\cdot \textnormal{\textsf{sum}}([n])- \alpha.   
	\end{equation}
%The above defined cost function is useful for the proof of hardness of CMB. We first use the following auxiliary results.  
	
	
%		\begin{lemma}
%		\label{lemma:wl}
%		For every $n,k,\alpha \in \mathbb{N}_{>0}$, and $S \subseteq [n], |S| = k$ such that $w_n(S) = B_{n,k,\alpha}$, it holds that $c_n(S) \leq L_{n,k,\alpha}$. 
%	\end{lemma}
%	
%	\begin{proof}
%	 By \eqref{eq:w}, \eqref{eq:B}, and that $|S| = k$ we have: \begin{equation}
%		\label{eq:x}
%		2 \cdot \textsf{sum}([n]) \cdot k+\alpha = B_{n,k,\alpha} = w_n(S) = 2 \cdot \textsf{sum}([n]) \cdot k+\textsf{sum}(S).
%	\end{equation} By \eqref{eq:x} we conclude that $\textsf{sum}(S) = \alpha$. Therefore, 
%	
%		$$c_n(S) = 2 \cdot \textsf{sum}([n]) \cdot k-\textsf{sum}(S) = 2 \cdot \textsf{sum}([n]) \cdot k-2\cdot \alpha = L_{n,k,\alpha}.$$
%	\end{proof}

We use the next auxiliary lemma in the proof of \Cref{thm:CMB}. 
	\begin{lemma}
	\label{lemma:wl}
	For every $n,k,\alpha \in \mathbb{N}_{>0}$, and $S \subseteq [n]$ such that  $|S| = k$ it holds that $w_n(S) \geq B_{n,k,\alpha}$ if and only if $c_n(S) \leq L_{n,k,\alpha}$. 
\end{lemma}

\begin{proof}
	If $w_n(S) \geq B_{n,k,\alpha}$, then by \eqref{eq:w}, \eqref{eq:B}, and since $|S| = k$ we have: \begin{equation}
		\label{eq:x}
		2 \cdot \textsf{sum}([n]) \cdot k+\alpha = B_{n,k,\alpha} \leq w_n(S) = 2 \cdot \textsf{sum}([n]) \cdot k+\textsf{sum}(S).
	\end{equation} By \eqref{eq:x} we conclude that $\textsf{sum}(S) \geq \alpha$. Therefore, 
	$$c_n(S) = 2 \cdot \textsf{sum}([n]) \cdot k-\textsf{sum}(S) \leq 2 \cdot \textsf{sum}([n]) \cdot k- \alpha = L_{n,k,\alpha}.$$
	For the second direction, if $c_n(S) \leq L_{n,k,\alpha}$, then by \eqref{leq:w}, \eqref{leq:B}, and since $|S| = k$ it holds that: \begin{equation}
		\label{leq:x}
		2 \cdot \textsf{sum}([n]) \cdot k-\alpha = L_{n,k,\alpha} \geq c_n(S) = 2 \cdot \textsf{sum}([n]) \cdot k-\textsf{sum}(S).
	\end{equation} By \eqref{leq:x} we conclude that $\textsf{sum}(S) \geq \alpha$. Then, 
	$$w_n(S) = 2 \cdot \textsf{sum}([n]) \cdot k+\textsf{sum}(S) \geq 2 \cdot \textsf{sum}([n]) \cdot k+ \alpha = B_{n,k,\alpha}.$$
\end{proof}

%	\begin{lemma}
%		\label{llemma:if}
%		For every $n,k,\alpha \in \mathbb{N}_{>0}, \Pi \subseteq 2^{[n]}$, and $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$, it holds that $c_n(S) = L_{n,k,\alpha}$. 
%	\end{lemma}
%	\begin{proof}
%		Let $S \in \mathcal{L}(\Pi)$. That is, by \eqref{eq:1} it holds that $|S| = k$ and $\textnormal{\textsf{sum}}(S) = \alpha$. %In addition, let $D = \{x_i~|~i \in S\}$. 
%		Then, \begin{equation*}
%			\label{leq:ole}
%			\begin{aligned}
%				c_n(S) = \sum_{i \in S} \left( 2 \cdot \textnormal{\textsf{sum}}([n])-i  \right) = |S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n])-\textnormal{\textsf{sum}}(S) = 2 k\cdot \textnormal{\textsf{sum}}([n])-\alpha = L_{n,k,\alpha}.  
%			\end{aligned}
%		\end{equation*}
%		%	 The last equality holds because $\alpha = \textnormal{\textsf{sum}}(S) \leq \textnormal{\textsf{sum}}([n])$. 
%		%	Since $S \in \mathcal{L}(\Pi)$ it holds that $S \in \cI$. Thus, by \eqref{eq:ole} $S$ is a solution for $U$ of profit exactly $B$. 
%	\end{proof}
	
	
%	Now, for the second direction, given $S \in \cI_{n,k,\alpha}(\Pi)$ such that $c_n(S) = B_{n,k,\alpha}$ we show that $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$.  
%	
%	\begin{lemma}
%		\label{llemma:onlyif}
%		Let $n,k, \in \mathbb{N}_{>0}, \alpha \in \left[ n^2\right], \Pi \subseteq 2^{[n]}$, and $S \in \cI_{n,k,\alpha}(\Pi)$ such that $w_{n}(S) = B_{n,k,\alpha}$. Then, $S \in \mathcal{L}_{n,k,\alpha}(\Pi)$. 
%	\end{lemma}
%	\begin{proof}
%		%Let $F$ be a solution for $U$ of profit at least $B$. Since $c(e) = p(e)$ for every element $e \in E$, then $p(F) = c(F) \leq B$, since $F$ satisfies the budget constraint; thus, since $p(F) \geq B$ we conclude that $p(F) = c(F) = B$. 
%		%For the following, 
%		%	We show that $F$ is also a solution for $I$. 
%		Since $S \in \cI_{n,k,\alpha}(\Pi)$, by \eqref{eq:1}, it is sufficient to show that $|S| = k$ and $\textsf{sum}(S) = \alpha$. First, assume towards a contradiction that $|S| \neq k$. We consider two cases. \begin{enumerate}
%			\item $|S|< k$. Then, \begin{equation}
%				\label{eq:ol3}
%				\begin{aligned}
%					w_{n}(S) ={} & \sum_{i \in S} i+|S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
%					\leq{} & \sum_{i \in S} i+(k-1) \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
%					\leq{} &  \textnormal{\textsf{sum}}([n])+(k-1) \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
%					<{} & 2 k\cdot \textnormal{\textsf{sum}}([n]) \\
%					<{} & B_{n,k,\alpha}.
%				\end{aligned}
%			\end{equation} 
%			
%			The last inequality holds since $\alpha \geq 1$. By \eqref{eq:ol3} we reach a contradiction that $w_{n}(S) = B_{n,k,\alpha}$.%	By the above we reach contradiction that $p(F) = B$. 
%			\item $|S|>k$. Since $S \in \cI_{n,k,\alpha}(\Pi)$, by \eqref{eq:1} it holds that $|S| \leq k$ and we reach a contradiction. 
%			
%			\comment{
%				\begin{equation}
%					\label{eq:ol2}
%					\begin{aligned}
%						w_{n}(S) ={} & \sum_{i \in S} i+|S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\
%						\geq{} & \sum_{i \in S} i+(k+1) \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) \\ 
%						\geq{} & 2  \cdot \textnormal{\textsf{sum}}([n]) +2 k\cdot \textnormal{\textsf{sum}}([n]) \\
%						>{} & B_{n,k,\alpha}.
%					\end{aligned}
%				\end{equation}
%				The last inequality holds since: if $n = 1$ then $\alpha \leq 1 < 2 \cdot \textsf{sum}([n])$; otherwise, $n > 1$ and it follows that $\alpha \leq n^2 < n^2+n = 2 \cdot \textnormal{\textsf{sum}}([n])$. }%By \eqref{eq:ol2} we reach a contradiction since $F$ is a solution for $U$.
%		\end{enumerate}By the above we conclude that $|S| = k$. Therefore, 
%		$$\textnormal{\textsf{sum}}(S) = \sum_{i \in S} i = w_{n}(S) - |S| \cdot 2 \cdot \textnormal{\textsf{sum}}([n]) = w_{n}(S) -  2 k \cdot \textnormal{\textsf{sum}}([n]) = B_{n,k,\alpha} - 2 k \cdot \textnormal{\textsf{sum}}([n]) = \alpha.$$ In conclusion, we have $S \in \cI(\Pi)$, $|S| = k$ and $\textnormal{\textsf{sum}}(S) = \alpha$. Thus, by \eqref{eq:1} it holds that $S \in \mathcal{L}(\Pi)$.
%	\end{proof}

	
%	\begin{lemma}
%	\label{lem:L}
%	For every $n,k,\alpha \in \mathbb{N}_{>0}$, and $S \subseteq [n]$ it holds that $w_n(S)  \leq B_{n,k,\alpha}$ if and only if $c_n(S) \geq L_{n,k,\alpha}$. 
%\end{lemma}

%\begin{proof}
%	Assume that $w_n(S)  \leq B_{n,k,\alpha}$; then, $$c_n(S) = w_n(S) -2 \cdot \textsf{sum}(S) w_n(S) \geq L_{n,k,\alpha}$$
%\end{proof}
%\thmcmb*
	
	\begin{proof}
		Assume towards a contradiction that there is a randomized Fully PTAS $\cA$ for CMB. We use $\cA$ to decide the $\Pi$-matroid problem.  Let $I = \left(n,k,\alpha,\mm\right)$ be a $\Pi$-matroid instance. Consider the following algorithm $\cB$ that decides $I$.
		\begin{enumerate}
			\item Construct the CMB instance $%U_{n,k,\alpha}(\Pi) 
			U= ([n],\cI_{n,k,\alpha}(\Pi),c_n,w_{n},L_{n,k,\alpha})$ along with the membership oracle of $M_{n,k,\alpha}(\Pi)$; note that the elements of $U$ are $[n] = \{1,\ldots, n \}$, the independent sets are the independent sets of the $\Pi$-matroid $\mm$ (i.e., $\cI_{n,k,\alpha}(\Pi)$), the cost is the standard cost function, the weight is the standard weight function $w_n$, and the bound is the standard bound with parameters $n,k,\alpha$. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
			\item Define $\eps = \frac{1}{6 \cdot n^3}$ and compute $\cA$ on $U$ and $\eps$; let $S$ be the returned solution.  
			\item Return that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. 
		\end{enumerate}
		Note that $U$ can be constructed from $I$ in time $\io$ and that $\frac{1}{\eps} = |I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is a (randomized) Fully PTAS. We now show correctness. %For the correctness, %we show that $\cB$ returns that $I$ has a solution if and only if $I$ indeed has a solution. 
		\begin{itemize}
			\item If $\cB$ returns that $I$ has a solution then  $w_n(S) = B_{n,k,\alpha}$; since $S$ is a solution for $U$ it also holds that $S \in \cI_{n,k,\alpha}(\Pi)$. Thus, by \Cref{cor:iff} it holds that $S\in \mathcal{L}_{n,k,\alpha}(\Pi)$, and thus  $I$ has a solution.  
			\item If $I$ has a solution then there is $T \in \mathcal{L}_{n,k,\alpha}(\Pi)$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$, which implies by \Cref{lemma:wl} that $c_n(T) \leq L_{n,k,\alpha}$. Then, since $T$ is a basis of $\mm$ ($T \in \mathcal{L}_{n,k,\alpha}(\Pi)$), it follows that $T$ is a solution for $U$.  Hence, with probability at least $\frac{1}{2}$:  
			\begin{equation}
				\label{eq:sOPTcmb}
				B_{n,k,\alpha} \leq \OPT(U) \leq w_n(S) \leq (1+\eps) \cdot w_n(T) \leq  w_n(T)+\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}+\frac{1}{2}.
			\end{equation} 	The first inequality follows from \Cref{lemma:wl} (note that $U$ has a solution since $T$ is a solution). %for every $S' \subseteq [n], |S'|<k$ it holds that $s$ every solution $S'$ for $U$ is a basis of $\mm$; thus, it follows that $w$ %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
		%	the profit and the cost of each element are the same, and the cost of a solution cannot exceed the budget. 
		The third inequality follows (with probability at least $\frac{1}{2}$) because $S,T$ are solutions for $U$, and $S$ is computed by a randomized Fully PTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPTcmb}, %w.p. at least $\frac{1}{2}$ 
			it holds that $w_n(S) = B_{n,k,\alpha}$ with probability  at least $\frac{1}{2}$. Thus, $\cB$ returns that $I$ has a solution w.p. at least $\frac{1}{2}$.  
		\end{itemize}
		Hence, %by computing $\cA$ on $U$ and getting a solution $S$, 
		we decide correctly $I$ w.p. at least $\frac{1}{2}$. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
		It follows that $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
		a randomized algorithm for the $\Pi$-matroid problem which runs in polynomial time, contradicting \Cref{cor:deter}. 
		
		
		
	\end{proof}
	
	
	\subsection{Knapsack Cover with a Matroid}
	\label{sec:abs_KCM}
	We are left to prove \Cref{thm:kcm}, whose proof is similar to the previous proofs in this section.
%	\thmkcm*
	
	\begin{proof}
		Assume towards a contradiction that there is a randomized Fully PTAS $\cA$ for KCM. We use $\cA$ to decide the $\Pi$-matroid problem.  Let $I = \left(n,k,\alpha,\mm\right)$ be a $\Pi$-matroid instance. Consider the following algorithm $\cB$ that decides $I$.
		\begin{enumerate}
			\item Construct the KCM instance $%U_{n,k,\alpha}(\Pi) 
			U= ([n],\cI_{n,k,\alpha}(\Pi),w_{n},w_{n},B_{n,k,\alpha})$ along with the membership oracle of $M_{n,k,\alpha}(\Pi)$; note that the elements of $U$ are $[n] = \{1,\ldots, n \}$, the independent sets are the independent sets of the $\Pi$-matroid $\mm$ (i.e., $\cI_{n,k,\alpha}(\Pi)$), the standard weight function $w_n$ is both the cost and the size function, and the demand is simply the standard budget with parameters $n,k,\alpha$. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
			\item Define $\eps = \frac{1}{6 \cdot n^3}$ and compute $\cA$ on $U$ and $\eps$; let $S$ be the returned solution.  
			\item Return that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. 
		\end{enumerate}
		
		Note that $U$ can be constructed from $I$ in time $\io$ and that $\frac{1}{\eps} = |I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is a (randomized) Fully PTAS. We now show correctness. %For the correctness, %we show that $\cB$ returns that $I$ has a solution if and only if $I$ indeed has a solution. 
		\begin{itemize}
			\item If $\cB$ returns that $I$ has a solution. Then, $w_n(S) = B_{n,k,\alpha}$; since $S$ is a solution for $U$ it also holds that $S \in \cI_{n,k,\alpha}(\Pi)$. Thus, by \Cref{cor:iff} it holds that $S$ is a solution for  $I$, and in particular $I$ has a solution.
			\item If $I$ has a solution. Then, there is $T \in \mathcal{L}_{n,k,\alpha}(\Pi)$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$ implying that $T$ is a solution for $U$.  Therefore, with probability at least $\frac{1}{2}$: 
			\begin{equation}
				\label{eq:sOPT}
				B_{n,k,\alpha} \leq \OPT(U) \leq w_n(S) \leq (1+\eps) \cdot w_n(T) \leq  w_n(T)+\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}+\frac{1}{2}.
			\end{equation} 	The first inequality holds since %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
			the size and the cost of each element are the same, and the size of a solution must be higher or equal from the demand. The third inequality follows (with probability at least $\frac{1}{2}$) because $S,T$ are solutions for $U$, and $S$ is computed by a randomized FPTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPT}, %w.p. at least $\frac{1}{2}$ 
			it holds that $w_n(S) = B_{n,k,\alpha}$ with probability at least $\frac{1}{2}$. Then, $\cB$ returns that $I$ has a solution with probability at least $\frac{1}{2}$.  
		\end{itemize}
		Hence, %by computing $\cA$ on $U$ and getting a solution $S$, 
		the algorithm correctly decides $I$ with probability at least $\frac{1}{2}$. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
		It follows that $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
		a randomized algorithm for $\Pi$-matroid problem which runs in polynomial time, contradicting  \Cref{cor:deter}.

	\end{proof}
	
	
	
	
	
	
%	\subsection{Knapsack Cover with Matroid Intersection}
	

==> LowerBounds-NP.tex <==

\label{sec:NPhard}
\subsection{Budgeted Matroid Independent Set}

\label{sec:bm_np}


\lemsatbm*

%\begin{proof}
%	We use a reduction from the SAT-matroid problem. Let $I \in \{0,1\}^*$ be a SAT-matroid instance; for simplicity, let $A = A_I, n = n(A), k = k_I$, and $\alpha = \alpha_I$.  
%	%
%	%If $k \notin \mathbb{N}_{>0}$, $\alpha \notin \left[ n^2 \right]$, or $A$ is not a SAT instance with $n$ variables, we can verify it in time $\io$ and decide correctly the SAT-matroid instance $I$ in time $|I|^{O(1)}$. Thus, for the following, assume that $n,k \in \mathbb{N}_{>0}, \alpha \in \left[ n^2 \right]$,  and that $A$ is a SAT instance with $n$ variables. %$I = \left(n,k,\alpha,\mm\right)$ be a $\Pi$-matroid instance. 
%	We define the $\fs$-BM instance $$U = (I,w_{n},w_{n},B_{n,k,\alpha}).$$ Note that $\fs (I) = M_{n,k,\alpha}(\mathcal{S}(A))$ by \Cref{def:SATencoder}. %is an encodable matroid by \Cref{lem:encodable}; 
%	Moreover, by \Cref{lem:encodable}, \eqref{eq:w}, and \eqref{eq:B} it follows that $U$ can be constructed from $I$ in time $|I|^{O(1)}$.   
%	%
%	%For all $S \subseteq [n]$ it holds that $w_{n}(S) \in \mathbb{N}$ and that $$\OPT \left( U\right) \leq n \cdot \max_{i \in [n]} p(i) = n^2 = \left| U \right|^{O(1)}.$$  
%	%
%	To show that $U$ is a scaled $\fs$-BM instance, observe that for all $S \subseteq [n]$ it holds that $w_{n}(S) \in \mathbb{N}$ and that $\OPT \left( U\right) = \left| U \right|^{O(1)}$ by \Cref{lem:OPTu}. Therefore, if $\fs$-BM has an FPTAS, by \Cref{lem:FPTAStoEXACT} there is an exact algorithm $\cA$ that finds in time $\left| U \right|^{O(1)} = \io$ an optimal solution for $U$. Clearly, $\OPT(U) \leq B_{n,k,\alpha}$ since the profit and the cost of each element are the same. Therefore, by \Cref{cor:iff} the algorithm $\cA$ on instance $U$ returns a solution for $U$ with profit $B_{n,k,\alpha}$ if and only if $I$ has a solution. %Hence, we can decide $I$ by computing $\cA$ on $U$ and return that $I$ has a solution if and only if $\cA$ returns that $U$ has a solution for $U$ with profit $B_{n,k,\alpha}$Thus, $\cA$ is a polynomial algorithm that decides the SAT-matroid problem, 
%	Hence, by computing $\cA$ on $U$ and getting a solution $S$, we can decide correctly $I$ by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. The above algorithm decides the SAT-matroid problem, which is impossible by \Cref{cor:Strong}, unless P=NP. 
%\end{proof}



\begin{proof}
	
	
	
	%	\noindent{\bf Proof of \Cref{lem:hard}:}
	Assume that P$\neq$NP and assume towards a contradiction that there is a Fully PTAS $\cA$ for $\fs$-BM. We use $\cA$ to decide the $\Pi$-matroid problem.  Let $I \in \{0,1\}^*$ be a SAT-matroid instance. Consider the following algorithm $\cB$ that decides $I$. For simplicity, let $A = A_I, n = n(A), k = k_I$, and $\alpha = \alpha_I$.  %let $n = n_I,k = k_I,\alpha = \alpha_I$, and $A = A_I$. 
	\begin{enumerate}
		\item Construct the $f_{\textnormal{SAT}}$-BM instance $%U_{n,k,\alpha}(\Pi) 
		U= (I,w_{n},w_{n},B_{n,k,\alpha})$. Note that $\fs (I) = M_{n,k,\alpha}(\mathcal{S}(A))$ by \Cref{def:SATencoder}. %is an encodable matroid by \Cref{lem:encodable}; 
		
		
		%; note that the elements of $U$ are $[n] = \{1,\ldots, n \}$, the independent sets are the independent sets of the $\Pi$-matroid $\mm$ (i.e., $\cI_{n,k,\alpha}(\Pi)$), the standard weight function $w_n$ is both the profit and the cost function, and the budget is simply the standard budget with parameters $n,k,\alpha$. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
		\item Define $\eps = \frac{1}{6 \cdot n^3}$ and compute $\cA$ on $U$ and $\eps$; let $S$ be the returned solution.  
		\item Return that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. 
	\end{enumerate}
	
By \Cref{lem:encodable}, \eqref{eq:w}, and \eqref{eq:B} it follows that $U$ can be constructed from $I$ in time $|I|^{O(1)}$.   In addition, %Note that $U$ can be constructed from $I$ in time $\io$ and that 
$\frac{1}{\eps} = n^{O(1)} =|I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is an FPTAS. We now show correctness. %For the correctness, %we show that $\cB$ returns that $I$ has a solution if and only if $I$ indeed has a solution. 
	\begin{itemize}
		\item If $\cB$ returns that $I$ has a solution then $w_n(S) = B_{n,k,\alpha}$; since $S$ is a solution for $U$ it also holds that $S \in \cI_{\fs (I)} = \cI_{n,k,\alpha}(\mathcal{S}(A))$. Thus, by \Cref{cor:iff} it holds that $I$ has a solution.  
		\item If $I$ has a solution then there is $T \in \mathcal{L}_{n,k,\alpha}(\mathcal{S}(A))$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$ implying that $T$ is a solution for $U$.  Therefore, %w.p. at least $\frac{1}{2}$: 
		\begin{equation}
			\label{eq:sOPT}
			B_{n,k,\alpha} \geq \OPT(U) \geq w_n(S) \geq (1-\eps) \cdot w_n(T) \geq  w_n(T)-\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}-\frac{1}{2}.
		\end{equation} 	The first inequality holds since %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
		the profit and the cost of each element are the same, and the cost of a solution cannot exceed the budget. The third inequality follows because $S,T$ are solutions for $U$, and $S$ is computed by an FPTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPT}, %w.p. at least $\frac{1}{2}$ 
		it holds that $w_n(S) = B_{n,k,\alpha}$. Then, $\cB$ returns that $I$ has a solution.  
	\end{itemize}
%	Hence, %by computing $\cA$ on $U$ and getting a solution $S$, 
%	the algorithm $\cB$ is an solves the SAT matroid problem correctly. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
Hence $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
	a polynomial time algorithm for the  SAT-matroid problem, contradicting \Cref{cor:Strong}. 
\end{proof}



\subsection{Exact Weight Matroid Independent Set}

Similarly to $f$-BM, we can define a variant of EMI for every matroid encoder $f$.

	\problem{ {\sc $f$-Exact Matroid Independent Set} ($f$-EMI)}{
	{\bf Encoder} & $f:\{0,1\}^* \rightarrow 2^{\mathbb{N}} \times 2^{2^{\mathbb{N}}}$ is a matroid encoder. \\
	{\bf Instance} &  $U =  (I,w,k,T)$, where $I \in \{0,1\}^*$, $w:E_{f(I)} \rightarrow \mathbb{N}$ gives the elements weights, $k\in \mathbb{N}$ is  the target cardinality, and $T \in \mathbb{N}$ is the target weight. \\
	{\bf Solution }& $S\in \cI_{f(I)}$ such that $|S|=k$ and $w(S)=T$.\\
{\bf Objective} & Decide if there exists a solution.
}



\begin{lemma}
	\label{lem:f-EMI}
	Unless \textnormal{W[1]=FPT}, for any computable function $f:\mathbb{N} \rightarrow \mathbb{N}$ there is no algorithm that decides \textnormal{EMI} in time $f(k) \cdot \left( T\cdot |I|\right)^{O(1)}$, where $|I|$ is the encoding size of the instance, $k$ is the target cardinality and $T$ is the target weight.
\end{lemma}
\begin{proof}
	Assume that \textnormal{W[1]}$\neq$\textnormal{FPT}. 
	Assume towards a contradiction that the statement of the lemma does not hold. Thus, there is a computable  function $f:\mathbb{N} \rightarrow \mathbb{N}$, and an algorithm $\cA$ that decides $\fs$-\textnormal{EMI} in time $f(k) \cdot {(T \cdot |I|)}^{O(1)}$. We use $\cA$ to decide the SAT-matroid problem. 
Let $I \in \{0,1\}^*$ be a SAT-matroid instance. Consider the following algorithm $\cB$ that decides $I$. For simplicity, let $A = A_I, n = n(A), k = k_I$, and $\alpha = \alpha_I$. Assume that $k \leq n$ or the instance can be trivially decided. 
	\begin{enumerate}
		\item Construct the $\fs$-EMI instance $%U_{n,k,\alpha}(\Pi) 
		U= (I,w_{n},k,B_{n,k,\alpha})$. Note that $\fs (I) = M_{n,k,\alpha}(\mathcal{S}(A))$ by \Cref{def:SATencoder}. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
		\item %Define $\eps = \frac{1}{6 \cdot n^3}$ and 
		Compute $\cA$ on $U$. %and let $S$ be the returned solution.  
		\item Return that $I$ has a solution if and only if $\cA$ returns that $U$ has a solution.   %$w_n(S) = B_{n,k,\alpha}$. 
	\end{enumerate}
	To show $\cB$ indeed solves the SAT-matroid instance, consider the following cases. 
	\begin{itemize}
		\item If  $\cB$ returns that $I$ has a solution then $w_n(S) = B_{n,k,\alpha}$ and $S \in \cI_{\fs (I)} = \cI_{n,k,\alpha}(\mathcal{S}(A))$. Thus, by \Cref{cor:iff} it holds that $I$ has a solution.  
		\item If $I$ has a solution then there is $T \in \mathcal{L}_{n,k,\alpha}(\mathcal{S}(A))$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$. Also, by the definition of $\mathcal{L}_{n,k,\alpha}(\mathcal{S}(A))$ it holds that $|T|=k$.  Therefore $T$ is a solution of $U$. Therefore, $\cA$ returns that $U$ has a solution; thus, $\cB$ returns that $I$ has a solution. 
	\end{itemize}
It follows that $\cB$ is an algorithm for the SAT-matroid problem.

%	Note that $U$ can be constructed naively from $I$ in time $n+n \cdot (2n^2+n)+2n \cdot k+n^2 \leq 6 \cdot n^3$ (recall that the weights are encoded in unary and that $k \leq n$); thus, the running time of $\cB$ on $I$ is bounded by $6 \cdot n^3+f(k) \cdot n^{q} = f(k) \cdot n^{O(1)}$. 
	Note that $B_{n,k,\alpha} = 2k \cdot \textsf{sum}(n) \leq 2k \cdot n^2 \leq 2 \cdot n^3$ since $k \leq n$.  The instance $U$ can be trivially constructed in time $|I|^{O(1)}$, thus the overall running time of $\cB$ is $f(k)\cdot (2\cdot n^3\cdot |I|^{O(1)})^{O(1)} \leq f(k)\cdot |I|^{O(1)}$. That is, $\cB$ is a parameterized algorithm for the SAT-matroid problem, in contradiction to \Cref{lem:FPT}. Thus, the statement of the lemma holds.
\end{proof}

























\subsection{Constrained minimum Basis of a Matroid}

We proceed to define a variant of CMB in which the matroid is encoded as part of the instance.
\problem{ {\sc $f$-Constrained minimum Basis of a Matroid} ($f$-CMB)}{
	{\bf Encoder} & $f:\{0,1\}^* \rightarrow 2^{\mathbb{N}} \times 2^{2^{\mathbb{N}}}$ is a matroid encoder. \\
	{\bf Instance} &  
	$U = (I,c,w,B)$, where $I \in \{0,1\}^*$,  $c:E_{f(I)} \rightarrow \mathbb{N}$ is a cost function, $w:E_{f(I)} \rightarrow \mathbb{N}$ is a weight function and $B \in \mathbb{N}$ is a budget.\\
	{\bf Solution}& A basis $S \in \cI_{f(I)}, |S| = \max_{S' \in \cI_{f(I)}} |S'|$ such that $c(S) \leq B$.\\
	{\bf Objective} & Find a solution $S$ of $U$ with minimum weight $w(S)$.
	%	{\bf Model } &The independent sets $\cI$ is only accessible via a membership oracle; the encoding cost of the instance $U$ is the encoding cost of $(E,c,p,B)$, the instance without $\cI$.
}

\begin{lemma}
	\label{lem:CMB-NP}
	Unless \textnormal{P=NP}, there is no \textnormal{Fully PTAS} for $f_{\textnormal{SAT}}$-\textnormal{CMB}. 
	%If there is an algorithm for \textnormal{BM} in $X(n)$   
\end{lemma}
	\begin{proof}
		Assume that P$\neq$NP and assume towards a contradiction that there is a Fully PTAS $\cA$ for $f_{\textnormal{SAT}}$-CMB. We use $\cA$ to decide the SAT-matroid problem.  Let $I \in \{0,1\}^*$ be a SAT-matroid instance. Consider the following algorithm $\cB$ that decides $I$. For simplicity, let $A = A_I, n = n(A), k = k_I$, and $\alpha = \alpha_I$. 
	\begin{enumerate}
		\item Construct the $f_{\textnormal{SAT}}$-CMB instance $%U_{n,k,\alpha}(\Pi) 
		U= (I,c_n,w_{n},L_{n,k,\alpha})$. Note that $\fs (I) = M_{n,k,\alpha}(\mathcal{S}(A))$ by \Cref{def:SATencoder}.  %along with the membership oracle of $M_{n,k,\alpha}(\Pi)$; note that the elements of $U$ are $[n] = \{1,\ldots, n \}$, the independent sets are the independent sets of the $\Pi$-matroid $\mm$ (i.e., $\cI_{n,k,\alpha}(\Pi)$), the cost is the standard cost function, the weight is the standard weight function $w_n$, and the bound is the standard bound with parameters $n,k,\alpha$. %Let $U = U_{n,k,\alpha}(\Pi)$ for simplicity.
		\item Define $\eps = \frac{1}{6 \cdot n^3}$ and compute $\cA$ on $U$ and $\eps$; let $S$ be the returned solution.  
		\item Return that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. 
	\end{enumerate}
By \Cref{lem:encodable}, \eqref{eq:w}, and \eqref{eq:B} it follows that $U$ can be constructed from $I$ in time $|I|^{O(1)}$.   In addition, %Note that $U$ can be constructed from $I$ in time $\io$ and that 
$\frac{1}{\eps} =n^{O(1)} = |I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is an FPTAS. We now show correctness.
	%Note that $U$ can be constructed from $I$ in time $\io$ and that $\frac{1}{\eps} = |I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is a (randomized) FPTAS. We now show correctness. %For the correctness, %we show that $\cB$ returns that $I$ has a solution if and only if $I$ indeed has a solution. 
	\begin{itemize}
		\item If $\cB$ returns that $I$ has a solution. Then, $w_n(S) = B_{n,k,\alpha}$; since $S$ is a solution for $U$ it also holds that $S \in \cI_{\fs (I)} = \cI_{n,k,\alpha}(\mathcal{S}(A))$. Thus, by \Cref{cor:iff} it holds that $I$ has a solution.  
		\item If $I$ has a solution. Then, there is $T \in \mathcal{L}_{n,k,\alpha}(\mathcal{S}(A))$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$, which implies by \Cref{lemma:wl} that $c_n(T) \leq L_{n,k,\alpha}$. Then, since $T$ is a basis of $\mm$ (recall that $T \in \mathcal{L}_{n,k,\alpha}(\mathcal{S}(A))$), it follows that $T$ is a solution for $U$.  Hence,   
		\begin{equation}
			\label{eq:sOPTcmb}
			B_{n,k,\alpha} \leq \OPT(U) \leq w_n(S) \leq (1+\eps) \cdot w_n(T) \leq  w_n(T)+\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}+\frac{1}{2}.
		\end{equation} 	The first inequality follows from \Cref{lemma:wl} (note that $U$ has a solution since $T$ is a solution). %for every $S' \subseteq [n], |S'|<k$ it holds that $s$ every solution $S'$ for $U$ is a basis of $\mm$; thus, it follows that $w$ %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
		%	the profit and the cost of each element are the same, and the cost of a solution cannot exceed the budget. 
		The third inequality follows because $S,T$ are solutions for $U$, and $S$ is computed by an FPTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPTcmb}, %w.p. at least $\frac{1}{2}$ 
		it holds that $w_n(S) = B_{n,k,\alpha}$. Then, $\cB$ returns that $I$ has a solution.  
	\end{itemize}
	Hence, %by computing $\cA$ on $U$ and getting a solution $S$, 
	we decide $I$ correctly. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
	It follows that $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
	a polynomial algorithm which decides the SAT-matroid problem, contradicting \Cref{cor:Strong}. 
\end{proof}























	\subsection{Knapsack Cover with a Matroid}

Finally, we define a variant of KCM with no oracle.

\problem{ {\sc $f$-Knapsack Cover with a Matroid} ($f$-KCM)}{
	{\bf Encoder} & $f:\{0,1\}^* \rightarrow 2^{\mathbb{N}} \times 2^{2^{\mathbb{N}}}$ is a matroid encoder. \\
	{\bf Instance} &  
	$U = (I,c,d,D)$, where $I \in \{0,1\}^*$,  $c:E_{f(I)} \rightarrow \mathbb{N}$ is a cost function, $d:E_{f(I)} \rightarrow \mathbb{N}$ is a size function, and $B \in \mathbb{N}$ is a demand.\\
	{\bf Solution}& $S \in \cI_{f(I)}$ such that $d(S) \geq D$.\\
	{\bf Objective} & Find a solution $S$ of $U$ with minimum cost $c(S)$.
	%	{\bf Model } &The independent sets $\cI$ is only accessible via a membership oracle; the encoding cost of the instance $U$ is the encoding cost of $(E,c,p,B)$, the instance without $\cI$.
}

\begin{lemma}
	\label{lem:KCM-NP}
	Unless \textnormal{P=NP}, there is no \textnormal{Fully PTAS} for $f_{\textnormal{SAT}}$-\textnormal{KCM}. 
	%If there is an algorithm for \textnormal{BM} in $X(n)$   
\end{lemma}

\begin{proof}
	Assume that P$\neq$NP and assume towards a contradiction that there is an FPTAS $\cA$ for $f_{\textnormal{SAT}}$-KCM. We use $\cA$ to decide the SAT-matroid problem. Let $I \in \{0,1\}^*$ be a SAT-matroid instance. Consider the following algorithm $\cB$ that decides $I$. For simplicity, let $A = A_I, n = n(A), k = k_I$, and $\alpha = \alpha_I$. 
	\begin{enumerate}
		\item Construct the $f_{\textnormal{SAT}}$-KCM instance $%U_{n,k,\alpha}(\Pi) 
	U= (I,w_n,w_{n},B_{n,k,\alpha})$. Note that $\fs(I) = M_{n,k,\alpha}(\mathcal{S}(A))$ by \Cref{def:SATencoder}. 
		\item Define $\eps = \frac{1}{6 \cdot n^3}$ and compute $\cA$ on $U$ and $\eps$; let $S$ be the returned solution.  
		\item Return that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. 
	\end{enumerate}
By \Cref{lem:encodable}, \eqref{eq:w}, and \eqref{eq:B} it follows that $U$ can be constructed from $I$ in time $|I|^{O(1)}$.   In addition, %Note that $U$ can be constructed from $I$ in time $\io$ and that 
$\frac{1}{\eps} =n^{O(1)} =  |I|^{O(1)}$; thus, the running time of $\cB$ on $I$ is $|I|^{O(1)}$, since $\cA$ is an FPTAS. We now show correctness.
	\begin{itemize}
		\item If $\cB$ returns that $I$ has a solution. Then, $w_n(S) = B_{n,k,\alpha}$; since $S$ is a solution for $U$ it also holds that $S \in \cI_{\fs (I)} =  \cI_{n,k,\alpha}(\mathcal{S}(A))$. Thus, by \Cref{cor:iff} it holds that $I$ has a solution.  
		\item If $I$ has a solution. Then, there is $T \in \mathcal{L}_{n,k,\alpha}(\mathcal{S}(A))$; thus, by  \Cref{cor:iff} it follows that $w_n(T) = B_{n,k,\alpha}$ implying that $T$ is a solution for $U$.  Therefore, 
		\begin{equation}
			\label{eq:sOPT}
			B_{n,k,\alpha} \leq \OPT(U) \leq w_n(S) \leq (1+\eps) \cdot w_n(T) \leq  w_n(T)+\frac{1}{6 \cdot n^3} \cdot 3 \cdot n^3 = B_{n,k,\alpha}+\frac{1}{2}.
		\end{equation} 	The first inequality holds since %$w_n(T) = B_{n,k,\alpha}$. In addition, $\OPT(U) \leq B_{n,k,\alpha}$ because 
		the size and the cost of each element are the same, and the size of a solution must be higher or equal from the demand. The third inequality follows because $S,T$ are solutions for $U$, and $S$ is computed by an FPTAS with the parameter $\eps$. The fourth inequality follows from \Cref{lem:OPTu} and by the selection of $\eps$. Observe that the value of $S$ is an integer by \eqref{eq:w}; thus, by \eqref{eq:sOPT}, %w.p. at least $\frac{1}{2}$ 
		it holds that $w_n(S) = B_{n,k,\alpha}$. Then, $\cB$ returns that $I$ has a solution.  
	\end{itemize}
	Hence, %by computing $\cA$ on $U$ and getting a solution $S$, 
	we decide $I$ correctly. %if and only if $w_n(S) = \OPT(U)$, which holds w.p. at least $\frac{1}{2}$. 
	It follows that $\cB$ is %by returning that $I$ has a solution if and only if $w_n(S) = B_{n,k,\alpha}$. Thus, we 
	a polynomial algorithm which decides the SAT-matroid problem, contradicting \Cref{cor:Strong}. 
\end{proof}

















==> algorithm.tex <==



	%Formally, 

\section{An EPTAS for Knapsack Cover with Matroid}



In this section we present an EPTAS for KCM. Generally, our approximation scheme defines an additional {\em partition matroid} constraint that bounds the number of items allowed for the solution from each {\em cost class} - items of almost similar costs, defined by rounding over the costs. Then, we find an optimal solution to the induced matroid intersection instance via {\em Lagrangian relaxation} and refined exchange properties of matroids.
 
An important part of our algorithm requires that we take a {\em basis} of a matroid, rather than an independent set. Thus, in the following we show that this does not make the problem any harder. A {\em KCM basis (KCMB)} instance $I = (E,\cI,c,d,D)$ is a KCM instance. A {\em solution} for $I$ (as a KCMB instance) is a basis $S \in \cI, |S| = \max_{S' \in \cI} |S'|$ such that $d(S) \geq D$. The goal is to find a solution $S$ for $I$ with minimum cost $c(S)$. %that is also solution for $I$ being a KCM instance. 

\begin{lemma}
	\label{lem:b}
%	For any $\rho \geq 1$, there is a $\rho$-approximation for \textnormal{KCMB} if and only if there is a $\rho$-approximation for \textnormal{KCM}. Moreover, there is an \textnormal{EPTAS} for \textnormal{KCM} if and only if there is an \textnormal{EPTAS} for \textnormal{KCMB}.
If there is an \textnormal{EPTAS} for \textnormal{KCMB} then there is an \textnormal{EPTAS} for \textnormal{KCM}.
\end{lemma}

\begin{proof}
	Let $I =  (E,\cI,c,d,D)$ be a KCM instance and let $\eps>$ be an error parameter. %Assume that the optimal solution of $I$ contains at least one element, or the problem is trivial. 
	In addition, let $k = \max_{S' \in \cI} |S'|$ be the cardinality of a basis of the matroid $(E,\cI)$ ($k$ is known as the {\em rank} of the matroid). Finally, let $\cA$ be an EPTAS for KCMB. For every $\alpha \in [k]$ define a KCMB instance $I_{\alpha} = (E,\cI_{\leq \alpha},c,d,D)$ such that $$\cI_{\leq \alpha} = \{S \in \cI~|~|S| \leq \alpha\}.$$ 
	Note that a solution for $I_{\alpha}$ contains exactly $\alpha$ elements since it is a basis of the matroid $(E,\cI_{\leq \alpha})$. Moreover, if $S \in \cI$ is a solution for the KCM instance $I$ it is also a solution for the KCMB instance $I_{\alpha}$, where $\alpha = |S|$. 
	On the other hand, for some $\alpha \in [k]$, if $S_{\alpha} \in \cI$ is a solution for $I_{\alpha}$ it is clearly also a solution for $I$ because $\cI_{\leq \alpha} \subseteq \cI$.  
	
	By the above, to obtain an EPTAS for KCM, we compute $\cA$ on each instance $I_{\alpha}$ for all $\alpha \in [k]$ with the error parameter $\eps$. We return the feasible solution for $I$ found through all iterations which has the minimum cost. Let $\alpha \in [k]$ such that there is a solution $S$ of $I$ that satisfies $c(S) = \OPT(I)$; there is such $\alpha$ since $I$ has a solution. Then for this value of $\alpha$, the EPTAS $\cA$ must return a solution $S_{\alpha}$ for $I_{\alpha}$ such that $c(S_{\alpha}) \leq (1+\eps) \cdot \OPT(I_{\alpha}) = (1+\eps) \cdot \OPT(I)$; we conclude that the constructed algorithm returns a $(1+\eps)$-approximate solution. Since $\cA$ is an EPTAS, there is a function $f:\mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ such that the running time of $\cA$ is bounded by $f(\frac{1}{\eps}) \cdot \io$; since we perform $k = \io$ iterations of $\cA$, the running time of the constructed algorithm is bounded by $f(\frac{1}{\eps}) \cdot \io$. Hence, we obtain an EPTAS for KCM. 
\end{proof}







By Lemma~\ref{lem:b} we first find an EPTAS for KCMB. %For the explanations and definitions in this section, consider a KCMB instance $I =  (E,\cI,c,d,D)$ and an error parameter $\eps>0$. 
We first need a constant factor approximation of the optimum cost for KCMB. %$\OPT(I)$; 
For this goal, we convert a PTAS for KCM to a PTAS for KCMB. \begin{lemma}
	\label{lem:B}
	There is an algorithm \textnormal{PTAS-KCMB} that is a \textnormal{PTAS} for \textnormal{KCMB}.
\end{lemma}

\begin{proof}
	let $\cA$ be a PTAS for KCM; such a PTAS exists by \cite{chakaravarthy2013knapsack}. Let $I =  (E,\cI,c,d,D)$ be a KCMB instance and let $\eps>$ be an error parameter. %Assume that $I$ has an optimal solution and that the optimal solution contains at least one element, or the problem is trivial. 
	Let $k = \max_{S' \in \cI} |S'|$ be the rank of the matroid $(E,\cI)$. Define a KCM instance $I' = (E,\cI,c,d',D')$ such that the following holds. \begin{enumerate}
		\item For all $e \in E$ define $d'(e) = d(e)+2 \cdot d(E)$.
		\item $D' = D+k \cdot 2 \cdot d(E)$. 
		%\item $\cI_{\leq \alpha} = \{S \in \cI~|~|S| \leq \alpha\}$. 
	\end{enumerate} Observe that a solution for $I'$ must contain exactly $k$ elements to cover the demand $D'$ and to be independent in the matroid $(E,\cI)$. Thus, $S \subseteq E$ is a solution for (the KCMB instance) $I$ if and only if it is a solution for (the KCM instance) $I'$ due to the new sizes and demand. 
	%
	By the above, we define algorithm PTAS-KCMB by returning the solution that $\cA$ computes for $I'$ and $\eps$. This results in a PTAS for KCMB.
	%
	%construct the KCM instance $I'$, and compute a $\rho$-approximation for KCM on $I$, which yields a $\rho$-approximation for KCMB as well.
\end{proof}

For our algorithm, we partition the element set of the given instance into {\em cost classes}. %Let $n_I = |E|$ be the number of elements in a KCMB instance $I$. Moreover, 
Let $I =  (E,\cI,c,d,D)$ be a KCMB instance and let $S'$ be a solution for $I$ obtained by using the PTAS PTAS-KCMB for KCMB with the error parameter $\eps'  = 2$ %There is a PTAS for KCMB using the PTAS for KCM \cite{chakaravarthy2013knapsack} and 
described in Lemma~\ref{lem:B}; we set $C_{I,\eps} = c(S')$. Note  that %Note that a PTAS for KCM is also a PTAS for KCMB by Lemma~\ref{lem:b}. 
$\OPT(I) \leq C_{I,\eps} \leq 2 \cdot \OPT(I)$.  For some $\eps>0$, define the $0$-th {\em cost class} of $I$ and $\eps$ as the set of elements with relatively small cost $E_0(I,\eps) = \{e \in E~|~ c(e) < \eps \cdot C_{I,\eps}\}$. Second, let $k_{\eps} = \ceil{\frac{1-\eps}{\eps^2}}$. For all $i \in [k_{\eps}]$ define the $i$-th cost class of $I$ and $\eps$ as \begin{equation}
	\label{eq:class}
	E_i(I,\eps) = \big\{e \in E~|~ \left(\eps+(i-1) \cdot \eps^2\right) \cdot C_{I,\eps} \leq c(e) < (\eps+i \cdot \eps^2) \cdot C_{I,\eps} \big\}. 
\end{equation} let $k = k_{\eps}$ and $E_i = E_i(I,\eps) \forall i \in \{0,1,\ldots,k\}$ when clear from the context. Observe that the difference in cost of any two elements from the same cost class is at most $2\eps^{2} \cdot C_{I,\eps}$ which will be used in the analysis. Our algorithm enumerates over all possibilities to the number of elements chosen for the algorithm from each cost class; we describe each option as a vector. Given a KCMB instance $I =  (E,\cI,c,d,D)$, let $n_I = |E|$ be the number of elements in $I$. Then, given $I$ and $\eps>0$, a {\em pattern vectors} of $I$ and $\eps$ is a vector $(n_0, \ldots, n_k) \in \mathbb{N}^{k+1}$ satisfying the following conditions. \begin{enumerate}
	\item $\sum^{k}_{i = 1} n_i \leq \frac{1}{\eps}$.
	\item $\sum^{k}_{i = 0} n_i \leq n_I$.   
\end{enumerate}	\begin{lemma}
	\label{lem:countK}
	For every \textnormal{KCMB} instance $I$ and $\eps>0$ there are $O\left( (k_{\eps}+1)^{\frac{1}{\eps}} \cdot n_I\right)$ pattern vectors of $I$ and $\eps$. 
\end{lemma}

\begin{proof}
	The number of patterns vectors can be bounded by the number of assignments of $0 \leq x \leq \frac{1}{\eps}$ identical balls into $k_{\eps}$ buckets (over all such  value for $x$), and independently choosing a value for $n_0$ in $\{0,1,\ldots,n_I\}$. Thus, the number of options is bounded by $ (k_{\eps}+1)^{\frac{1}{\eps}} \cdot n_I$.  
\end{proof} 

Wee seek pattern vectors that, informally, describe how many elements the optimum takes from each cost class. More concretely, \begin{definition}
	\label{def:good}
 Let $I =  (E,\cI,c,d,D)$ be a KCMB instance and let $\eps>0$. A pattern vector $(n_0, \ldots, n_k)$ of $I$ and $\eps$ is a {\bf good pattern vector} of $I$ and $\eps$ if there is solution $\OPT$ of $I$ that has an optimal cost $c(\OPT) = \OPT(I)$, such that for all $i \in \{0,1,\ldots,k\}$ it holds that $|\OPT \cap E_i(I,\eps)| = n_i$.	
\end{definition} 
%A pattern vector $(n_0, \ldots, n_k)$ of $I$ and $\eps$ is a {\em good pattern vector} of $I$ and $\eps$ if there is an optimal solution $\OPT$ of $I$ such that for all $i \in \{0,1,\ldots,k\}$ it holds that $|\OPT \cap E_i| = n_i$. %, where $\OPT$ is some fixed optimal solution for $I$. 
By Lemma~\ref{lem:countK} we can enumerate over all pattern vectors in time suitable for an EPTAS; one of them is guaranteed to be a good pattern vector.  %Thus, for the simplicity of the presentation, let $P = (n_0, \ldots, n_k)$  be a fixed good pattern vector, which is determined by enumeration in our scheme. 
%For the following, fix a pattern vector $(n_0, \ldots, n_k)$. 
We use a good pattern vector to define the number of elements allowed for the solution from every cost class. This is modeled by the bounds of a partition matroid.  %, used to bound the number of elements selected from each cost class as in the optimum $\OPT$. 
Formally,

\begin{definition}
	\label{def:partitionMatroid}
	  Let $I =  (E,\cI,c,d,D)$ be a KCMB instance, let $\eps>0$, and let $P = (n_0, \ldots, n_k)$ be a pattern vector of $I$ and $\eps$. Define $(E,\cj_{I,\eps}(P))$ as the partition matroid of $I,\eps,P$ such that \begin{equation}
		\label{eq:J}
		\cj_{I,\eps}(P) = \{S \subseteq E~|~\forall i \in \{0,1,\ldots,k\}:~|S \cap E_i| \leq n_i\}. 
	\end{equation} Let $b = \max_{S \in \cI} |S|$ be the rank of $(E,\cI)$ and let $\cG_{I,\eps}(P) = \{S \in \cI \cap \cj_{I,\eps}(P)~|~|S| = b\}$ be all common bases of $\cI$ and $\cj$. 
\end{definition}

%$\sum^{k}_{i = 1} n_i \leq \frac{1}{\eps}$ which. 





%We assume, w.l.o.g, that for all solutions $S,S'$ of $I$ it holds that $|S| = |S'|$; we can indeed make such an assumption if we alter the size function and the demand of $I$ such that a feasible solution for $I$ must be a basis of $(E,\cI)$; 
The above definition of the set of common bases of the given matroid of an instance $I$ with the constructed partition matroid describes a set that we seek a member of this set with minimum {\em lagrangian weight}, that is a function of the cost and size of the given instance. Specifically, our algorithm relies on the following {\em Lagrangian relaxation} of a KCMB instance $I = (E,\cI,c,d,D)$, $\eps>0$, a pattern vector $P$ of $I$ and a parameter $\lambda' \geq 0$: \begin{equation}
	\label{eq:LR}
	LR_{I,\eps,P}(\lambda') = \min_{S \in \cG_{I,\eps}(P)} c(S)+\lambda' \cdot (D-d(S)). 
\end{equation} Clearly, for any $\lambda' \geq 0$ it holds that $LR_{I,\eps,P}(\lambda') \leq \OPT(I)$, and we consider $\lambda$ that gives the tightest such lower bound: \begin{equation}
	\label{eq:Lambda}
	\lambda_{I,\eps,P} = \argmax_{\lambda' \geq 0} LR_{I,\eps,P}(\lambda').
\end{equation} Observe that for every $\lambda' \geq 0 $ we can compute $LR_{I,\eps,P}(\lambda')$ in time $\io$ since it is an instance of matroid intersection basis maximization, known to be polynomially solvable (see, e.g., \cite{schrijver2003combinatorial}). Therefore, $LR_{I,\eps,P}(\lambda')$ (as a function of $\lambda'$) is a minimum of a set of linear functions (e.g., one for
every $S \in \cG_{I,\eps}(P)$); thus, $LR_{I,\eps,P}(\lambda')$ is a concave and piecewise linear function (see, e.g., Fact 1.1 in \cite{gusfield1983parametric}). Therefore, we can compute $\lambda$ in time $\io$ (see \cite{hassin2004efficient} for a more detailed explanation). 

For the following consider again a KCMB instance $I = (E,\cI,c,d,D)$, $\eps>0$, and a pattern vector $P$ of $I$; for simplicity, let $\lambda = 	\lambda_{I,\eps,P} $. Define the cost function of $\lambda$ as $c_{\lambda} : E \rightarrow \mathbb{R}_{\geq 0}$ such that $c_{\lambda}(e) = c(e)-\lambda \cdot d(e)$ for every $e \in E$. In addition, let $$\co_{I,\eps}(P) = \{S \in\cG_{I,\eps}(P)~|~\forall S' \in \cG_{I,\eps}(P) : c_{\lambda}(S) \leq c_{\lambda}(S')\}$$ be all optimal solutions to the Lagrangian relaxation w.r.t. $I,\eps,P$. %the optimal parameter $\lambda$ (and the good vector pattern $P$). 
The next result generalizes the results of \cite{hassin2004efficient,frederickson1989algorithms,ravi1996constrained} to a general matroid and a partition matroid. The proof  follows from Lemma~3 in \cite{hassin2004efficient}, relaying on the properties of the intersection of a general matroid with a partition matroid provided by \cite{brezovec1988matroid}.\footnote{The proof of Lemma~3 in \cite{hassin2004efficient} is stated for graphic matroids along with a partition matroid; however, the proof does not rely on any property of a specific matroid and applies to general matroids.}
% Let $I =  (E,\cI,c,d,D)$ be a KCMB instance, let $\eps>0$, and let $P = (n_0, \ldots, n_k)$ be a pattern vector of $I$ and $\eps$. 
%\begin{lemma}
%	\label{lem:chain}
%	There is a polynomial time algorithm that given $S,S' \in \co$ finds a sequence $S = S_0, S_1, \ldots, S_{\ell} = S' \in \co$, $\ell \in [n]$, such that for all $i \in \{0,1,\ldots,k\}$ and $j \in \{0,1,\ldots,\ell-1\}$ it holds that \begin{equation*}
%		\label{eq:lem} 
%		\left|  (S_j \setminus S_{j+1}) \cap E_i \right|  = \left|  (S_{j+1} \setminus S_{j}) \cap E_i \right| \leq 1.
%	\end{equation*} %$$ \left|  (S_j \setminus S_{j+1}) \cap E_i \right|  = \left|  (S_{j+1} \setminus S_{j}) \cap E_i \right| \leq 1.$$
%	
%	%satisfying the following. \begin{itemize}
%		%			\item For all 
%		%		\end{itemize}
%\end{lemma}


%\begin{lemma}
%	\label{lem:chain}
%	There is an algorithm \textnormal{\textsf{Exchange}} that given a \textnormal{KCMB} instance $I =  (E,\cI,c,d,D)$, $\eps>0$, a pattern vector $P$ of $I$ and $\eps$, and $S,S' \in \co_{I,\eps}(P)$ returns in time $\io$ a set $S'' \in \co_{I,\eps}(P)$ such that $\left|S^{\prime \prime} \backslash S^{\prime}\right|<\left|S \backslash S^{\prime}\right|=x$ and for all $i \in \{0,1,\ldots,k_{\eps}\}$ it holds that \begin{equation*}
%		\label{eq:lem} 
%		\left|  (S'' \setminus S) \cap E_i(I,\eps) \right|  = \left|  (S \setminus S'') \cap E_i(I,\eps) \right| \leq 1.
%	\end{equation*} %$$ \left|  (S_j \setminus S_{j+1}) \cap E_i \right|  = \left|  (S_{j+1} \setminus S_{j}) \cap E_i \right| \leq 1.$$
%	
%	%satisfying the following. \begin{itemize}
%		%			\item For all 
%		%		\end{itemize}
%\end{lemma}
%
%\begin{proof}
%		Let $\lambda = \lambda_{I,\eps,P}$ and let $c_{\lambda}(e) = c(e)-\lambda \cdot d(e)$ for every $e \in E$. %In addition, if $c_{\lambda}(e) = 0$ for all $e \in E$ the define $\eps' = 1$; otherwise, define $\eps' = \frac{\min_{e \in E} c_{\lambda}(e)}{2 \cdot |E|}$. 
%		We consider an altered cost function $c'$ (w.r.t. a small enough $\eps'>0$) defined as follows. 
%	
%	$$
%	c^{\prime}(e)= \begin{cases}\infty & \text { if } e \notin S \cup S^{\prime} \\ c_{\lambda}(e)+\epsilon^{\prime} & \text { if } e \in S \backslash S^{\prime} \\ c_{\lambda}(e)-\epsilon^{\prime} & \text { if } e \in S^{\prime} \backslash S \\ c_{\lambda}(e) & \text { if } e \in S \cap S^{\prime}\end{cases}
%	$$
%
%	As a consequence of Theorem 4 in \cite{brezovec1988matroid}, we can compute in time $\io$ a common basis $S^{\prime \prime}$ of $\cI$ and $\cj_{I,\eps}(P)$ that has a smaller cost than $S$ w.r.t. $c^{\prime}$ and that for all $i \in \{0,1,\ldots, k_{\eps}\}$ it holds that $|(S \setminus S'') \cap E_i| = |(S'' \setminus S) \cap E_i| \leq 1$; therefore, $S^{\prime \prime} \in \mathcal{O}_{I,\eps}(P)$. Observe that $S^{\prime \prime} \subseteq S \cup S^{\prime}$ otherwise the cost of $S''$ w.r.t. $c'$ is $\infty$ in contradiction that $c'(S'')< c'(S)$. Moreover, $S^{\prime \prime} \neq S$ since $c'(S'')< c'(S)$; therefore, by the definition of the cost function $c'$ and since $c'(S'')< c'(S)$, it holds that $\left|S^{\prime \prime} \backslash S^{\prime}\right|<\left|S \backslash S^{\prime}\right|$.
%\end{proof}



\begin{lemma}
	\label{lem:chain}
	There is an algorithm \textnormal{\textsf{Chain}} that given a \textnormal{KCMB} instance $I =  (E,\cI,c,d,D)$, $\eps>0$, a pattern vector $P$ of $I$ and $\eps$, and $S,S' \in \co_{I,\eps}(P)$ returns in time $\io$ a sequence $S = S_0, S_1, \ldots, S_{\ell} = S' \in \co_{I,\eps}(P)$, $\ell \in [n_I]$, such that for all $i \in \{0,1,\ldots,k_{\eps}\}$ and $j \in \{0,1,\ldots,\ell-1\}$ it holds that \begin{equation*}
		\label{eq:lem} 
		\left|  (S_j \setminus S_{j+1}) \cap E_i(I,\eps) \right|  = \left|  (S_{j+1} \setminus S_{j}) \cap E_i(I,\eps) \right| \leq 1.
	\end{equation*} %$$ \left|  (S_j \setminus S_{j+1}) \cap E_i \right|  = \left|  (S_{j+1} \setminus S_{j}) \cap E_i \right| \leq 1.$$
	
	%satisfying the following. \begin{itemize}
		%			\item For all 
		%		\end{itemize}
\end{lemma}




\begin{algorithm}[h]
	\caption{$\textsf{EPTAS}(I = (E, \cI, c,d, D),\eps)$}
	\label{alg:findRep}
	\SetKwInOut{Input}{input}
	\SetKwInOut{Output}{output}
	
%	\Input{A KCMB instance $I$ and error parameter $\eps>0$. }%\ariel{I removed $\alpha$, it was not required. } }
%
%\Output{A representative set $R$ of $I$ and $\eps$.}

%	Compute a $2$-approximation $S^*$ for $I$ using a PTAS for BM  with parameter $\eps' = \frac{1}{2}$.\label{step:REPAPP}
%	
%	Set $\alpha \leftarrow p(S^*)$. \label{step:REPalpha}

%		\If{$|I|<\ell^{(k-1) \cdot \ell}$}{Return $E$.\label{step:ifR}}
%	
%	Initialize $R \leftarrow \emptyset$.


%\If{$\ell^{(k-1) \cdot \ell } \cdot k^2  \cdot \eps^{-2}> |I|$}{Return $E$.\label{step:IF}}
%
%Compute $\alpha \leftarrow \textsf{ApproxBM}(I)$.\label{step:A}

Compute a solution $A$ of $I$. 

\For{\textnormal{pattern vectors $P$ of $I$ and $\eps$} \label{step:REPforr}}{
	
	Compute $S,S' \in \co_{I,\eps}(P)$ such that $d(S) \leq D \leq d(S')$.
	
	Compute $(S_0,\ldots, S_{\ell_P}) \leftarrow \textsf{Chain}(I,\eps,P,S,S')$.

Let $j \in \{0,1,\ldots\ell_P-1\}$ be the first index such that $c(S_j) \leq LR_{I,\eps}(\lambda_{I,\eps,P}) \leq c(S_{j+1})$
	
	\If{$S_{j+1}$ is a solution of $I$ and $c(S_{j+1})< c(A)$}{

Update $A \leftarrow S_{j+1}$. 	

}
}

Return $A$.\label{step:REPret}
\end{algorithm}

%\begin{proof}
%	Algorithm \textsf{Chain} is defined as follows. If $S = S'$ then return $S$. Otherwise, compute algorithm $\textsf{Exchange}$ on $I,\eps,P,S,S'$ to get a set $S''$. Then, return $S$ concatenated by the result from a recursive application of algorithm $\textsf{Exchange}$ on $I,\eps,P,S'',S'$. Observe that $|S'' \setminus S'| < |S \setminus S'|$ by Lemma~\ref{lem:exchange}; thus, the algorithm stops after at most $|E|$ iterations. Since each iteration take $\io$ computation time, the overall running time of algorithm $\textsf{Chain}$ is $\io$. We prove by induction on $|S' \setminus S|$ that algorithm \textsf{Chain} returns the desired sequence. For the base case, if $|S' \setminus S| = 0$, the claim follows by the stopping condition of the algorithm; otherwise, assume that the algorithm the desired sequence for $|S'\setminus S| = x-1$ for some $x \in \mathbb{N}$; then, by Lemma~\ref{lem:exchange}, the assumption of the induction, we immediately have the claim. 
%	
%%	We show that we can find a sequence as described in the statement of the lemma in time $\io$; we construct the sequence inductively on $|S' \setminus S|$. We show that our algorithm returns the desired sequence in length at most $|S' \setminus S|$ and in time $\io$. For $|S' \setminus S| = 1$, our algorithm simply returns the sequence $S,S'$ which satisfies the conditions of the lemma. Assume that the claim holds for $|S' \setminus S| = x-1$ for some $x$; that is, assume that we can compute in time $\io$.
%%	
%%	we now prove it for $|S' \setminus S| = x$. 
%%	
%%	
%%	Let $\lambda = \lambda_{I,\eps,P}$ and let $c_{\lambda}(e) = c(e)-\lambda \cdot d(e)$ for every $e \in E$. We consider an altered cost function $c'$ that considers a small enough $\eps'>0$ defined as follows. 
%%	
%%	$$
%%	c^{\prime}(e)= \begin{cases}\infty & \text { if } e \notin S \cup S^{\prime} \\ c_{\lambda}(e)+\epsilon^{\prime} & \text { if } e \in S \backslash S^{\prime} \\ c_{\lambda}(e)-\epsilon^{\prime} & \text { if } e \in S^{\prime} \backslash S \\ c_{\lambda}(e) & \text { if } e \in S \cap S^{\prime}\end{cases}
%%	$$
%%	%We take $T$ to be the initial solution to the primal algorithm in \cite{brezovec1988matroid}. $T$ is not optimal with respect to $c^{\prime}$ (because $T^{\prime}$ is the unique optimal solution with respect to $c^{\prime}$ ), and therefore the algorithm finds a negative cycle in a graph $S$. 
%%%	We define  a graph $H$ to be used in the algorithm; for the definition of $H$, we use the following auxiliary bipartite directed graph $B=\left(V, V^{\prime}, A\right)$ (see also \cite{brezovec1986two} and \cite{brezovec1988matroid}). For every $e \in S$ we define a vertex in $V$, and for every $e^{\prime} \in E \backslash S$ we have a vertex in $V^{\prime}$. For every $e_i \in S$ and $e_j^{\prime} \in E \backslash S$ we construct an edge $\left(e_i, e_j^{\prime}\right)$ with cost $c\left(e_i, e_j^{\prime}\right)=c^{\prime}\left(e_i\right)-c^{\prime}\left(e_j\right)$ if and only if $(S-e_i)+e'_j \in \cI$ (is independent in the matroid  $(E,\cI)$); moreover, we construct an edge $\left(e_j^{\prime}, e_i\right)$ with cost $c\left(e_j^{\prime}, e_i\right)=0$ if and only if $(S-e_i)+e'_j \in \cj_{I,\eps}(P)$ (is independent in the partition matroid $(E,\cj_{I,\eps}(P))$); i.e., $e_i$ and $e_j^{\prime}$ belong to the same set of the partition in $\cj_{I,\eps}(P)$. Since for $e \notin S \cup S^{\prime}$ it holds that $c^{\prime}(e)=\infty$, a directed cycle in $B$ with negative total cost (a {\em negative cycle}) cannot contain $e$ since it has an infinite cost and there are only a finite number of edges with negative costs which all have finite costs.  Now, define the graph $H = (V,\{v_0,\ldots,v_k\},\mathcal{E})$ as follows. First, $V$ is the set $S$ as defined for the graph $B$. Second, for every $i \in \{0,1,\ldots,k\}$ we have  a vertex $v_i$, such that for all $e \in V$ there is an edge $(v,v_i) \in \mathcal{E}$ if and only if there is $e' \in (E \setminus S) \cap E_{i}(I,\eps)$ such that $(e,e') \in A$ (is an edge in the graph $B$). 
%%%	
%%%	We construct a negative cycle $\cC$ in $H$ with minimum number of edges among all negative cycles in $B$. The cycle $\cC$ can be computed in time $\io$ (see, e.g., \cite{brezovec1988matroid} for more details). % by uniting the set of vertices corresponding to elements from $(E \backslash S) \cap E_i(I,\eps)$ in $V^{\prime}$ to a single vertex $v_i$ for every $i \in [k_{\eps}]$, and removing parallel edges.
%%	%
%%	By Theorem 4 in \cite{brezovec1988matroid}, we can compute in time $\io$ a common basis $S^{\prime \prime}$ of $\cI$ and $\cj_{I,\eps}(P)$ that has a smaller cost than $S$ w.r.t. $c^{\prime}$ and that for all $i \in \{0,1,\ldots, k_{\eps}\}$ it holds that $|(S \setminus S'') \cap E_i| = |(S'' \setminus S) \cap E_i| \leq 1$; therefore, $S^{\prime \prime} \in \mathcal{O}_{I,\eps}(P)$. 
%%	
%%	%Moreover, $S^{\prime \prime}$ can be computed in time $\io$ from $S$ by swapping edges along the negative cycle $\cC$. Suppose that the sequence of vertices along the cycle $\cC$ corresponds to the elements $\left(e_1, e_1^{\prime}, e_2, e_2^{\prime}, \ldots, e_l, e_l^{\prime}, e_1\right)$ such that $e_r \in E_{i_r}(I,\eps)$ for $r \in [\ell]$ and $e'_r \in S$ for $r \in [\ell]$. Since $\cC$ is a negative cycle with minimum number of edges, it clearly holds that $C$ is a simple cycle; therefore, $i_r \neq i_{r^{\prime}}$ for all $r,r^{\prime} \in [\ell], r \neq r^{\prime}$. Thus, $S^{\prime \prime} \in \mathcal{O}_{I,\eps}(P)$. 
%%	Observe that $S^{\prime \prime} \subseteq S \cup S^{\prime}$ otherwise the cost of $S''$ w.r.t. $c'$ is $\infty$ in contradiction that $c'(S'')< c'(S)$. Moreover, and $S^{\prime \prime} \neq S$ since $c'(S'')< c'(S)$; therefore, $\left|S^{\prime \prime} \backslash S^{\prime}\right|<\left|S \backslash S^{\prime}\right|=x$. Thus, by the induction assumption, we can compute the entire sequence from $S$ as desired. Observe that adding one set $S_i$ to the sequence takes $\io$ time by By Theorem 4. Moreover, the length of the sequence is at most $|S \setminus S''| \leq |E|$; thus, algorithm $\textsf{Chain}$ runs in time $\io$. 
%\end{proof}

%\begin{proof}
%	We show that we can find the described sequence in time $\io$; we construct the sequence inductively on $|S' \setminus S|$. For $|S' \setminus S| = 1$, the claim trivially holds and the algorithm just returns the sequence $S,S'$. Assume that the claim holds for $|S' \setminus S| = x-1$ for some $x$; we now prove it for $|S' \setminus S| = x$. Let $\lambda = \lambda_{I,\eps,P}$ and let $c_{\lambda}(e) = c(e)-\lambda \cdot d(e)$ for every $e \in E$. We consider an altered cost function $c'$ that considers a small enough $\eps'>0$ defined as follows. 
%	
%	$$
%	c^{\prime}(e)= \begin{cases}\infty & \text { if } e \notin S \cup S^{\prime} \\ c_{\lambda}(e)+\epsilon^{\prime} & \text { if } e \in S \backslash S^{\prime} \\ c_{\lambda}(e)-\epsilon^{\prime} & \text { if } e \in S^{\prime} \backslash S \\ c_{\lambda}(e) & \text { if } e \in S \cap S^{\prime}\end{cases}
%	$$
%	%We take $T$ to be the initial solution to the primal algorithm in \cite{brezovec1988matroid}. $T$ is not optimal with respect to $c^{\prime}$ (because $T^{\prime}$ is the unique optimal solution with respect to $c^{\prime}$ ), and therefore the algorithm finds a negative cycle in a graph $S$. 
%	We define an auxiliary bipartite directed graph $B=\left(V, V^{\prime}, A\right)$ as follows (see \cite{brezovec1986two} and \cite{brezovec1988matroid}). For every $e \in S$ we define a vertex in $V$, and for every $e^{\prime} \in E \backslash T$ we have a vertex in $V^{\prime}$. For every $e_i \in S$ and $e_j^{\prime} \in E \backslash S$ we construct an edge $\left(e_i, e_j^{\prime}\right)$ with cost $c\left(e_i, e_j^{\prime}\right)=c^{\prime}\left(e_i\right)-c^{\prime}\left(e_j\right)$ if and only if $(S-e_i)+e'_j \in \cI$ (is independent in the matroid  $(E,\cI)$); moreover, we construct an edge $\left(e_j^{\prime}, e_i\right)$ with cost $c\left(e_j^{\prime}, e_i\right)=0$ if and only if $(S-e_i)+e'_j \in \cj_{I,\eps}(P)$ (is independent in the partition matroid $(E,\cj_{I,\eps}(P))$); i.e., $e_i$ and $e_j^{\prime}$ belong to the same set of the partition in $\cj_{I,\eps}(P)$. Since for $e \notin S \cup S^{\prime}$ it holds that $c^{\prime}(e)=\infty$, a directed cycle in $B$ with negative total cost (a {\em negative cycle}) cannot contain $e$ since it has an infinite cost and there are only a finite number of edges with negative costs which all have finite costs.  
%	
%	We construct a negative cycle $\cC$ in $B$. The cycle $\cC$ is obtained from $B$ (see \cite{brezovec1988matroid}) by uniting the set of vertices corresponding to elements from $(E \backslash S) \cap E_i(I,\eps)$ in $V^{\prime}$ to a single vertex $v_i$ for every $i \in [k_{\eps}]$, and removing parallel edges.
%	
%	By Theorem 4 in \cite{brezovec1988matroid}, there is a common base $S^{\prime \prime}$ of $\cI$ and $\cj_{I,\eps}(P)$ that has a smaller cost than $S$ with respect to $c^{\prime}$; therefore, $S^{\prime \prime} \in \mathcal{O}_{I,\eps}(P)$, and it holds that such that $S^{\prime \prime}$ is obtained from $S$ by swapping edges along a negative cycle $\cC$ that has a minimum number of edges (among all the negative cycles in $S$). Suppose that the nodes along the cycle $C$ correspond to edges $\left(e_1, e_1^{\prime}, e_2, e_2^{\prime}, \ldots, e_l, e_l^{\prime}, e_1\right)$ such that $e_k \in E_{i_k}$ for $k=1, \ldots, l$. $C$ is simple, and therefore, $i_k \neq i_{k^{\prime}} \forall k \neq k^{\prime}$ and $T^{\prime \prime} \in \mathcal{O}$.
%	$T^{\prime \prime} \subseteq T \cup T^{\prime}$ and $T^{\prime \prime} \neq T$, and therefore, $\left|T^{\prime \prime} \backslash T^{\prime}\right|<\left|T \backslash T^{\prime}\right|=x$. Therefore, by the induction assumption, the lemma's claim holds.
%\end{proof}


%\begin{proof}
%	We show that we can find the described sequence in time $\io$; we construct the sequence inductively on $|S' \setminus S|$. For $|S' \setminus S| = 1$, the claim trivially holds and the algorithm just returns the sequence $S,S'$. Assume that the claim holds for $|S' \setminus S| = x-1$ for some $x$; we now prove it for $|S' \setminus S| = x$. Let $\lambda = \lambda_{I,\eps,P}$ and let $c_{\lambda}(e) = c(e)-\lambda \cdot d(e)$ for every $e \in E$. We consider an altered cost function $c'$ that considers a small enough $\eps'>0$ defined as follows. 
%	
%	$$
%	c^{\prime}(e)= \begin{cases}\infty & \text { if } e \notin S \cup S^{\prime} \\ c_{\lambda}(e)+\epsilon^{\prime} & \text { if } e \in S \backslash S^{\prime} \\ c_{\lambda}(e)-\epsilon^{\prime} & \text { if } e \in S^{\prime} \backslash S \\ c_{\lambda}(e) & \text { if } e \in S \cap S^{\prime}\end{cases}
%	$$
%	%We take $T$ to be the initial solution to the primal algorithm in \cite{brezovec1988matroid}. $T$ is not optimal with respect to $c^{\prime}$ (because $T^{\prime}$ is the unique optimal solution with respect to $c^{\prime}$ ), and therefore the algorithm finds a negative cycle in a graph $S$. 
%	We define  a graph $H$ to be used in the algorithm; for the definition of $H$, we use the following auxiliary bipartite directed graph $B=\left(V, V^{\prime}, A\right)$ (see also \cite{brezovec1986two} and \cite{brezovec1988matroid}). For every $e \in S$ we define a vertex in $V$, and for every $e^{\prime} \in E \backslash S$ we have a vertex in $V^{\prime}$. For every $e_i \in S$ and $e_j^{\prime} \in E \backslash S$ we construct an edge $\left(e_i, e_j^{\prime}\right)$ with cost $c\left(e_i, e_j^{\prime}\right)=c^{\prime}\left(e_i\right)-c^{\prime}\left(e_j\right)$ if and only if $(S-e_i)+e'_j \in \cI$ (is independent in the matroid  $(E,\cI)$); moreover, we construct an edge $\left(e_j^{\prime}, e_i\right)$ with cost $c\left(e_j^{\prime}, e_i\right)=0$ if and only if $(S-e_i)+e'_j \in \cj_{I,\eps}(P)$ (is independent in the partition matroid $(E,\cj_{I,\eps}(P))$); i.e., $e_i$ and $e_j^{\prime}$ belong to the same set of the partition in $\cj_{I,\eps}(P)$. Since for $e \notin S \cup S^{\prime}$ it holds that $c^{\prime}(e)=\infty$, a directed cycle in $B$ with negative total cost (a {\em negative cycle}) cannot contain $e$ since it has an infinite cost and there are only a finite number of edges with negative costs which all have finite costs.  Now, define the graph $H = (V,\{v_0,\ldots,v_k\},\mathcal{E})$ as follows. First, $V$ is the set $S$ as defined for the graph $B$. Second, for every $i \in \{0,1,\ldots,k\}$ we have  a vertex $v_i$, such that for all $e \in V$ there is an edge $(v,v_i) \in \mathcal{E}$ if and only if there is $e' \in (E \setminus S) \cap E_{i}(I,\eps)$ such that $(e,e') \in A$ (is an edge in the graph $B$). 
%	
%	 We construct a negative cycle $\cC$ in $H$ with minimum number of edges among all negative cycles in $B$. The cycle $\cC$ can be computed in time $\io$ (see, e.g., \cite{brezovec1988matroid} for more details). % by uniting the set of vertices corresponding to elements from $(E \backslash S) \cap E_i(I,\eps)$ in $V^{\prime}$ to a single vertex $v_i$ for every $i \in [k_{\eps}]$, and removing parallel edges.
%	%
%	By Theorem 4 in \cite{brezovec1988matroid}, there is a common basis $S^{\prime \prime}$ of $\cI$ and $\cj_{I,\eps}(P)$ that has a smaller cost than $S$ with respect to $c^{\prime}$; therefore, $S^{\prime \prime} \in \mathcal{O}_{I,\eps}(P)$. Moreover, $S^{\prime \prime}$ can be computed in time $\io$ from $S$ by swapping edges along the negative cycle $\cC$. Suppose that the sequence of vertices along the cycle $\cC$ corresponds to the elements $\left(e_1, e_1^{\prime}, e_2, e_2^{\prime}, \ldots, e_l, e_l^{\prime}, e_1\right)$ such that $e_r \in E_{i_r}(I,\eps)$ for $r \in [\ell]$ and $e'_r \in S$ for $r \in [\ell]$. Since $\cC$ is a negative cycle with minimum number of edges, it clearly holds that $C$ is a simple cycle; therefore, $i_r \neq i_{r^{\prime}}$ for all $r,r^{\prime} \in [\ell], r \neq r^{\prime}$. Thus, $S^{\prime \prime} \in \mathcal{O}_{I,\eps}(P)$. 
%	$T^{\prime \prime} \subseteq T \cup T^{\prime}$ and $T^{\prime \prime} \neq T$, and therefore, $\left|T^{\prime \prime} \backslash T^{\prime}\right|<\left|T \backslash T^{\prime}\right|=x$. Therefore, by the induction assumption, the lemma's claim holds.
%\end{proof}

\comment{
	\begin{proof}
		The proof of 
		
		\comment{the lemma is based on exchanging elements from $S$ until reaching $S'$. The proof uses induction on $x = |S \setminus S'|$. For $x = 0$ the claim trivially follows. Assume that the claim holds for any pair $S,S'$ with $|S \setminus S'| = x-1$. We now prove the claim for $|S \setminus S'| = x$. We define an altered cost function to isolate the specific optimal solution $S'$ of $\co$.  For all $e \in E$ and a sufficiently small $\delta>0$ define \begin{equation}
				\label{eq:c'}
				c'(e) = 
				\begin{cases}
					\infty &  e \notin S \cup S', \\
					c_{\lambda}(e)+\delta &  e \in S \setminus S', \\
					c_{\lambda}(e)-\delta &  e \in S' \setminus S, \\
					c_{\lambda}(e) &  e \in S' \cap S. \\
				\end{cases}
			\end{equation} Note that by \eqref{eq:c'} we have that $S'$ is the unique optimal solution of \eqref{eq:LR} with parameter $\lambda$ with the cost function $c'$ (if $\delta$ is small enough). Thus, $S$ is not optimal w.r.t. $c'$. We define the directed bipartite graph $B= (T,E\setminus T,A)$ (i.e., the vertices of $B$ are $E$, with the bipartition $T,E \setminus T$ and the edge set is $A$) such that the following holds. \begin{enumerate}
				\item $B$
		\end{enumerate}}
\end{proof}}
%	Thus, using the work of Megiddo \cite{megiddo1978combinatorial} we can find $M_1, M_2 \in \cm(G), M_1 \cap L = M_2 \cap L = L^*$ such that the following holds. 
%		
%		\begin{equation}
	%			\label{eq:Megido}
	%			\begin{aligned}
		%				c(M_2) \leq{} & D \leq c(M_1), \\
		%				\\
		%				c_{\lambda} (M_1) ={} & c_{\lambda} (M_2) = LR(\lambda). 
		%			\end{aligned}
	%		\end{equation} We can now state the following inequality, for each matching $M \in \{M_1, M_2\}$: \begin{equation}
	%			\label{eq:opt}
	%			s
	%		\end{equation}



\begin{lemma}
	\label{lem:EPTASbound}
	We can find $S \in \co$ such that $c(S) \leq (1+4 \cdot \eps) \cdot \OPT(I)$ and $d(S) \geq D$. 
\end{lemma}

\begin{proof}
	Since the matroid intersection problem is polynomially solvable, the problems described in \eqref{eq:LR} and \eqref{eq:Lambda} are polynomially solvable. Thus, using the parametric search technique \cite{megiddo1978combinatorial} we can find in polynomial time $S,S' \in \co$ such that $d(S) \leq D \leq d(S')$ and therefore $c(S) \leq LR(\lambda) \leq c(S')$. Then, by Lemma~\ref{lem:chain} we can find a sequence $S = S_0, S_1, \ldots, S_{\ell} = S' \in \co$, $\ell \in [n]$ satisfying the conditions of the lemma. Since $c(S') \leq LR(\lambda) \leq c(S)$, there is $j \in \{0,1,\ldots,\ell-1\}$ such that $c(S_j) \leq LR(\lambda) \leq c(S_{j+1})$. Hence, \begin{equation}
		\label{eq:2}
		c(S_{j+1}) \leq c(S_j)+\sum_{i \in \{0,1,\ldots,k\}} \left(\max_{e \in E_i} c(e) - \min_{e \in E_i} c(e)\right) \leq \OPT(I) + \eps \cdot C+ \frac{1}{\eps} \cdot \eps^2 C \leq (1+4 \cdot \eps) \cdot \OPT(I). 
	\end{equation} The first inequality holds by Lemma~\ref{lem:chain} and \eqref{eq:class}. The second inequality follows since the class $E_0$ may contribute to the sum at most $\eps \cdot C$, and only other $\frac{1}{\eps}$ cost classes can contribute to the sum, where the contribution of such a cost class is bounded by $\eps^2 \cdot C$ due to \eqref{eq:class}. The last inequality holds since $C \leq 2 \cdot \OPT$.  Finally, since $S_{j+1} \in \co$ and $c(S_{j+1} \geq LR(\lambda))$ it follows that $d(S_{j+1}) \geq D$. 
	%			Let $\lambda^{-} = \lambda - \delta$ for a small enough $\delta>0$. It follows that there is $S^- \in \co$ that is optimal also w.r.t. the cost function $c_{\lambda^{-}}$ (rather than $c_{\lambda}$). Since $c_{\lambda}(S^-) = LR(\lambda^-) \leq LR(\lambda)$ it follows that \begin{equation}
		%				\label{eq:-}
		%			c(S^-)+ \lambda^- \cdot (D-d(S^-)) \leq c(S^-) +  \lambda \cdot (D-d(S^-)) = LR(\lambda).
		%			\end{equation} The equality follows since $S^- \in \co$. 
\end{proof}

The above gives an EPTAS for KCMB and therefore also to KCM by Lemma~\ref{lem:b}. 	(TODO: add pseudocode and further details)
%	We can now describe our EPTAS. Given a KCM instance we first reduce it to a family of KCMB instances $I_{\alpha}$, for all $\alpha$ that can be the cardinality of the optimum of $I$ (i.e., $\alpha \in [b]$ where $b$ is the maximal independent set in the given matroid), as in the proof of Lemma~\ref{lem:b}. For each instance $I_{\alpha}$ we compute the two approximation $C$, enumerate over all pattern vectors, for each pattern vector we define a corresponding partition matroid


\comment{
\section{Hardness result for KCM}


(TODO: change the size function to $d$)


%In the following, we define a family of matroids. 
\begin{lemma}
	\label{lem:KCM}
	There is no \textnormal{FPTAS} for \textnormal{KCM} unless \textnormal{P=NP}.%is Strongly \textnormal{NP}-complete
\end{lemma}

\noindent	{\em Proof.}
%Let $X = (E,v,\sigma,H,T)$ be an GSS instance and let $n = |E|$. 
We give a reduction from the $k$-clique problem. Let $G = (V,E)$ be a graph and let $k \in \mathbb{N}_{>0}$; the goal is to decide whether there is a clique of size $k$ in $G$. Let $C(G)$ be all cliques in $G$. Let $|V| = n$ and let $\sigma : V \rightarrow [n]$ be an arbitrary bijeciton. For every $\alpha \in [n^2]$ define the matroid $M_{\alpha} = (V,\cI_{\alpha})$, $\cI_{\alpha} = \cI^1_{\alpha} \cup \cI^2_{\alpha} \cup \cI^3_{\alpha}$, such that \begin{equation}
	\label{eq:1}
	\begin{aligned}
		\cI^1_{\alpha} = {} & \{S \subseteq V~\big|~ |S| < k\} \\
		\cI^2_{\alpha} = {} & \{S \subseteq V~\big|~ |S| = k, \sigma(S) \neq \alpha\} \\
		\cI^3_{\alpha} = {} & \{S \subseteq V~\big|~ |S| = k, \sigma(S) = \alpha, S \in C(G)\}. \\
	\end{aligned}
\end{equation}
\begin{claim}
	\label{claim:1}
	For all $\alpha \in [n^2]$ it holds that $M_{\alpha}$ is a matroid.
\end{claim}
\begin{proof}
	First, note that $\emptyset \in \cI^1_{\alpha}$ since $k \geq 1$ and it follows that $\emptyset \in \cI_{\alpha}$. For the hereditary property, let $A \in \cI_{\alpha}$. For all $B \subset A$ it holds that $|B| < k$; thus, $B \in \cI^1_{\alpha}$ and it follows that $B \in \cI_{\alpha}$. For the exchange property, let $A,B \in \cI_{\alpha}$ such that $|A| > |B|$. We consider the following cases. \begin{itemize}
		\item $|B| < k-1$. Then, for all $e \in A \setminus B$ it holds that $|B+e| < k-1+1 = k$; thus, $B+e \in \cI^1_{\alpha}$ and it follows that $B+e \in \cI_{\alpha}$. Note that there is such $e  \in A \setminus B$ because $|A| > |B|$. 
		
		\item $|B| = k-1$ and $|A| = k$. We consider two sub cases.  \begin{enumerate}
			\item $B \subseteq A$. Then, because $|A| > |B|$ there is $e \in A \setminus B$; thus, $B+e = A$ (because $|B| = k-1$ and $|A| = k$). Hence, since $A \in \cI_k$ it follows that $B+e \in \cI_k$.
			
			\item $B \not\subseteq A$.  Then, since $|B| = k-1$ and $|A| = k$ it follows that $|B \cap A| < |B| = k-1$; thus, $|A \setminus B| = |A|-|A \cap B| > k - (k-1) = 1$. Thus, there are $e,f \in A \setminus B, e\neq f$; since $\sigma$ is a bijection, it holds that $\sigma(e) \neq \sigma(f)$. Therefore, there is $g \in \{e,f\}$ such that $\sigma(B+g) \neq \alpha$. We conclude that $B+g \in \cI^2_{\alpha}$ and it follows that $B+g \in \cI_{\alpha}$. 
		\end{enumerate}
	\end{itemize}
\end{proof}

%Let $\alpha = 2 \cdot n^2$ and $\beta = 2 \cdot v(E)$. We assume w.l.o.g that $n \geq 1$ and that $v(E) > 0$. 
Let $r = 2n^2$. For every ${\alpha} \in  [n^2]$ define the KCM instance $I_{\alpha} = (V,\cI_{\alpha},c,s,D_{\alpha})$ such that the following holds. \begin{equation}
	\label{eq:def}
	\begin{aligned}
		c(e) ={} &  \sigma(e)  ~~\forall e \in V \\
		s(e) ={} & r+\sigma(e)~~\forall e \in V \\
		D_{\alpha} ={} &  k \cdot r+\alpha. %eta \cdot H+T.
	\end{aligned}
\end{equation}

We need to resolve a small technical issue for the single case where $I_{\alpha}$ is not well defined. Since $\sigma$ is a bijection, there is exactly one set $H \subseteq E$ that contains the $k$ elements with maximal values according to $\sigma$. If $\sigma(H) = \alpha$ and $H \notin C(G)$, then there is no solution for $I_{\alpha}$; in this case, we call $I_{\alpha}$ a {\em pseudo} KCM instance. Alternatively, for any $\alpha \in [n^2]$ it holds that $H \in \cI_{\alpha}$ and $s(H) \geq D_{\alpha}$ and thus $I_{\alpha}$ has a solution and is well defined. %If $H \in \cI_{\alpha}$, then we say that $I_{\alpha}$ is a {\em }

%taking the set $H$ of the $k$ vertices with the largest value of $\sigma$ is a solution for $\alpha$: either $\sigma(H) \neq \alpha$ and then $H \in \cI^2_{\alpha}$ and therefore $H \in \cI_{\alpha}$; otherwise, if $\sigma(H) = \alpha$ then we repeat the construction with any bijection $\sigma': V \rightarrow [n]$,
\comment{
	\begin{claim}
		\label{claim:aux1}
		Let $k \in [n]$ and let $S_k$ be an optimal solution for $I_k$. Then the following holds. \begin{enumerate}
			\item $|S_k| \geq k$. 
			\item %If $|S_k| < k$ then $s(S_k)< k \cdot \alpha+H$ and 
			$c(S_k) \geq k \cdot \alpha+H$.
			\item It holds that $\sigma(S_k) \leq H$. 
		\end{enumerate}
	\end{claim}
	
	\begin{proof}
		For the first property of the claim, assume towards a contradiction that $|S_k| < k$. Then,  \begin{equation*}
			\label{eq:sB2}
			\begin{aligned}
				c(S_k) = {} & |S_k| \cdot \alpha+\sigma(S_k) \leq (k-1) \cdot \alpha+\sigma(E) \leq (k-1) \cdot 2 \cdot n^2 +n^2 = k \cdot \alpha-n^2  < k \cdot \alpha \leq k \cdot \alpha +D. 
			\end{aligned}
		\end{equation*} The first inequality holds since $\sigma$ is non negative and assuming that $|S_k| < k$. The second inequality uses that $\sigma(E) \leq n^2$. %Now, if $|S_k| = k$
		For the second property of the claim, assume towards a contradiction that $\sigma(S_k)>D$. Then, \begin{equation*}
			\label{eq:sB2}
			\begin{aligned}
				c(S_k) = {} & \beta \cdot \sigma(S_k)+v(S_k) \geq \beta \cdot (D+1)+v(S_k) \geq \beta \cdot D+\beta = \beta \cdot D+2 \cdot v(E) > \beta \cdot D+T = B.
			\end{aligned}
		\end{equation*} The first inequality follows from our assumption and that $\sigma$ gives integral values for the elements. By the above, we reach a contradiction that $S_k$ is a solution for $I_k$. Therefore, we conclude that $\sigma(S_k) \leq D$ and it follows that $p(S_k) \leq k \cdot \alpha+D$ (because $|S_k| \leq k$).  
	\end{proof}
	
	\begin{claim}
		\label{claim:iff}
		There is a solution for the \textnormal{GSS} instance $X$ if and only if there is $k \in [n]$ such that the optimal solution for $I_k$ has cost exactly $k \cdot \alpha+H$. 
	\end{claim}
	
	\begin{proof}
		For the first direction, let $Y \subseteq E$ be a solution for $X$, i.e., it holds that $v(Y) = T$ and $\sigma(Y) = D$. Let $k = |Y|$.  Observe that $c(Y) = \beta \cdot \sigma(Y) +v(Y) = \beta \cdot D+T = B$; moreover, $|Y| = k ,v(Y) = T$, and $\sigma(Y) = D$ and it follows that $Y \in \cI^3_k \subseteq \cI_k$. Thus, $Y$ is a feasible solution for $I_k$. Moreover, it holds that $p(Y) = \alpha \cdot k+\sigma(Y) = \alpha \cdot k+D$; thus, $Y$ is an optimal solution for $I_k$ by Claim~\ref{claim:aux1}. 
		
		For the second direction, let  $k \in [n]$ and let $S_k$ be an optimal solution for $I_k$ of profit exactly $k \cdot \alpha+D$. By Claim~\ref{claim:aux1} and that $p(S_k) = k \cdot \alpha +D$ it follows that $|S_k| \geq k$; we get that $|S_k| = k$ because $S_k \in \cI_k$. Moreover, it follows that $\sigma(S_k) = D$ to have that $p(S_k) = k \cdot \alpha +D$. Then, because $S_k \in \cI_k, |S_k| = k$, and $\sigma(S_k) = D$ it follows by \eqref{eq:1} that $v(S_k) = T$. Overall, we conclude that $S_k$ is a solution for $X$. %and $\sigma(S_k) = D$.  %, assume that there is no solution for $X$. 
	\end{proof}
	
	%By Claim~\ref{claim:iff}, we can 
	
}

\begin{claim}
	\label{claim:alpha}
	For any $\alpha \in [n^2]$ and a solution $S$ for $I_{\alpha}$ it holds that $c(S) \geq \alpha$. 
\end{claim}

\begin{proof}
	We have
	$$c(S) = \sigma(S) = s(S)-r \cdot |S| \geq D_{\alpha} - r \cdot |S| \geq D_{\alpha} - r \cdot k = \alpha.$$ The equalities follow from \eqref{eq:def}. The inequalities hold since $S$ is a solution for $I_{\alpha}$: the first inequality holds since $s(S) \geq D_{\alpha}$ and the second inequality holds since $S \in \cI_{\alpha}$ and thus $|S| \leq k$. 
\end{proof}



\begin{claim}
	\label{claim:iff}
	There is a a clique of size $k$ in $G$ if and only if there is $\alpha \in [n^2]$ such that there is a solution for $I_{\alpha}$ with cost exactly $\alpha$. 
\end{claim}

\begin{proof}
	For the first direction, let $Q$ be a clique of size $k$ in $G$. Let $\sigma(Q) = \alpha$. Then, \begin{equation*}
		\label{eq:D}
		s(Q) = k \cdot r+\sigma(Q) = k \cdot r+\alpha = D_{\alpha}
	\end{equation*} Moreover, since $|Q| = k$, $\sigma(Q) = \alpha$ and $Q \in C(G)$ it follows that $Q \in \cI^3_{\alpha}$ and therefore $Q \in \cI_{\alpha}$. We conclude that $Q$ is a solution for $I_{\alpha}$ with cost $c(Q) = \sigma(Q) = \alpha$. For the second direction, let $\alpha \in [n^2]$ and let $T$ be a solution for $I_{\alpha}$ with cost exactly $\alpha$. Note that if $|T| < k$ it holds that $$s(T) \leq (k-1) \cdot r+ \alpha \leq (k-1) \cdot r+n^2 < k \cdot r < k \cdot r+\alpha = D_{\alpha}.$$ Since in this case $T$ is not a solution for $I_{\alpha}$ we conclude that $|T| \geq k$; moreover, by \eqref{eq:1} it follows that $|T| = k$ since $T \in \cI_{\alpha}$.  In addition, $c(T) = \sigma(T) = \alpha$; thus, since $T \in \cI_{\alpha}$, $|T| = k$, and $\sigma(T) = \alpha$, we conclude that $T \in \cI^3_{\alpha}$. Therefore, $T \in C(G)$ where $|T| = k$ as required.  
	%	For the first direction, let $Y \subseteq E$ be a solution for $X$, i.e., it holds that $v(Y) = T$ and $\sigma(Y) = D$. Let $k = |Y|$.  Observe that $c(Y) = \beta \cdot \sigma(Y) +v(Y) = \beta \cdot D+T = B$; moreover, $|Y| = k ,v(Y) = T$, and $\sigma(Y) = D$ and it follows that $Y \in \cI^3_k \subseteq \cI_k$. Thus, $Y$ is a feasible solution for $I_k$. Moreover, it holds that $p(Y) = \alpha \cdot k+\sigma(Y) = \alpha \cdot k+D$; thus, $Y$ is an optimal solution for $I_k$ by Claim~\ref{claim:aux1}. 
	%	
	%	For the second direction, let  $k \in [n]$ and let $S_k$ be an optimal solution for $I_k$ of profit exactly $k \cdot \alpha+D$. By Claim~\ref{claim:aux1} and that $p(S_k) = k \cdot \alpha +D$ it follows that $|S_k| \geq k$; we get that $|S_k| = k$ because $S_k \in \cI_k$. Moreover, it follows that $\sigma(S_k) = D$ to have that $p(S_k) = k \cdot \alpha +D$. Then, because $S_k \in \cI_k, |S_k| = k$, and $\sigma(S_k) = D$ it follows by \eqref{eq:1} that $v(S_k) = T$. Overall, we conclude that $S_k$ is a solution for $X$. %and $\sigma(S_k) = D$.  %, assume that there is no solution for $X$. 
\end{proof}

Given an FPTAS for KCM we can decide if there is a clique of size $k$ in $G$. We first consider the only value  $\alpha' \in [n^2]$ such that $I_{\alpha'}$ is possibly a pseudo KCM instance (i.e., may not have a feasible solution). In this case, we just check if the set $H$ of the $k$ items with largest values according to $\sigma$ is a clique in $G$; if $H \in C(G)$, we return that there is a clique of size $k$ in $G$. Otherwise, we iterate over all other values $\alpha \in  [n^2] \setminus \{\alpha'\}$, and compute an optimal solution $S_{\alpha}$ for $I_{\alpha}$ using the FPTAS with parameter $\eps = \frac{1}{2 \cdot n^2}$ (these are all well defined instances). Note that the running time is polynomial since $\frac{1}{\eps}$ is polynomial in the input size. If there is $\alpha \in  [n^2] \setminus \{\alpha'\}$ such that $c(S_{\alpha}) = \alpha$, we return that here is a clique of size $k$ in $G$; otherwise, if for all $\alpha \in  [n^2] \setminus \{\alpha'\}$  it holds that  $c(S_{\alpha}) \neq \alpha$, we return that there is no clique of size $k$ in $G$. Note that $\OPT(I_{\alpha}) \leq n \cdot \max_{e \in E} c(e) = n^2$. Thus, 
by the approximation guarantee of the FPTAS with our parameter $\eps$ it follows that $$c(S_{\alpha}) \leq (1+\eps) \cdot \OPT(I_{\alpha}) \leq \OPT(I_{\alpha}) + \frac{n^2}{2 \cdot n^2} < \OPT(I_{\alpha})+1.$$ Since the costs of all the elements are integers, we conclude that $c(S_{\alpha}) = \OPT(I_k)$. %We use the FPTAS with parameter $\eps = \frac{1}{3 \cdot n^3}$. 
%Since for all $k \in [n]$ it holds that $\OPT(I_k)$

By Claim~\ref{claim:alpha} and Claim~\ref{claim:iff} there is a clique of size $k$ in $G$ if and only if $H \in C(G)$ or there is $\alpha \in [n^2] \setminus \{\alpha'\}$ such that $\OPT(I_{\alpha}) = \alpha$. Therefore, we decide correctly whether there is a clique of size $k$ in $G$ in polynomial time. Since the $k$-clique problem is known to be NP-complete, we conclude that KCM does not have an FPTAS unless P=NP.
$\blacksquare$



\section{A Hardness Result for Constrained Minimum Matroid Basis}

Formally, a {\em  constrained minimum matroid masis (CMB)} instance is a tuple $I =  (E,\cI,c,s,L)$, where $(E,\cI)$ is a matroid along with a membership oracle, $c:E \rightarrow \mathbb{R}_{\geq 0}$  gives the element costs, $s:E \rightarrow \mathbb{R}_{\geq 0}$ gives the elements sizes, and $L \in \mathbb{R}_{\geq 0}$ is a budget. A {\em solution} of $I$ is a basis $B \in \cI$ such that $s(B) \leq L$; in addition, the {\em cost} of the solution is $c(B)$ and let $\OPT(I)$ denote the cost of a solution of $I$ with minimum cost. The goal is to find a solution of $I$ of minimum cost. 


%	\section{Hardness result for KCM}


%	(TODO: change the size function to $d$)

%In the following, we define a family of matroids. 
\begin{lemma}
	\label{lem:KCM2}
	There is no \textnormal{FPTAS} for \textnormal{CMB} unless \textnormal{P=NP}.%is Strongly \textnormal{NP}-complete
\end{lemma}

\noindent	{\em Proof.}
%Let $X = (E,v,\sigma,H,T)$ be an GSS instance and let $n = |E|$. 

We give a reduction from the $k$-clique problem. Let $G = (V,E)$ be a graph and let $k \in \mathbb{N}_{>0}$; the goal is to decide whether there is a clique of size $k$ in $G$. Let $C(G)$ be all cliques in $G$. Let $|V| = n$ and let $\sigma : V \rightarrow [n]$ be an arbitrary bijection. For every $\alpha \in [n^2]$ we consider the matroid $M_{\alpha}$ as defined in the previous section. 

%= (V,\cI_{\alpha})$, $\cI_{\alpha} = \cI^1_{\alpha} \cup \cI^2_{\alpha} \cup \cI^3_{\alpha}$, such that \begin{equation}
	%	\label{eq:1}
	%	\begin{aligned}
		%		\cI^1_{\alpha} = {} & \{S \subseteq V~\big|~ |S| < k\} \\
		%		\cI^2_{\alpha} = {} & \{S \subseteq V~\big|~ |S| = k, \sigma(S) \neq \alpha\} \\
		%		\cI^3_{\alpha} = {} & \{S \subseteq V~\big|~ |S| = k, \sigma(S) = \alpha, S \in C(G)\}. \\
		%	\end{aligned}
	%\end{equation}
	%\begin{claim}
	%	\label{claim:1}
	%	For all $\alpha \in [n^2]$ it holds that $M_{\alpha}$ is a matroid.
	%\end{claim}
	%\begin{proof}
	%	First, note that $\emptyset \in \cI^1_{\alpha}$ since $k \geq 1$ and it follows that $\emptyset \in \cI_{\alpha}$. For the hereditary property, let $A \in \cI_{\alpha}$. For all $B \subset A$ it holds that $|B| < k$; thus, $B \in \cI^1_{\alpha}$ and it follows that $B \in \cI_{\alpha}$. For the exchange property, let $A,B \in \cI_{\alpha}$ such that $|A| > |B|$. We consider the following cases. \begin{itemize}
		%		\item $|B| < k-1$. Then, for all $e \in A \setminus B$ it holds that $|B+e| < k-1+1 = k$; thus, $B+e \in \cI^1_{\alpha}$ and it follows that $B+e \in \cI_{\alpha}$. Note that there is such $e  \in A \setminus B$ because $|A| > |B|$. 
		%		
		%		\item $|B| = k-1$ and $|A| = k$. We consider two sub cases.  \begin{enumerate}
			%			\item $B \subseteq A$. Then, because $|A| > |B|$ there is $e \in A \setminus B$; thus, $B+e = A$ (because $|B| = k-1$ and $|A| = k$). Hence, since $A \in \cI_k$ it follows that $B+e \in \cI_k$.
			%			
			%			\item $B \not\subseteq A$.  Then, since $|B| = k-1$ and $|A| = k$ it follows that $|B \cap A| < |B| = k-1$; thus, $|A \setminus B| = |A|-|A \cap B| > k - (k-1) = 1$. Thus, there are $e,f \in A \setminus B, e\neq f$; since $\sigma$ is a bijection, it holds that $\sigma(e) \neq \sigma(f)$. Therefore, there is $g \in \{e,f\}$ such that $\sigma(B+g) \neq \alpha$. We conclude that $B+g \in \cI^2_{\alpha}$ and it follows that $B+g \in \cI_{\alpha}$. 
			%		\end{enumerate}
		%	\end{itemize}
	%\end{proof}
	
	%Let $\alpha = 2 \cdot n^2$ and $\beta = 2 \cdot v(E)$. We assume w.l.o.g that $n \geq 1$ and that $v(E) > 0$. 
	Let $r = 2n^2$ and let $z = \sum^{k}_{i = 2} i $. %and note that $z \in [n^2]$. 
	For every ${\alpha} \in  [n^2] \setminus [z]$ define the CMB instance $I_{\alpha} = (V,\cI_{\alpha},c,s,L_{\alpha})$ such that the following holds. \begin{equation}
		\label{eq:def2}
		\begin{aligned}
			c(e) ={} &  r-\sigma(e)  ~~\forall e \in V \\
			s(e) ={} & \sigma(e)~~\forall e \in V \\
			L_{\alpha} ={} &  \alpha. 
		\end{aligned}
	\end{equation}
	
	We need to resolve a small technical issue for the single case where $I_{\alpha}$ is not well defined. Since $\sigma$ is a bijection, there is exactly one set $H \subseteq E$ that contains the $k$ elements with minimal values according to $\sigma$. If $\sigma(H) = \alpha$ and $H \notin C(G)$, then there is no solution for $I_{\alpha}$ (we either violate the matroid constraint or the knapsack constraint). In this case, we call $I_{\alpha}$ a {\em pseudo} CMB instance. 
	Alternatively, for any $\alpha \in [n^2] \setminus [z]$ it holds that $H \in \cI_{\alpha}$ and $s(H) \leq L_{\alpha}$ and thus $I_{\alpha}$ has at least one solution and is well defined. %If $H \in \cI_{\alpha}$, then we say that $I_{\alpha}$ is a {\em }
	
	
	
	
	
	\begin{claim}
		\label{claim:alpha2}
		For any $\alpha \in [n^2] \setminus [z]$ and a solution $S$ for $I_{\alpha}$ it holds that $c(S) \geq r \cdot k-\alpha$. 
	\end{claim}
	
	\begin{proof}
		We have
		$$c(S) = r \cdot |S|-\sigma(S)  = r \cdot k-\sigma(S) = r \cdot k-s(S) \geq r \cdot k -L_{\alpha} = r \cdot k -\alpha.$$ The equalities follow from \eqref{eq:def2}; also note that $|S| = k$ because $S$ is a basis of $M_{\alpha}$. The inequality holds since $S$ is a solution for $I_{\alpha}$ and it holds that $s(S) \leq L_{\alpha}$. 
	\end{proof}
	
	
	
	\begin{claim}
		\label{claim:iff2}
		There is a a clique of size $k$ in $G$ if and only if there is $\alpha \in [n^2] \setminus [z]$ such that there is a solution for $I_{\alpha}$ with cost exactly $r \cdot k-\alpha$. 
	\end{claim}
	
	\begin{proof}
		For the first direction, let $Q$ be a clique of size $k$ in $G$. Let $\alpha  = \sigma(Q)$ and observe that $\alpha \in [n^2] \setminus [z]$. Then, \begin{equation*}
			\label{eq:D2}
			s(Q) =\sigma(Q) = \alpha = L_{\alpha}. 
		\end{equation*} Moreover, since $|Q| = k$, $\sigma(Q) = \alpha$ and $Q \in C(G)$ it follows that $Q \in \cI^3_{\alpha}$ and therefore $Q \in \cI_{\alpha}$. We conclude that $Q$ is a solution for $I_{\alpha}$ with cost $$c(Q) = r \cdot |Q| - \sigma(Q) = r \cdot k - \sigma(Q) = r \cdot k - \alpha.$$ 
		
		For the second direction, let $\alpha \in [n^2] \setminus [z]$ and let $T$ be a solution for $I_{\alpha}$ with cost exactly $r \cdot k - \alpha$. Since $T$ is a solution for $I_{\alpha}$ it is a basis of $M_{\alpha}$ and it follows that $|T| = k$. 
		%
		%Note that if $|T| < k$ it holds that $$s(T) \leq (k-1) \cdot r+ \alpha \leq (k-1) \cdot r+n^2 < k \cdot r < k \cdot r+\alpha = D_{\alpha}.$$ Since in this case $T$ is not a solution for $I_{\alpha}$ we conclude that $|T| \geq k$; moreover, by \eqref{eq:1} it follows that $|T| = k$ since $T \in \cI_{\alpha}$.  
		%
		In addition, $$\sigma(T) = r \cdot |T|-c(T) = r \cdot k- c(T) = r \cdot k- (r \cdot k - \alpha) = \alpha.$$ Thus, since $T \in \cI_{\alpha}$, $|T| = k$, and $\sigma(T) = \alpha$, we conclude that $T \in \cI^3_{\alpha}$. Therefore, $T \in C(G)$ where $|T| = k$ as required.  
		%	For the first direction, let $Y \subseteq E$ be a solution for $X$, i.e., it holds that $v(Y) = T$ and $\sigma(Y) = D$. Let $k = |Y|$.  Observe that $c(Y) = \beta \cdot \sigma(Y) +v(Y) = \beta \cdot D+T = B$; moreover, $|Y| = k ,v(Y) = T$, and $\sigma(Y) = D$ and it follows that $Y \in \cI^3_k \subseteq \cI_k$. Thus, $Y$ is a feasible solution for $I_k$. Moreover, it holds that $p(Y) = \alpha \cdot k+\sigma(Y) = \alpha \cdot k+D$; thus, $Y$ is an optimal solution for $I_k$ by Claim~\ref{claim:aux1}. 
		%	
		%	For the second direction, let  $k \in [n]$ and let $S_k$ be an optimal solution for $I_k$ of profit exactly $k \cdot \alpha+D$. By Claim~\ref{claim:aux1} and that $p(S_k) = k \cdot \alpha +D$ it follows that $|S_k| \geq k$; we get that $|S_k| = k$ because $S_k \in \cI_k$. Moreover, it follows that $\sigma(S_k) = D$ to have that $p(S_k) = k \cdot \alpha +D$. Then, because $S_k \in \cI_k, |S_k| = k$, and $\sigma(S_k) = D$ it follows by \eqref{eq:1} that $v(S_k) = T$. Overall, we conclude that $S_k$ is a solution for $X$. %and $\sigma(S_k) = D$.  %, assume that there is no solution for $X$. 
	\end{proof}
	
	Given an FPTAS for CMB we can decide if there is a clique of size $k$ in $G$. We first consider the only value $\alpha' = z+1$ such that $I_{\alpha'}$ is possibly a pseudo CMB instance (i.e., may not have a feasible solution). In this case, we just check if the set $H$ of the $k$ items with the smallest values according to $\sigma$ is a clique in $G$; if $H \in C(G)$, we return that there is a clique of size $k$ in $G$. Otherwise, we iterate over all other values $\alpha \in  [n^2] \setminus ([z] \cup \{\alpha'\})$, and compute an optimal solution $S_{\alpha}$ for $I_{\alpha}$ using the FPTAS with parameter $\eps = \frac{1}{2 \cdot n^2}$ (these are all well defined instances). Note that the running time is polynomial since $\frac{1}{\eps}$ is polynomial in the input size. If there is $\alpha \in  [n^2] \setminus ([z] \cup \{\alpha'\})$ such that $c(S_{\alpha}) = r \cdot k-\alpha$, we return that here is a clique of size $k$ in $G$; otherwise, if for all $\alpha \in  [n^2]\setminus ([z] \cup \{\alpha'\})$  it holds that  $c(S_{\alpha}) \neq r \cdot k-\alpha$, we return that there is no clique of size $k$ in $G$. Note that $\OPT(I_{\alpha}) \leq n \cdot \max_{e \in E} c(e) = n^2$. Thus, 
	by the approximation guarantee of the FPTAS with our parameter $\eps$ it follows that $$c(S_{\alpha}) \leq (1+\eps) \cdot \OPT(I_{\alpha}) \leq \OPT(I_{\alpha}) + \frac{n^2}{2 \cdot n^2} < \OPT(I_{\alpha})+1.$$ Since the costs of all the elements are integers, we conclude that $c(S_{\alpha}) = \OPT(I_k)$. %We use the FPTAS with parameter $\eps = \frac{1}{3 \cdot n^3}$. 
	%Since for all $k \in [n]$ it holds that $\OPT(I_k)$
	
	By Claim~\ref{claim:alpha2} and Claim~\ref{claim:iff2} there is a clique of size $k$ in $G$ if and only if $H \in C(G)$ or there is $\alpha \in [n^2] \setminus ([z] \cup \{\alpha'\})$ such that $\OPT(I_{\alpha}) = r \cdot k-\alpha$. Therefore, we decide correctly whether there is a clique of size $k$ in $G$ in polynomial time. Since the $k$-clique problem is known to be NP-complete, we conclude that CMB does not have an FPTAS unless P=NP.
	$\blacksquare$
	
	
	
}






%\begin{tikzpicture}
%	\fill[gray, opacity=0.5] (0,0) rectangle (4,2);
%\end{tikzpicture}

% \begin{figure} %\hspace*{6cm}
%	%	\label{fig:2}
%	\begin{tikzpicture}[ultra thick]
%		\node[draw, rectangle, minimum width=5cm, minimum height=4cm] (R) at (0,0) {};
%		
%		\node[draw=none] at (4.8, 0) {Representative Set $\bf R$};
%		
%		\node[draw=none] at (-4, -0.5) {Exchange Set}; 
%		
%		\node[draw=none] at (0, 1.5) {$\bf {R \cap  \textcolor{teal}{\mathcal{K}_1(\alpha)}}$};
%		\node[draw=none] at (0, 0.5) {$\bf R \cap  \textcolor{red}{\mathcal{K}_2(\alpha)}$};
%		\node[draw=none] at (0, -0.5) {$\bf R \cap \textcolor{blue}{\mathcal{K}_3(\alpha)}$};
%		\node[draw=none] at (0, -1.5) {$\bf R \cap  \textcolor{brown}{\mathcal{K}_4(\alpha)}$};
%		
%		\draw ([yshift=-1cm]R.north west) -- ([yshift=-1cm]R.north east) 
%		;
%		\draw ([yshift=-2cm]R.north west) -- ([yshift=-2cm]R.north east) 
%		;
%		\draw ([yshift=+1cm]R.south west) -- ([yshift=+1cm]R.south east) 
%		;
%		\draw [decorate,
%		decoration = {calligraphic brace}] (-2.7,-1) --  (-2.7,0);
%		
%		\draw [decorate,
%		decoration = {calligraphic brace}] (2.8,2) --  (2.8,-2);
%		% \draw [decorate, decoration={brace, amplitude=10pt, mirror}, xshift=-6pt, yshift=0pt];
%		%([xshift=-6pt]R.south east) -- ([xshift=-6pt]R.north east);
%	\end{tikzpicture}
%	\caption{\label{fig:2} An illustration of our construction of a representative set $R$, using a union of exchange sets, one for each profit class $\mathcal{K}_1(\alpha)$, $\mathcal{K}_2(\alpha)$, $\mathcal{K}_3(\alpha)$, $\mathcal{K}_4(\alpha)$. }
%\end{figure}





%	\begin{figure}
%	\centering
%	\vspace{-4cm} 
%	\begin{tikzpicture}[scale=1.4, every node/.style={draw, circle, inner sep=1pt}]
%		\node (11) at (5.5,4) {$\bf \textcolor{teal}{1}$};
%		\node (22) at (7,4) {$\bf \textcolor{black}{2}$};
%		\node (33) at (5.5,3) {$\bf \textcolor{red}{3}$};
%		\node (44) at (7,3) {$\bf \textcolor{blue}{4}$};
%		\draw (11) -- (22);
%		\draw (11) -- (33);
%		\draw (11) -- (44);
%		\draw (22) -- (44);
%		\draw (33) -- (44);
%		
%		\node[draw=none] at (9, 3.5) {$~\Pi = \{\textnormal{independent sets of } G\}$};
%		
%		\node[draw=none] at (4.5, 3.5) {A graph $G$};
%		% Formula
%		\node[draw=none] at (6.75, 2.5) {$\mathcal{J}_{4,2} = \{\emptyset, \{$\bf \textcolor{teal}{1}$\},\{$\bf \textcolor{black}{2}$\},\{$\bf \textcolor{red}{3}$\},\{$\bf \textcolor{blue}{4}$\}\}, ~~\mathcal{K}_{4,2,5} = \{\{$\bf \textcolor{black}{2}$,$\bf \textcolor{blue}{4}$\},\{$\bf \textcolor{black}{2}$,$\bf \textcolor{teal}{1}$\},\{$\bf \textcolor{blue}{4}$,$\bf \textcolor{red}{3}$\},\{$\bf \textcolor{red}{3}$,$\bf \textcolor{teal}{1}$\}\}, ~~\mathcal{L}_{4,2,5}(\Pi) = \{\{$\bf \textcolor{black}{2}$,$\bf \textcolor{red}{3}$\}\}$};
%	\end{tikzpicture}
%	\vspace{-7.5cm} 
%	\caption{\label{fig:Pi} The independent sets of the $\Pi$-matroid $M_{n,k,\alpha}(\Pi)$, with parameters $n = 4$, $k = 2$, $\alpha = 5$. The secret set $\Pi$ contains all independent sets in the graph $G$, where $\{2,3\}$ is the only independent set in $G$ with $k$ elements.}
%	
%\end{figure}





==> guess.tex <==
%\section{Guessing Profitable elements}
%\label{sec:guess}

%In this section we describe the assignment of elements with relatively large profits 



\section{introduction}
\label{sec:introduction}

The problem of {\em budgeted matroid independent set (BMI)} consists of finding an independent set in a matroid with bounded {\em size} of maximal {\em profit}. TBA...

\section{Preliminaries}
\label{sec:preliminaries}

For the simplicity of the notation, for any set $A$ and some element $a$, let $A+a$, $A-a$ be $A \cup \{a\}$ and $A \setminus \{a\}$, respectively. In addition, for all $k \in \mathbb{N}$ let $[k]$ be the set $\{1,2,\ldots,k\}$. Finally, for any function $f:A \rightarrow B$ and $C \subseteq A$ let $f(C) = \sum_{\ell \in C} f(\ell)$. 

\subsection{Matroids}

Let $E$ be a finite {\em ground set} and let $\cI \subseteq 2^E$ be a non-empty set containing subsets of $E$ called the {\em independent sets} of $E$. Then, $\cm = (E, \cI)$ is a {\em matroid} if the following hold: 

\begin{enumerate}
	\item (The Hereditary Property) For all $A \in \cI$ and $B \subseteq A$ it holds that $B \in \cI$.
	
	\item(The exchange Property) For every $A,B \in \cI$ where $|A| > |B|$, there is $x \in A \setminus B$ such that $B +x \in \cI$. 
\end{enumerate}

Throughout this paper, determining whether a subset of elements forms an independent set of a matroid is assumed to be relied on an {\em oracle} and is considered to take polynomial time in the size of a matroid. Specifically, we assume that there is a polynomial time algorithm that given a matroid $\cm = (E, \cI)$ and a subset of elements $S \subseteq E$, returns "yes" if $S \in \cI$ and "no" otherwise. The next lemma gathers known results which follow from the definition of matroid (see, e.g., \cite{schrijver2003combinatorial} for more details). 


\begin{lemma}
	\label{lem:prel}
	
	The following hold for any matroid $\cm = (E, \cI)$. 
	%
	\begin{enumerate}
		
		\item For all $A,B \in \cI$ where $|A| \geq |B|$, there is $C \subseteq A \setminus B$, $|C| = |A|-|B|$ such that $B \cup C \in \cI$. 
		
		
		\item For every $F \subseteq E$ then $\cm - F = (E \setminus F, \cI')$ is a matroid where $\cI' = \{A \in \cI~|~ A \cap F = \emptyset\}$. 
		
		\item For every $F \in \cI$ then $\cm / F = (E \setminus F, \cI')$ is a matroid where $\cI' = \{A \subseteq E'~|~ A \cup F \in \cI\}$. 
		
		\item For every $q \in \mathbb{N}$ then $\cm^q = (E, \cI^q)$ is a matroid where $\cI^q = \{A \in \cI~|~ |A| \leq q\}$. 
	\end{enumerate}
	\comment{
	\begin{enumerate}
		
		\item For all $A,B \in \cI$ where $|A| \geq |B|$, there is $C \subseteq A \setminus B$, $|C| = |A|-|B|$ such that $B \cup C \in \cI$. 
		
		
		\item For every $F \subseteq E$ then $M - F = (E', \cI')$ is a matroid called the deletion of $F$ in $M$ where $E' = E \setminus F$ and $\cI' = \{A \in \cI~|~ A \cap F = \emptyset\}$. 
		
		\item For every $F \in \cI$ then $M / F = (E', \cI')$ is a matroid called the contraction of $F$ in $M$ where $E' = E \setminus F$ and $\cI' = \{A \subseteq E'~|~ A \cup F \in \cI\}$. 
		
			\item For every $q \in \mathbb{N}$ then $M^q = (E, \cI^q)$ is a matroid called the truncation of $q$ in $M$ where $\cI^q = \{A \in \cI~|~ |A| \leq q\}$. 
	\end{enumerate}
}
	\end{lemma}


\subsection{Matroid polytope}

%with $n$ elements numbered as $\{1,\ldots,n\}$
%A {\em basis} of $M$ is an independent set $B \in \cI$ such that for all $a \in E \setminus B$ it holds that $B+a \notin \cI$. Let $\textsf{bases}(M)$ be the set of all bases of $M$. Given a basis $B$ of $M$, 

Let $\cm = (E, \cI)$ be a matroid. Given $B \in \cI$, the {\em indicator vector} of $B$ is the vector $\bar{I}^B \in \{0,1\}^E$ where for all $i \in B$ and $j \in [n] \setminus B$ we have $\bar{I}^B_i = 1$ and  $\bar{I}^B_j = 0$, respectively. Then, the {\em matroid polytope} of $M$ is the convex hull of the set of indicator vectors of all independent sets of $\cm$: $P_{\cm} = \textsf{conv} \{\bar{I}^B~|~B \in \cI\}$. In addition, a {\em face} of a polytope $P$ is the intersection of P with any closed half-space whose boundary is disjoint from the interior of $P$. The next result is due to \cite{grandoni2010approximation}.

 \begin{lemma}
	\label{lem:integral}
	Let $\cm$ be a matroid and let $F$ be a face of dimension
	$d$ of the matroid polytope $P_{\cm}$. Then any $\bar{x} \in F$ has at most $2d$ non-integral
	components.
\end{lemma}


\subsection{Instance and Solution}

%For all $Q \subseteq E$, let $s(Q) = \sum_{\ell \in Q} s(\ell)$ and $p(Q) = \sum_{\ell \in Q} p(\ell)$. 

Formally, a BMI instance is a tuple $\ck =  (E,\cI,s,p)$, where $(E,\cI)$ is a matroid, $s:E \rightarrow [0,1]$  gives the element sizes and $p:E \rightarrow \mathbb{R}^+$ gives the elements profits. A {\em solution} of $\ck$ is an independent set $X \in \cI$ such that $s(X) \leq 1$; in addition, the {\em profit} of the solution is $p(X)$ and let $\OPT(\ck)$ denote the profit of a solution of $\ck$ with maximal profit. %In this section we prove the following result. 



\section{The Algorithm}
\label{sec:alg}


In this section an EPTAS for BMI is presented. The algorithm is relied on handling elements with high profit separately, where we find a small subset of elements from which the most profitable elements of the solution are chosen. Additional elements with lower profits are then added using a {\em linear program (LP)}. For the remainder of this section, fix a BMI instance $\ck =  (E,\cI,s,p)$ and a parameter $0<\eps<1$, where without the loss of generality, we assume that $\eps^{-1} \in \mathbb{N}$ and that for all $\ell \in E$ it holds that $\{\ell\} \in \cI$ (or this element can be omitted). For the flow of the reading, some of the more technical proofs are deferred to Section~\ref{sec:proofs}. 


In the following, we use rounding on profit of elements with relatively large profits. We start with computing a constant factor approximation of the optimum $\OPT(\ck)$. By the results of Grandoni and Zenklusen, the {\em $k$-budgeted matroid independent set} admits a PTAS \cite{grandoni2010approximation}. Since BMI is a special case of the latter problem with a single budget, using parameter $\eps' = \frac{1}{2}$, we can compute in polynomial time a solution $B^*$ of $\ck$ such that $p(B^*) \geq \frac{\OPT(\ck)}{2}$. Moreover, let $t = \eps^{-1}+1$ and let $h = \eps^t \cdot p(B^*)$. 

We say that an element $\ell \in E$ is {\em profitable} if $p(\ell) \geq h$ and {\em unprofitable} otherwise. Let $H$ denote the set of profitable elements; that is, $H = \{\ell \in E~|~ p(\ell) \geq h\}$. In our algorithm, we round the profits of the profitable elements down to the next multiple of $\eps \cdot h$; note that each elementmay lose only a small fraction of the profit by the above rounding (see Lemma~\ref{lem:J}). Formally, define the {\em profit classes} as $$T = \big\{r \cdot \eps \cdot h ~|~r \in \mathbb{N}_{>0}, r \cdot \eps \cdot h \leq 2 \cdot p(B^*)\big\}$$ which is the set containing the possible profits of profitable elements after the rounding. Now, define $\bar{p}: E \rightarrow \mathbb{R}^+$ as the {\em rounded profit function} such that for all unprofitable elements $\ell \in E \setminus H$ it holds that $\bar{p}(\ell) = p(\ell)$ and for all profitable elements $\ell \in H$ it holds that \begin{equation}
	\label{eq:max}
	\bar{p}(\ell) = \max_{\{y \in T~|~ y ~\leq ~ p(\ell)\}} y.
\end{equation} %Now, let $\cJ = (I,\mathcal{G},s,\bar{p},m,c)$ be the instance where the profits are rounded down as defined above. 


\begin{lemma}
	\label{lem:J}
	For any $A \subseteq E$ it holds that $\bar{p}(A) \geq (1-\eps) \cdot p(A)$. 
\end{lemma} 




Hence, by Lemma~\ref{lem:J} finding a solution with high profit w.r.t. $\bar{p}$ yields a solution with almost the same profit w.r.t. $p$; on the other hand, the number of distinct profits of profitable elements for $\bar{p}$ is bounded by a function of $\eps^{-1}$. Let $q = 2 \cdot \eps^{-t-1}$. By the next result, $q$ is an upper bound on the number of profitable elements in a solution of $\cm$ and on the number of profit classes. 

\begin{lemma}
	\label{q}
	For any solution $A$ of $\cm$ it holds that (i) $|H \cap A| \leq q$ and (ii) $|T| \leq q$. 
\end{lemma}



Our scheme finds a subset of the profitable elements $S$ of size bounded by $q^2$; these are the {\em chosen elements}. By enumerating over all subsets of the chosen elements,  we find $F \subseteq S$ which forms the set of profitable elements returned by the scheme. Then, additional unprofitable elements are added to $F$ using an LP. Surprisingly, despite the small number of chosen elements which depends solely on $\eps$, this simple approach loses only a small portion of the overall profit, in comparison to an optimal solution. 




The construction of $S$ is explained below.  For every profit class $y \in T$, let $E_y = \{\ell \in E~|~p(\ell) = y)\}$ be the subset of elements with profit $y$. For all $y \in T$, we construct a subset of elements $B_y \subseteq E_y$ independently of the remaining profit classes. Recall that the {\em truncation} of $q$ in $M$ is the matroid $M^q = (E,\cI^q)$ where $\cI^q = \{A \in \cI~|~ |A| \leq q\}$ contains all independent sets in $\cm$ with cardinality at most $q$. 

We construct $B_y$ by taking the independent set in $E_y \cap \cI^q$ with maximal number of elements (i.e., a {\em basis}) that has a minimal total size of elements. This can be computed easily by the following greedy approach. Let $E_y  = \{y(1), \ldots, y(n_y)\}$ be non decreasing order of $E_y$ by elementsizes; that is, for all $i,j \in [n_y], i \leq j$ we have $s\left(y(i)\right) \leq s\left(y(j)\right)$. Then, initialize $B_y = \emptyset$ and the next element$y(i) \in E_y$ according to the sorted order is added to $B_y$ if $B_y+y(i)$ forms an independent set in the truncation of $q$ in $M$. Finally, the chosen elements are $S = \bigcup_{y \in T} B_y$ that is the union of the elements chosen for $B_y$ for all profit classes. The algorithm for constructing the chosen elements is reffered to as Algorithm \textsf{Chosen} and the pseudocode of the algorithm is given in Algorithm~\ref{alg:chosen}. \ilan{I dont have time in this iteration by I have a suggestion for improving Algorithm Chosen: to define a minimal basis with at most $q$ elementfor each $E_y$, and in the algorithm just write that we take the union of the minimal bases of all $y \in T$.}


 \begin{algorithm}[h]
	\caption{$\textsf{Chosen}((E,\cI,s,p),q,T)$}
	\label{alg:chosen}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	\For{$y \in T$}{
		
		Initialize $B_y \leftarrow \emptyset$.
		
		Sort $E_y$ in non decreasing order by element ysizes $y(1), \ldots, y(n_y)$.\label{order}
		
		\For{$i = 1,\ldots,n_y$}{
			
			\If{$B_y + y(i) \in \cI^q$ \label{step:if}}{
				
				Update $B_y \leftarrow B_y+y(i)$
				
			} 
			
		}
		
	}
	
	Return $S = \bigcup_{y \in T} B_y$. 
\end{algorithm}




 
 
\begin{theorem}
	\label{lem:main}
	For all $G \in \cI^q$, where $G \subseteq H$, there is $Z \in \cI^q$,  where $Z \subseteq H$, such that the following hold. 
	
	\begin{enumerate}
		\item$s(Z) \leq s(G)$.
		
		\item For all $y \in T$ it holds that $|E_y \cap Z| = |E_y \cap G|$.
		
		\item$Z \subseteq S$. 
	\end{enumerate} 
\end{theorem} The proof of Theorem~\ref{lem:main} is given in Section~\ref{sec:lemMainProof}. Theorem~\ref{lem:main} is the key component in the analysis of the scheme: the profitable elements of an optimal solution may be replaced by a subset of the chosen elements with similar profit without increasing the total size of elements. However, for the unprofitable elements other techniques are required. 

For adding unprofitable elements to the solution, we use an LP based on a matroid polytope.  Let $F \subseteq H$ be some subset of the profitable elements. In the following, we define an LP whose objective is to find a subset of the unprofitable elements of maximal profit that together with $F$ forms a solution of $\cm$. Since $F$ may prevent an addition of an optimal subset of the unprofitable elements due to the matroid constraint, we restrict the potential unprofitable elements to be of significantly smaller profit in comparison with the elements in $F$. In the analysis, this turns out to be beneficial and decreases the potential profit only slightly by choosing an appropriate $F$. Formally, let \begin{equation}
	\label{E_F}
	E_F = \big\{\ell \in E \setminus H~|~ p(\ell) \leq \eps \cdot \min_{j \in F} p(j)\big\}
\end{equation} be the {\em potential elements} for $F$. The elements in $E_F$ are of profits bounded by $\eps$ times the minimal profit of an elementin $F$. Now, define the $F$-{\em matroid} as $M_F = (E_F,\cI_F)$ where  $\cI_F = \{A \subseteq E_F~|~ A \cup F \in \cI\}$. In other words, the $F$-matroid is the deletion of $E\setminus E_F$ in $M$ combined with the contraction of $F$ in $M$; hence, the $F$-matroid is indeed a matroid by Lemma~\ref{lem:prel} for $F \in \cI$. Finally, define the $F$-LP as the following relaxation of the problem:

 \begin{equation}
 	\label{LP}
 	\begin{aligned}
 		~~~~~ \max\quad        & ~~~\sum_{\ell \in E_F} \bar{x}_{\ell}   \cdot p(\ell)             ~~~~~~~~~~~~~~~~~~~~~                                                \\
 		\textsf{s.t.\quad} & ~~~\sum_{\ell \in E_F} \bar{x}_{\ell}  \cdot s(\ell)         \leq  1-s(F) ~~~~~~~~~~~~~~~~~~~~~           \\  
 		& ~~~\bar{x} \in P_{M_F} \\
 		%& ~~~\bar{x} \in [0,1]^{E_F} 
 	\end{aligned}
 \end{equation}  The $F$-LP maximizes the total profit of a point in the $F$-matroid, with total size of elements at most $1-s(F)$; that is, the residual capacity of a solution without the elements in $F$. In particular, observe that there is no solution to the $F$-LP if $s(F) > 1$ and there is only an all-zero solution in case that $F \notin \cI$.  In addition, observe that a vertex $\bar{\lambda}$ of the $F$-LP is in  a face of dimension $1$ (i.e., an edge) of the $F$-matroid polytope $P_{M_F}$, since the $F$-LP is obtained from $P_{M_F}$ by adding a single linear constraint for bounding the capacity. Hence, by Lemma~\ref{lem:integral} it follows that $\bar{\lambda}$ has at most $2$ non-integral entries. Using the above, we have the required components for designing the following EPTAS for BMI. 




 \begin{algorithm}[h]
	\caption{$\textsf{EPTAS}(\cm = (E,\cI,s,p),\eps)$}
	\label{alg:EPTAS}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	Construct $q,T$ using a $2$-approximation for BMI. 
	
	Construct the chosen elements $S = \textsf{Chosen}(\cm,q,T)$. 
	
	
	Initialize $A \leftarrow \emptyset$.\label{step:init}
	
	\For{$F \subseteq S$ \label{step:for}}{
		
		
		Find a vertex optimal solution $\bar{\lambda}^F$ of the $F$-LP and construct $C(F)$.\label{step:vertex}
		
			
			\If{$C(F)$ is a solution of $\cm$ and $p\left(C(F)\right) > p(A)$}{
				
				Update $A \leftarrow C(F)$\label{step:update}
				
			} 
			
		
	}
	
	Return $A$. 
\end{algorithm}

Let $S$ be the chosen elements returned by Algorithm \textsf{Chosen} on input $\cm,q,T$. For all subsets $F \subseteq S$, we find a vertex $\bar{\lambda}^F$ of the $F$-LP and round down the entries of $\bar{x}^F$: let $\bar{\gamma}^F \in \{0,1\}^{E_F}$ be the vector where $\bar{\gamma}^F_{\ell} = \floor{\bar{\lambda}^F_{\ell}}$.  In addition, let $\textsf{supp}\left(\bar{\gamma}^F\right) = \{\ell \in E_F~|~ \bar{\gamma}^F_{\ell} = 1\}$ be the {\em support} of $\bar{\gamma}^F$ and let the  {\em solution} of $F$ be the set $C(F) = F \cup \textsf{supp}\left(\bar{\gamma}^F\right)$. The solution of $F$ is called the {\em solution } of $F$ if it forms a solution of $\cm$. Finally, our algorithm chooses among the solutions of all $F \subseteq S$ a solution $C(F^*)$ with maximal total profit. The pseudocode of our scheme is given in Algorithm~\ref{alg:EPTAS}. For the following, let $|\cm|$ be the encoding size of $\cm$. 


\begin{lemma}
	\label{lem:runningTime}
	There is a function $f:\mathbb{R} \rightarrow \mathbb{R}$ such that Algorithm~\ref{alg:EPTAS} runs in time $f(\frac{1}{\eps}) \cdot |\cm|^{O(1)}$. 
\end{lemma} The following is the main result of this paper. 

\begin{theorem}
	Algorithm~\ref{alg:EPTAS} is an EPTAS for BMI.
\end{theorem}

\begin{proof}
	Let $\cm =  (E,\cI,s,p)$ be a BMI instance and let $0<\eps<1$. By Lemma~\ref{lem:runningTime}, the running time of Algorithm~\ref{alg:EPTAS} is of an EPTAS algorithm. In addition, by Step~\ref{step:init} and Step~\ref{step:update} of Algorithm~\ref{alg:EPTAS} the returned set $A$ is a solution of $\cm$. Therefore, by the above it suffices to show a lower bound on the profit of $A$. 
	
	Let $U$ be a solution of $\cm$ with profit $p(U) = \OPT(\cm)$. In the following we partition a subset (with possibly empty sets in the partition) of the profitable elements in $U$ into $\eps^{-1}$ disjoint sets. Formally, for all $i \in \left[\eps^{-1}\right]$ let 
	
	\begin{equation}
		\label{J_i}
J_i = \big\{\ell \in H \cap U~\big|~ p(\ell) \in \big[\eps^{i+1} \cdot p\left(B^*\right), \eps^{i} \cdot p\left(B^*\right) \big) \big\}		
	\end{equation}
	
 be all elements in $H \cap U$ with profits in the interval $\big[\eps^{i+1} \cdot p\left(B^*\right), \eps^{i} \cdot p\left(B^*\right) \big) $. Since $J_1,\ldots, J_{\eps^{-1}}$ are $\eps^{-1}$ disjoint  subsets of elements within $U$, there is $i^* \in \left[\eps^{-1}\right]$ such that $p(J_{i^*}) \leq \eps \cdot \OPT(\cm)$ as otherwise it implies that $p(U) > \OPT(\cm)$ in contradiction. Now, define $J_0 = (H \cap U) \setminus \bigcup_{i \in [\eps^{-1}]} J_i$ as the largest profitable elements in $H \cap U$ not counted in the above subsets; in addition, let $L =  \bigcup_{k < i^*} J_k$ (including $J_0$) be the {\em most profitable} and $Q = U \setminus (L \cup J_{i^*})$ the {\em less profitable} elements. 
 
 Since $L \subseteq H \cap U$, by the hereditary property and Lemma~\ref{q} it holds that $L \in \cI^q$; hence, by Theorem~\ref{lem:main} there is $Z \subseteq S$, where $S = \textsf{Chosen}(\cm,T,q)$, such that $s(Z) \leq s(L)$, for all $ y \in T$ it holds that $|Z \cap E_y| = |E_y \cap L|$ and $Z \in \cI^q$.  Then, because $Z \subseteq S$, there is an iteration of Algorithm~\ref{alg:EPTAS} such that $F = Z$ in Step~\ref{step:for}. We use the following auxiliary claim whose proof is given in Section~\ref{sec:proofs}.
	
	\begin{claim}
		\label{claim:x}
		There is a point $\bar{x}^*$ in the $Z$-LP such that $p(Z)+\sum_{\ell \in E_Z} \bar{x}^* \cdot p(\ell) \geq (1-3 \eps) \OPT(\cm)$.
	\end{claim}


	
	
	Recall the optimal vertex solution to the $Z$-LP, that is $\bar{\lambda}^Z$, constructed in Step~\ref{step:vertex} of Algorithm~\ref{alg:EPTAS} in the iteration for $F = Z$. Now, 
	
	
		\begin{equation*}
		\label{eq:p(x)}
		\begin{aligned}
			p(A) \geq p(C(Z)) \geq  p(Z)+\sum_{\ell \in E_Z} \bar{\lambda}^Z \cdot p(\ell) -2\eps \cdot p(B^*) \geq (1-3 \eps) \OPT(\cm) - 2\eps \cdot p(B^*) \geq  (1-5 \eps) \OPT(\cm)
		\end{aligned}
	\end{equation*} The first inequality is because $Z \in \cI$ and $s(Z) \leq s(L) \leq s(U)$; it follows that $C(Z)$ is a solution of $\cm$ and $A$ is updated in Step~\ref{step:update} to be a solution of at least the same profit. The second inequality is because \eqref{LP} is in a face of dimension $1$ of $P_{M_Z}$; then, by Lemma~\ref{lem:integral} there are at most $2$ fractional entries in $\bar{\lambda}^Z$; in addition, the fractional entries correspond to elements in $E_Z$ with profits at most $\eps p(B^*)$ by \eqref{E_F} and \eqref{J_i}. The third inequality is by Claim~\ref{claim:x} and because $\bar{\lambda}^Z$ is an optimal solution to the $Z$-LP. The last inequality is because $B^*$ is a solution of $\cm$. By the above and using parameter $\delta = \frac{\eps}{5}$, we have an EPTAS for BMI. 
	%(\max\{|Z|-|Q|,0\}) \eps^{i^*+1} \cdot p(B^*)  

\end{proof}

\comment{arg1
We construct the {\em profit classes} as the set containing the possible profits of profitable elements after the rounding (i.e., by $\bar{p}$), that is $T = \{\bar{p}(\ell)~|~\ell \in H\}$ and assume that for all $\ell \in I$ it holds that $p(\ell) \leq \OPT(\cI)$ since otherwise $\ell$ does not belong to any solution of $\mathcal{I}$.


\begin{lemma}
	\label{T}
	$|T| \leq q$. 
\end{lemma}

\begin{proof}
	
	
	Let $r^* =  \max_{\{r \in \mathbb{N}~|~ r \cdot \eps \cdot h \in T\}} r$. If $r^* >q$, it holds that there is an element$\ell \in E$ such that $$p(\ell) = r^* \cdot \eps \cdot h > q \cdot \eps \cdot  h = 2 \cdot \eps^{-t-1} \cdot \eps \cdot \eps^{t} \cdot p(B^*) = 2p(B^*)  \geq \OPT(\cm).$$ We reach a contradiction since for all $\ell \in E$ it holds that $p(\ell) \leq \OPT(\cm)$ and the claim follows. 
	
\end{proof}
}


\comment{



In the following we describe the construction of a subset of elements $S \subseteq I$ for the proof of Theorem~\ref{thm:guess}. Let $y \in T$  be a profit class. We choose up to $2q$ groups, and from each group we take up to $2q$ elements with profit $y$ for $S$. This is done greedily, where we take elements small as possible as explained next more concretely.  

We define the following order on $\cG$. Let $y \in T$ be a profit class. Let $\cG_y = \{G \in \cG~|~\exists \ell \in G \text{ s.t. } p(\ell) = y\}$. For all $G \in \cG_y$, let \begin{equation}
	f_y(G) = \min_{\ell \in G \text{ s.t. } p(\ell) = y} s(\ell).
\end{equation} In words, $f_y(G)$ is the minimal size of an elementin $G$ with profit exactly $y$.  Let $|\cG_y| = n$ and let $G_1, \ldots, G_n$ be a non decreasing order of $\cG_y$ by the function $f_y$. Finally, let $q_y = \max\{2q, |\cG_y|\}$. These are the {\em chosen groups} for $y$ and let $F(y) = \{G_1, \ldots, G_{q_y}\}$ be this set of groups. For each chosen group $G \in F(y)$ we choose the {\em chosen elements} as follows. Let $G(y) = \{\ell \in G~|~p(\ell) = y\}$ be the elements in $G$ with profit $y$. Now, let $\ell_1, \ldots, \ell_{\alpha}$ be the elements in $G(y)$ according to a non decreasing order by the elementsizes (the function $s$). We define the chosen elements as the set $G^i(y) =  \{\ell_1, \ldots, \ell_{\beta}\}$ where $\beta = \min\{2q, |\cG(y)|\}$ elements in the above order. 

Finally, let the $y${\em-elements} be the union of the chosen elements for all chosen groups of $y$:  $S_y = \bigcup_{i \in [q_y]} G^i(y)$. Then, our algorithm then computes the union of the $y$-elements for all profit classes $y \in T$. That is, $S = \bigcup_{y \in T} S_y$. The pseudocode of Algorithm \textsf{Profitable} is given in Algorithm~\ref{alg:guess}. 


\comment{arg1
	\begin{equation}
		\label{D}
		S_y = \bigcup_{i \in [q_y]} G^i(y). 
\end{equation}} 


\begin{algorithm}[h]
	\caption{$\textsf{Profitable}(\mathcal{I} = (I,\cG,s,p,m,c), \eps)$}
	\label{alg:guess}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	For each $y \in T$ compute the $y$-elements $S_y$. 
	
	Return $S = \bigcup_{y \in T} S_y$. 
\end{algorithm}


\begin{lemma}
	\label{S}
	$S$ returned by Algorithm~\ref{alg:guess} satisfies $|S| \leq \exp(\eps^{-3})$.
\end{lemma}

\begin{proof}
	We use the following inequality:
	
	\begin{equation}
		\label{q3}
		\begin{aligned}
			q^3 ={} & \left(\ceil{2 \cdot \eps^{-t-1}} \right)^3 \leq \left(2 \cdot \eps^{-t-1}+1\right)^3 \leq \left(2 \cdot \eps^{-t-1}+2 \cdot \eps^{-t-1}\right)^3 \leq  \left(\eps^{-t-2}\right)^3 \\ 
			\leq{} &	\left(\eps^{-\eps^{-1}-3}\right)^3 \leq 	\left(\eps^{-2\eps^{-1}-}\right)^3 = \eps^{-6\eps^{-1}} \leq \eps^{-\eps^{-2}}   \leq \exp(\eps^{-1})^{\eps^{-2}} \leq \exp(\eps^{-3}). 
		\end{aligned}	
	\end{equation} The inequalities follow since $0<\eps<0.1$. Now, 
	
	$$|S| = \left|\bigcup_{y \in T} S_y\right| \leq \bigcup_{y \in T} \left|S_y\right| \leq |T| \cdot 2q\cdot 2q \leq 4q^3 \leq 4 \exp(\eps^{-3}) \leq \exp(\eps^{-4}).$$ The second inequality is by the definition of the $y$-elements. The third inequality is by Lemma~\ref{T}. The fourth inequality is by \eqref{q3}. 
\end{proof}

\begin{lemma}
	The running time of Algorithm~\ref{alg:guess} is $f(1/\eps) \cdot |\cI|^{O(1)}$. 
\end{lemma}

\begin{proof}
	Computing $X$ is polynomial in $ |\cI|^{O(1)}$ by \cite{fleischer2011tight}. Then, we can also compute $\cJ$ in polynomial time. As $|T|$ and $q$ are bounded by a function of $1/\eps$, we can also compute the $y$-elements for all $y \in T$ in polynomial time. 
\end{proof}

For the proof of Theorem~\ref{thm:guess}, given an optimal solution $Z$ of $\mathcal{J}$ we construct a solution as explained next. This requires some definitions. Let $A$ be a solution of $\mathcal{J}$ and let the profitable elements assigned to a bin of $A$ be $$\textsf{elements}(A) = H \cap \bigcup_{i \in [m]} A_i.$$ Moreover, let $\cG_A = \{G \in \cG~|~ G \cap \textsf{elements}(A) = \emptyset\}$ be the set of groups that do not contain a profitable elementin the solution $A$. For all $\ell \in I$, $G \in \cG$ such that $\ell \in G$, let $\textsf{group}(\ell) = G$ be the {\em group of} $\ell$. Finally, for all $y \in T$ let $S_y[A] = \{\ell \in S_y ~|~ \textsf{group}(\ell) \notin \cG_A\}$ be the elements in $S_y$ of groups disjoint to the solution $A$ and let the elementof smallest size in this set be\footnote{assume that the elements have distinct sizes, or choose arbitrarily an elementof smallest size.}

\begin{equation}
	\label{item}
	\ell_y[A] = \arg \min_{\ell \in S_y[A]} s(\ell). 
\end{equation} Furthermore, let $A_y = \textsf{elements}(A) \cap \{\ell \in I ~|~p(\ell) = y\}$ be profitable elements in $A$ with profit $y$. We do the following process. We start with an optimal solution $Z^0$ for $\mathcal{J}$. If there is $y \in T$ such that $Z^0_y \setminus S \neq \emptyset$, then let  $i \in [m]$ such that there is $\ell \in (Z^0_i \cap Z^0_y) \setminus S$; we define an {\em exchange} in $Z_i$: let $Z^1_i = (Z^0_i \setminus \{\ell\}) \cup \{\ell_y[Z^0]\}$ and for all $j \in [m] \setminus \{i\}$ let $Z^1_j = Z^0_j$; finally, let $Z^1 = (Z^1_1, \ldots, Z^1_m)$ be the solution after one iteration and let $S^1 = S \setminus \{\ell_y[Z^0]\}$.

In general, after $r$ iterations, the process finds $y \in T$ (if exists) such that $Z^r_y \setminus S^{r} \neq \emptyset$, then chooses arbitrary $i \in [m]$ such that there is $\ell \in (Z^{r}_i \cap Z^{r}_y) \setminus S^{r}$; we define an {\em exchange} in $Z^r_i$: let $Z^{r+1}_i = (Z^{r}_i \setminus \{\ell\}) \cup \{\ell_y[Z^{r}]\}$ and for all $j \in [m] \setminus \{i\}$ let $Z^{r+1}_j = Z^r_j$; finally, let $Z^{r+1} = (Z^{r+1}_1, \ldots, Z^{r+1}_m)$ be the solution after iteration $r$. The pseudocode of the process is given in Algorithm~\ref{alg:2}. 

\begin{algorithm}[h]
	\caption{$\textsf{solution}(\cJ, Z^0)$}
	\label{alg:2}
	
	Initialize $r = 0$. 
	
	
	\While{$\exists y \in T$ such that $Z^r_y \setminus S^{r} \neq \emptyset$ }{
		
		Let $i \in [m]$ such that there is $\ell \in (Z^{r}_i \cap Z^{r}_y) \setminus S^{r}$. 
		
		Let $Z^{r+1}_i = (Z^{r}_i \setminus \{\ell\}) \cup \{\ell_y[Z^{r}]\}$ and for all $j \in [m] \setminus \{i\}$ let $Z^{r+1}_j = Z^r_j$. 
		
		Let $Z^{r+1} = (Z^{r+1}_1, \ldots, Z^{r+1}_m)$
		
		Update $r \leftarrow r+1$. 
	}
	
	Return $B = Z^r$ and $A = (Z^r_1 \cap H, \ldots, Z^r_b \cap H)$. 
	
\end{algorithm}

%While there are $i \in [m]$, $\ell \in Z_i \setminus S$ such that $p(\ell) = y$, then let 

%We use the following bin structuring technique from \cite{jansen2010parameterized}. 
}

\section{Properties of the chosen elements}
\label{sec:lemMainProof}

In this section we prove Theorem~\ref{lem:main} mainly based on simple properties of matroids. %For all $y \in T$, By the following lemma, given some independent set $F$, each elementin $F$ can be replaced by an elementfrom the chosen elements, with the same profit and smaller size, while resulting in an independent set.  

\begin{lemma}
	\label{lem:1}
	For all $y \in T$, $F \in \cI^q$, and $d \in F \cap \left(E_y \setminus B_y \right)$, there is $b \in B_y$ such that (i) $F-d+b \in \cI^q$ and (ii) s$\left(b\right) \leq s(d)$. 
\end{lemma}


\comment{ \begin{equation}
		\label{R}
		R(i) = \{b_j~|~i \in [n], b_j < b_i\}
\end{equation}}

\begin{proof}
\comment{arg1	Let $n = |B_y|$ and for all $i \in [n]$ let $b_i$ be the $i$-th elementadded to $B_y$ in Algorithm \textsf{Chosen}; in addition, let $	R(i) = \{b_j~|~i \in [n], b_j < b_i\}$ be the first elements added to $B_y$ until the predecessor elementto $y(b_i)$.

 Let the elementadded to $B_y$ which satisfies (i) and with minimal size be \begin{equation}
		\label{b*}
		b^* = \arg \min_{\{b \in B_y ~|~  F-d+b \in \cI\}} s(b).
	\end{equation} If there is more than one such $b^*$ choose the first such elementadded to $B_y$. We use the following variable. First, if there is no $b \in B_y$ such that $F-d+b \in \cI$ then let $R = \emptyset$; otherwise, let $R = \{b \in B_y~|~ s(b)<s(b^*)\}$ be all elements added to $B_y$ before element$b^*$. Observe that for all $b \in R$ it holds that $s(b)<s(b^*)$ since $b^*$ is the first elementadded to $B_y$ with size $s(b^*)$. Assume towards a contradiction that $s\left(b^*\right) > s(d)$. We reach in two complementary cases, as follows. }


Define the subset of elements in $B_y$ satisfying (i) and (ii) as: 

\begin{equation}
	\label{R}
	R = \{b \in B_y~|~ F-d+b \in \cI^q, s(b) \leq s(d)\}. 
\end{equation} If $R \neq \emptyset$ the claim follows by \eqref{R}. Therefore, Assume towards a contradiction that $R = \emptyset$. Because $d \in F$, it follows that $|R|<|F|$. Then, by Property~1 of Lemma~\ref{lem:prel} there is $C \in F \setminus R, |C| = |F|-|R|$ such that $R \cup C \in \cI^q$. We use the following auxiliary claim. 

\begin{claim}
\label{dC}
$d \notin C$. 
\end{claim}
%Second, $|B| \leq |R|<|F| \leq q$ (recall that $F \in \cI^q$) and it holds that $|B| \leq q-1$. 
\begin{proof}
Assume towards a contradiction that $d \in C$; thus, since $R \cup C \in \cI^q$ and $\{d\} \subseteq C$, we get by the hereditary property that $R+d \in \cI^q$. Let $B$ be the temporary set $B_y$ right before Step~\ref{step:if} of Algorithm~\ref{alg:chosen} for $y(i) = d$. Observe that $B \subseteq R$ by \eqref{R} and by the ordering of the elements in Step~\ref{order} of Algorithm~\ref{alg:chosen}. Then, because $R+d \in \cI^q$ then by the hereditary property it follows that $B+d \in \cI^q$. Therefore, by Step~\ref{step:if} of Algorithm~\ref{alg:chosen}, we should add $d$ to $B_y$ and it follows that $d \in B_y$ in contradiction. 
\end{proof} 	Therefore, $|R \cup C| = |F|> |F-d|$ since $d \in F$; by the exchange property of $(E,\cI^q)$, there is $b^* \in (R \cup C) \setminus (F-d)$ such that $F-d+b \in \cI^q$. Since $C \subseteq F$ and $d \notin C$ by Claim~\ref{dC}, it holds that $C \subseteq F-d$; it follows that $b^* \in R$ in contradiction that $R = \emptyset$. 
%Observe that $d \notin R$ since $d \notin B_y$. 
\end{proof}

%We split the proof into two complementary cases and in each show the existence of $b^* \in B_y$ which satisfies (i) and (ii). 
	\comment{arg1
	\begin{itemize}
		\itemIf $|R| \geq |F|$. Then, it follows that $|R| \geq |F| > |F-d|$ since $d \in F$. Therefore, by the exchange property of $(E,\cI^q)$, there is $b^* \in R \setminus (F-d)$ such that $ F-d+b^* \in \cI^q$. Hence, by \eqref{R} we have that $b^*$ satisfies the conditions of the lemma.%By the definition of $R$ we have that $s(b)<s(b^*)$ in contradiction to \eqref{b*}.
		
		\itemIf $|R| < |F|$. 
	}
		
		


	\noindent{\bf Proof of Lemma~\ref{lem:main}}:  Let $Z \in \cI^q$ such that (a) $s(Z) \leq s(G)$, (b)  for all $y \in T$ it holds that $|E_y \cap Z| = |E_y \cap G|$ and $|Z \cap S|$ is maximal among all $Z' \in \cI^q$ satisfying (a) and (b). Assume towards a contradiction that there is $a \in Z \setminus S$ and let $y = p(a)$.  Because $a \notin S$ and $B_y \subseteq S$, by Lemma~\ref{lem:1} there is $b^* \in B_y$ such that (i) $Z-a+b^* \in \cI^q$ and (ii) $s(b^*) \leq s(a)$; we define $W = Z-a+b^*$. It holds that $s(W) = s(Z)-s(a)+s(b^*) \leq s(Z)$ by (ii). In addition, for all $y' \in T -y$ it holds that $|E_{y'} \cap W| = |E_{y'} \cap G|$ and $|E_{y} \cap W| = |E_{y} \cap G|$ because $a, b^* \in E_y$ and by (b). Furthermore, $|W \cap S| > |Z \cap S|$ because $a \notin S$ and $b^* \in S$. Hence, $W$ satisfies (a), (b) and $|W \cap S| > |Z \cap S|$ which contradicts the maximality of $|Z \cap S|$. \qed

\section{Deferred Proofs}
\label{sec:proofs}


	\noindent{\bf Proof of Lemma~\ref{lem:J}}: 
	We use the following inequality. For any $\ell \in H$, by \eqref{eq:max} there is $r \in \mathbb{N}$ such that $\bar{p}(\ell) = r \cdot \eps \cdot h$ and $p(\ell) < (r+1) \cdot \eps \cdot h$; therefore,  		\begin{equation}
			\label{claim:1}
			p(\ell)-\bar{p}(\ell) \leq (r+1) \cdot \eps \cdot h- r \cdot \eps \cdot h =  \eps \cdot h \leq \eps \cdot p(\ell).
		\end{equation} The first inequality is by \eqref{eq:max}. The second inequality is because $\ell \in H$. Now, 
%	\end{proof} 


	
	$$\bar{p}(A) = \sum_{\ell \in A} \bar{p}(\ell) \geq \sum_{\ell \in A} (1-\eps) \cdot p(\ell) = (1-\eps) \sum_{\ell \in A} p(\ell) = (1-\eps) \cdot p(A).$$ The inequality follows for all $\ell \in E \setminus H$ since $\bar{p}(\ell) = p(\ell) \geq (1-\eps) p(\ell)$; furthermore, for all $\ell \in H$ the inequality follows by \eqref{claim:1}.\qed






	\noindent{\bf Proof of Lemma~\ref{q}}: 
	We split the proof into the two parts (i) and (ii). 

\begin{itemize}
	\item(i). 	Assume towards a contradiction that there is a solution $A$ of $\cm$ such that $q < |H \cap A|$. Therefore, 
	
	
	
	\begin{equation}
		\label{contradiction1}
		\begin{aligned}
			p(A) ={} & \sum_{\ell \in A} p(\ell) \geq  \sum_{\ell \in H \cap A} p(\ell) \geq \sum_{\ell \in H \cap A} h   = h \cdot |H \cap A| > h \cdot q = \eps^{t} \cdot p\left(B^*\right) \cdot 2 \eps^{-t-1} \\ ={} & 2 \cdot p\left(B^*\right)  \eps^{-1} \geq \OPT(\cm) \cdot \eps^{-1}  >   \OPT(\cm). 
		\end{aligned}
	\end{equation} The second inequality is because for all $\ell \in H$ it holds that $p(\ell) \geq h$. The third inequality is by the assumption that $q < |H \cap A|$. the fourth inequality is because $B^*$ is a $2$-approximation for $\cm$. By \eqref{contradiction1} we reach a contradiction that $A$ is a solution of $\cm$ with profit strictly larger than $\OPT(\cm)$. 
	
	\item(ii). 	Let $r^* =  \max_{\{r \in \mathbb{N}~|~ r \cdot \eps \cdot h \in T\}} r$. If $r^* >q$, it holds that there is an element$\ell \in E$ such that $$p(\ell) = r^* \cdot \eps \cdot h > q \cdot \eps \cdot  h = 2 \cdot \eps^{-t-1} \cdot \eps \cdot \eps^{t} \cdot p(B^*) = 2p(B^*)  \geq \OPT(\cm).$$ We reach a contradiction since $A = \{\ell\}$ is a solution with $p(A) > \OPT(\cm)$. By the above, $|T| \leq |\{r \in[q]\}| = q.$ \qed
\end{itemize}

	\noindent{\bf Proof of Lemma~\ref{lem:runningTime}}: 
	
		\noindent{\bf Proof of Claim~\ref{claim:x}}: 
		Because $U \in \cI$ and $Q \subseteq U$, by the hereditary property it follows that $Q \in \cI$. We define a point in the $Z$-LP relied on the following defined subset of elements. First, if $|Z| > |Q|$ then define $C = \emptyset$. Otherwise, $|Q| \geq |Z|$; then, by Lemma~\ref{lem:prel} there is $C' \subseteq Q \setminus Z, |C'|  = |Q| - |Z|$ such that $Z \cup C' \in \cI$; in this case, define $C = C'$. Now, define $\bar{x}^* \in \{0,1\}^{E_Z}$ such that for all $\ell \in C$ define $\bar{x}^*_{\ell} = 1$ and for all $\ell \in E_Z \setminus C$ define $\bar{x}^*_{\ell} = 0$. It is shown below that $\bar{x}^*$ is in the $Z$-LP. Because $Z \cup C \in \cI$, it follows by the definition of the matroid polytope that $\bar{x}^* \in P_{M_Z}$, the matroid polytope of $Z$. In addition, $$\sum_{\ell \in E_Z} \bar{x}^* \cdot s(\ell) = \sum_{\ell \in C} s(\ell) \leq \sum_{\ell \in Q} s(\ell) = s(Q) \leq 1-s(U \setminus Q) \leq 1-s(L) \leq 1-s(Z).$$ By the above and by \eqref{LP}, it holds that $\bar{x}^*$ is in the $Z$-LP. For the profit, we use the following inequalities.
		
		\begin{equation}
			\label{eq:11}
			\begin{aligned}
				\eps \cdot p(Z)-p(Q \setminus C) \geq \eps \cdot p(Z)- |Z| \cdot \eps \cdot  \min_{\ell \in Z} p(\ell) \geq \eps \cdot p(Z)-\eps \cdot p(Z) = 0.
			\end{aligned}
		\end{equation} The first inequality is because $C \subseteq Q \setminus Z$, $|C|  = |Q| - |Z|$ or $C = \emptyset$ if $|Z| > |Q|$ and it follows that $|Q \setminus C| \leq |Z|$; in addition, by the definition of $E_Z$ all elements in $Q \setminus C$ are of profits at most $\eps \cdot \min_{\ell \in Z} p(\ell)$. In addition, 
		
		\begin{equation}
			\label{eq:p(x)2}
			\begin{aligned}
				p(Z)+p(Q) \geq{} & \bar{p}(Z)+p(Q)  =  (\bar{p}(L)+p(Q)) \geq  (1-\eps)\cdot p(L)+p(Q) \geq  (1-\eps) \left( p(L)+p(Q)\right) \\ = {} &  (1-\eps)  p(U \setminus J_{i^*}) \geq (1-\eps) (1-\eps)\OPT(\cm) \geq (1-2\eps)  \OPT(\cm). 
			\end{aligned}
		\end{equation} The first equality is because $Z,L \subseteq H$ and for all $y \in T$ it holds that $|Z \cap E_y| = |E_y \cap L|$. The second inequality is by Lemma~\ref{lem:J}. Therefore,
		
		\begin{equation*}
			\label{eq:p(x)}
			\begin{aligned}
				p(Z)+\sum_{\ell \in E_Z} \bar{x}^* \cdot p(\ell) ={} & p(Z)+\sum_{\ell \in C} p(\ell) = p(Z)+p(C) = p(Z)+p(Q) - p(Q \setminus C) \\ \geq{} & (1-\eps) (p(Z)+p(Q))+\eps \cdot p(Z)-p(Q \setminus C)  \geq (1-3\eps) \OPT(\cm).
			\end{aligned}
		\end{equation*} The last inequality is by \eqref{eq:11} and \eqref{eq:p(x)2}.  Hence, $\bar{x}^*$ satisfies the conditions of the claim. \qed

==> preliminaries.tex <==
	\section{Preliminaries}
\label{sec:prel}

%For the simplicity of the notation, for any set $A$ and some element $a$, let $A+a$, $A-a$ be $A \cup \{a\}$ and $A \setminus \{a\}$, respectively. 
%The above text was moved to the intro. --H
%\ariel{the line should be placed before the definition of matroids}


